Discrete Probabilistic Inverse Optimal Transport

Optimal transport (OT) formalizes the problem of finding an optimal coupling between probability measures given a cost matrix. The inverse problem of inferring the cost given a coupling is Inverse Optimal Transport (IOT). IOT is less well understood than OT. We formalize and systematically analyze the properties of IOT using tools from the study of entropy-regularized OT. Theoretical contributions include characterization of the manifold of cross-ratio equivalent costs, the implications of model priors, and derivation of an MCMC sampler. Empirical contributions include visualizations of cross-ratio equivalent effect on basic examples and simulations validating theoretical results.

==> AISTATS_2022/1-intro.tex <==
\section{Introduction}

%A common goal in machine learning is to infer, given some observations, estimate the model(s) that may have generated the observations. 
%Suppose, however, that the observed data are not the outcome of a single model, but a collection of models and the observed data they produce are an efficient assignment of models to instances. Such situations commonly occur among collections of individuals, where the possible outcomes are a constrained set, all of which must be covered. See
%In such situations, we may also wish to draw inferences about the underlying models, but in order to do so we must account for the interactions among individuals arising from the coupling process. This class of problems is naturally formalized via Inverse Optimal Transport (IOT). 

%\pat{set up the paper against prior work. assume squared noise on plan. do not understand underlying geometric structure}
%
%\pat{our contributions: 
%(1) describe geometry of underlying manifold 
%(2) Geometry provides insight into missing value problems
%(3) Algorithm for inference based on geometry (current algorithm, show it works for randomly generated matrix)
%(4) standardly assumed noise model iteracts with support (claim: high CR means more concentrated posterior, due to "fewer" manifolds in the same gaussian ball.)
%(5) improved inference for standard noise model based on cross ratios??? 
%-- Clever way for thinking about which manifolds are nearby, avoids computing sinkhorn over and over
%(6) Geometry provides insight into behavior of different possible noise models (multiple agents, noise on perceived costs)
%}

%A common goal in machine learning is to infer, given some observations, estimate the costs that underlie the observations. 
%Given a coupling of two discrete probability distributions, can we infer the underlying costs that explain the observed joint density? Such couplings appear commonly when one set is matched with a second set. Examples include inferring the underlying distances given transportation patterns, affinity between matched pairs \cite{}, and  \pat{FIXME}. The forward problem of computing stochastic couplings is typically formulated as Entropy regularized optimal transport. Here we investigate the problem of inferring underlying costs via Inverse entropy regularized Optimal Transport.  

Inverse Optimal Transport \citep{stuart2020inverse,li2019learning,paty2020regularized} has received less systematic attention than (entropy-regularized) Optimal Transport (OT) \citep{villani2008optimal,cuturi2013sinkhorn}. 
%Although researchers have studied IOT in migration \citep{stuart2020inverse} and matching problems \citep{li2019learning}, and through adversarial robustness \citep{paty2020regularized} formulation and investigation of the general problem of probabilistic inference of latent costs from stochastic couplings given priors has not been systematically undertaken. 
Formulation and investigation of the general problem of probabilistic inference of latent costs from stochastic couplings given priors has not been systematically undertaken.
Like EOT, IOT inherits interesting geometric structure from Sinkhorn scaling \citep{sinkhorn1964relationship}, which gives rise to natural questions about the nature of posterior distributions, the existence of samplers, and questions about the feasibility and effectiveness of inferences from observed couplings to underlying costs. 

In recent years IOT problems have been studied and applied in many areas. Practical examples include: (1) inferring the cost criterion of international migration (Stuart and Wolfram, 2020); (2) estimating the marriage matching affinity (Dupuy \textit{et al.}, 2019); (3) learning interaction cost function from noisy and incomplete matching matrix and make prediction on new matching (Li \textit{et al.}, 2019). These works provide methodologies to solve certain IOT problems, while in our article we provide a framework for analyzing the general problem to understand the geometric properties of probabilistic inverse optimal transport (PIOT).

Our contributions include: (1) formulating the PIOT problem and provide basic results; 
(2) characterizing the geometry of the support manifold of PIOT solutions along with the implications of prior distributions on posterior inference; 
(3) presenting MCMC algorithms for posterior inference which derives directly from properties
of Sinkhorn scaling; 
(4) demonstrating the ability of PIOT through simulating general examples.

%We investigate properties of PIOT with several contributions. We formalize the general problem and proving basic results; characterize the manifold of support of the posterior distribution along with the implications of prior distributions on posterior inference; and present MCMC algorithms for posterior inference which derives directly from properties of Sinkhorn scaling, and show by simulation that samplers are effective on synthetic problems.  
%Our third contribution is to explore the feasibility of inference in this model by simulation and by demonstration on a real-world performance of NBA basketball teams. We conclude by discussing implications of the approach and interesting directions for extending the work. 

\textbf{Notation:} $\mathbb{R}^*$ is non-negative reals,  
$\overline{\mathbb{R}^*}$ denotes the extended non-negative reals $ \mathbb{R}^* \cup \{+\infty\}$. 
$\Delta_k$ is the $k$-dimensional simplex.
For a space $X$, $\mathcal{P}(X)$ denotes the set of distributions over $X$. 
%All matrices are assumed to be non-negative, and have no zero rows or zero columns unless otherwise stated. 
Matrices are in uppercase and their elements are in the corresponding lowercase.
For a matrix $A_{m\times n}$, $\mathbf{a}_1, \dots,\mathbf{a}_{n}$ denotes columns of $A$. %$\text{Col}(M)$ denotes column normalization of $M$.
Column normalizing a matrix $A_{m\times n}$
with respect to a $n$-dim row vector $\nu$ is defined as 
$\text{Col}(A, \nu) = A \text{diag} (\frac{\nu}{\mathbf{1}_{m} A})$, 
where $\mathbf{1}_{m}$ is a $m$-dim row vector with each element equals to~$1$. 
`with respect to $\nu$' is omitted when $\nu = \mathbf{1}_{n}$. 
Row normalization is defined in the same fashion.

==> AISTATS_2022/2-theory.tex <==


\section{Background and Related Work}
%Consider the situation where data from a collection of models were observed and the inference needs to be made on the underlying interactions between those models.
%In this section we formalize such inference as probabilistic inverse optimal transport. 
%\pw{discuss, notations, name for H,  T and C, $t_{ij}, c_{ij}$}
%\pat{pull out all details about column normalization to make it fully general to dirichlet prior on cost}

Given two spaces $X = \{x_1, \dots, x_m\}$ and $Y = \{y_1, \dots, y_n\}$, 
let $T = (t_{ij})_{m\times n} \in (\mathbb{R}^*)^{m\times n}$ 
be a \textit{coupling} that records the co-occurrence distribution between $X$ and $Y$.
Note that $t_{ij}$ is allowed to be zero here.
%Each column of $P$ is indexed by an $h$ and each row of $P$ is indexed by a $d$.
Each element $t_{ij}$ represents the probability of observing $x_i$ and $y_j$ simultaneously. 
The interaction between $X$ and $Y$ can be captured by a \textit{cost matrix} 
$C = (c_{ij})_{m\times n} \in (\overline{\mathbb{R}^*})^{m\times n}$, 
where $c_{ij}$ measures the underlying cost of coupling $x_i$ and $y_j$. 
Hence, the probabilistic inference on the underlying structure over $X$ and $Y$ is then to obtain $P(C|T)$, 
the distribution over all possible $C$ given an observed coupling $T$.

%The total cost of a plan $T$ is defined to be $\langle C, T\rangle = \sum_{i\in \D, j\in \hp} c_{ij}t_{ij}$, the Frobenius inner product.
%Let the prior of $C$ be $P_0(C)$, a distribution over $(\mathbb{R}^*)^{m\times n}$. %($\mathbb{R}^*$ is the set of non-negative real numbers). 
%Then the inference on $C$ 
%can be concluded using Bayes Rule: $P_t(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$.

% \pw{How do we justify the assumption that $T$ is optimal, by assuming the underlying model is cooperative?}
% \pw{directly go for EOT or OT}

%Assuming the $T$ is obtained by minimizing the total cost, we may 
\textbf{Entropy regularized optimal transport} is an fundamental building block in modelling $P(C|T)$. 
Given a cost matrix $C$ and distributions $\mu,\nu$ over $X$ and $Y$ respectively, 
\textit{Entropy regularized optimal transport} (EOT) \citep{cuturi2013sinkhorn,peyre2019computational} solves the optimal coupling $T^{\lambda}$ that 
minimizes the entropy regularized cost of transfer $X$ with distribution $\mu$ into $Y$ with distribution $\nu$. 
Thus for a parameter $\lambda >0$: 
\begin{equation}\label{eq:eot}
T^{\lambda} = \text{argmin}_{T\in U(\mu, \nu)} \{\langle C, T\rangle - \frac{1}{\lambda} H(T)\}
\end{equation}
\noindent where $U(\mu, \nu)$ is the set of all couplings between 
between $\mu$ and $\nu$ (i.e. joint distributions with marginals $\mu$ and $\nu$), $\langle C, T\rangle = \sum_{i\in X, j\in Y} c_{ij}t_{ij}$ is 
the Frobenius inner product between $C$ and $T$, and $H(T) := - \sum_{i=1}^{m}\sum_{j=1}^{n} t_{ij} \log t_{ij}$ 
is the \textit{entropy} of $T$. $T^{\lambda}$ is called an \textit{optimal coupling} with parameter $\lambda$. 

\textbf{Sinkhorn scaling} is used to efficiently compute optimal couplings.
$(\mu,\nu)$-\textit{Sinkhorn Scaling (SK)} \citep{sinkhorn1964relationship} of a matrix M 
is the iterated alternation between row normalization of $M$ with respect to $\mu$ and 
column normalization of $M$ with respect to $\nu$. \citep{cuturi2013sinkhorn} proved that: 
given a cost matrix $C$, the optimal coupling $T^{\lambda}$ between $\mu$ and $\nu$ 
can be solved by applying $(\mu, \nu)$-Sinkhorn scaling on 
the \textit{negative exponential cost matrix} $K^{\lambda}$,
where $K^{\lambda} = e^{-\lambda C} = (e^{-\lambda\cdot c_{ij}})_{m\times n}$.
% \pw{include an example of Sinkhorn?}
% \pat{yeah. i think this will help when we need to define the inverse.}

\begin{example}\label{eg: sk}
Let $\mu =\nu=(\frac{3}{8},\frac{5}{8})$, 
$\tiny C = \begin{pmatrix} \ln 1 & \ln 2 \\
 \ln 4 & \ln 1 \end{pmatrix}$. 
For $\lambda=1$, we may obtain $T$ by applying SK scaling on
$\tiny K^{\lambda} = e^{-C} = \begin{pmatrix} 1 & 1/2\\ 1/4 & 1 \end{pmatrix}$:
first, row normalize $K^{\lambda} $ with respect to $\mu$ results:
$\tiny K_1^{\lambda} =  \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
Then column normalization of $ K_1^{\lambda}$ with respect to $\nu$ outputs 
$\tiny K_2^{\lambda} = \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
As $K_1^{\lambda}= K_2^{\lambda}$, the SK scaling has converged with $T = K_1^{\lambda}$.
In general, multiple iterations may be required to reach the limit.
\end{example}

Given a coupling $T$, the inference on the cost matrix $C$
can be formulated as an inverse entropy regularized optimal transport problem. 
%can be interpreted as map from an optimal coupling $T^{\lambda}$ to the set of all possible triples of cost and marginals $\{(\widehat{C}, \widehat{\mu},\widehat{\nu})\}$. 
Given $\lambda$, EOT is the map $\Phi$:$(\mathbb{R}^*)^{m\times n} \times \mathcal{P} (\mathbb{R}^{m}) \times 
\mathcal{P} (\mathbb{R}^{n}) \to \mathcal{P} ((\mathbb{R}^*)^{m\times n})$ with $\Phi(C, \mu, \nu) = T^{\lambda}$.
Therefore \textbf{inverse entropy regularized optimal transport (IOT)} can be defined as $\Phi^{-1}: T^{\lambda} \to \{(C, \mu,\nu)\}$,
where $\{(C, \mu,\nu)\}$ represents the preimage set of $T^{\lambda}$ under $\Phi$.


\begin{remark}
In IOT, when $T^{\lambda}$ is observed without any noise,
$T^{\lambda}$ completely determines $\mu$ and $\nu$. 
Indeed $(C, \mu,\nu) \in \Phi^{-1}(T^{\lambda})$ implies that
$T^{\lambda} \in U(\mu,\nu)$. Thus $\mu$ and $\nu$ must equal the row and column marginals of $T^{\lambda}$.
Hence we may reduce IOT into $\Phi^{-1}: T^{\lambda} \to \{C\}$. 

Further, note that $\Phi^{-1}: T^{\lambda} \to \{C\}$ 
is not well-defined as a function, 
since $T^{\lambda}$ does not uniquely determine cost $C$. 
For instance, any matrix $C'$ in form of 
$\tiny C' = \begin{pmatrix} \ln \alpha \cdot 1 & \ln \alpha \cdot 2 \\
 \ln \beta \cdot 4 & \ln \beta \cdot 1 \end{pmatrix}$, for $\alpha, \beta>0$
outputs the same optimal coupling $T$ as $C$ in Example~\ref{eg: sk}
%\pat{insert example here too? build off the SK one}
\end{remark}

%\pw{we probably may move the next two paragraphs into intro.}

\textbf{Related Work.} 
The forward OT problem has a long history and is an active field of research 
\citep{kantorovich1942translocation, villani2008optimal,peyre2019computational,genvay2016stochastic}.
Applications in machine learning include: 
supervised learning \citep{frogner2015learning}, Bayesian inference \citep{el2012bayesian}, generative models \citep{salimans2018improving},
Transfer learning \citep{courty2016optimal}, and NLP \citep{alaux2018unsupervised}. 

However, the inverse OT problem is much less studied. The few existing inverse OT papers \citep{dupuy2019estimating, li2019learning, stuart2020inverse}, 
to our best knowledge, all 
focused on obtaining a unique approximation of the `ground truth' $C^*$, even though $\Phi^{-1}(T)$ contains a set of cost matrices.
To output an estimate of $C^*$, existing approaches place constraints on the cost matrix. 
For example in \citet{stuart2020inverse}, $C$ has to be either a Toeplitz matrix or
determined by a given graph structure.
In \citet{li2019learning}, $C$ must be constructed from a metric over a space where both $X$ and $Y$ are able to embedded in, plus $X$ and $Y$ need to have the same dimensionality. In \citet{dupuy2019estimating}, the affinity matrix has a low-rank constraint.
These assumptions do not hold in general.

%Rather than adding another constraint, 
We aim to analyze the intrinsic properties and 
the underlying geometric structure of the set $ \{C\} = \Phi^{-1} (T^{\lambda})$ 
for the general case in the following sections.
%
% Other related approaches, largely the lovely work of Curturi and colleagues, formulate the problem as ground metric learning. 
% \citep{cuturi2014ground} proposed algorithms for Ground Metric Learning (GML) which learns a distance from labeled normalized histograms given a criterion.
% \citep{heitz2021ground} extended the work of GML to learn the ground metric where only a geodesic distance on a graph is considered.
% \citep{paty2020regularized} re-interpreted regularized OT problems as ground cost adversarial and solved for robust solutions under different regularization. 
%
To simplify the notation, we will omit the superscript $\lambda$,
and fix $\lambda = 1$ unless otherwise stated.
% Some results will be described in term of negative exponential cost matrix $K$. 
% Corresponding statements in terms of $C$ can be obtained by $K = e^{-C}$.
% % Prior $P_0(K)$ is set to be the distribution where each column is follows symmetric Dirichlet distribution with hyperparameter $\alpha$ independently.
% Since for any non-negative cost matrix $C$, elements in $K$ are in the range of $(0,1]$, which can be cross-ratio equivalently 
% converted into a $K$ in the prior by column normalization.
% Observed $T$ is assumed to be a positive matrix, the case when $T$ is non-negative can be derived using  machinery of \textit{maximal partial pattern} 
% developed in \citep{pei2019generalizing}.









\section{Probabilistic inverse optimal transport} \label{sec:piot}

%\pat{remind people of our goal?}-\pw{added}
%In this section, we formalize the general IOT problem through Bayesian inference, 
%analyze key properties of $\Phi^{-1}(T)$ and reveal its underlying geometric structure. 


\begin{definition}\label{def: PIOT}
Let $T$ be a noisy observation of the optimal coupling~$T^*$.
\textbf{Probabilistic inverse optimal transport} is defined as: 

\begin{equation} \label{eq: PIOT}
 P(C|T) = \int _{T^* \in (\mathbb{R}^*)^{m\times n}} P(C|T^*) P(T^*|T) d T^*,    
\end{equation}

where $\displaystyle P(C|T^*) $ is obtained through Bayes' Rule:
\begin{equation} \label{eq: bayes}
 P(C|T^*)  = \frac{P(T^*|C) P_0(C)}{P(T^*)},   
\end{equation}
$P_0(C)$ is a prior of cost matrix $C$ over $(\mathbb{R}^*)^{m\times n}$; 
$P(T^*) = \int P(T^*|C) P_0(C) \text{d} C$ is the normalizing constant;
Likelihood $P(T|C) = 1$ if $C\in \Phi^{-1}(T)$, otherwise $P(T|C) = 0$. 
$P(K|T)$ is used to denote the induced posterior on $K = e^{-C}$.
\end{definition}


\subsection{No observation noise}
%In this section, we study the case when the observation is perfect, i.e. $T^* = T$.
As a direct application of Definition~\ref{def: PIOT}, we have:
\begin{prop}\label{prop:piot}\footnote{Proofs for all results are included in the supplemental materials.}
$ P(C|T)$ is supported on the intersection between $\Phi^{-1} (T)$ and the domain of $ P_0(C)$. Moreover, we have that 
$\displaystyle P(C|T) = \frac{P_0(C)}{\int_{\Phi^{-1} (T)} P_0(C) \text{d} C}$.
\end{prop}

Therefore, characterization of $\Phi^{-1} (T)$ is essential to understand
the manifold where the posterior distribution $P(C|T)$ is supported on.

Notice that for any $C \in \Phi^{-1} (T)$, 
a Sinkhorn scaling of $K = e^{-C}$ results in $T$, and 
each step of Sinkhorn Scaling is a normalization which equivalent to 
multiplication of a diagonal matrix. We show that: 

\begin{prop}\label{prop:DAD}
Let $T$ be a non-negative optimal coupling of dimension $m\times n$. $C \in \Phi^{-1} (T)$ if and only if for every $\epsilon > 0$,
there exist two positive diagonal matrices $D^r = \diag\{d^r_1, \dots, d^r_m\}$ and $D^c =\diag \{d^c_1,\dots, d^c_n\}$ such that: 
$\displaystyle |D^r K D^c - T| < \epsilon$, where $K = e^{-C}$ and $|\cdot|$ is the $L^1$ norm. 
In particular, if $T$ is a positive matrix, then $C \in \Phi^{-1} (T)$ 
if and only if there exist positive diagonal matrices $D^r,D^c$ such that $D^r K D^c = T$, i.e.
\begin{equation}\label{eq:diag_equiv}
\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}    
\end{equation}

\end{prop}

Proposition~\ref{prop:DAD} identifies a key feature of matrices in $\Phi^{-1} (T)$. 
However, it is not easy to
verify whether an arbitrary matrix belongs to $\Phi^{-1} (T)$ nor reveal any underlying 
geometric structure of $\Phi^{-1} (T)$.

Towards these goals, we now introduce an equivalent condition: \textit{cross ratio equivalence} between \textit{positive} matrices, 
and show that the IOT set $\Phi^{-1} (T)$ can be completely characterized by $T$'s \textit{cross ratios}. 

\begin{definition}
Let $A, B$ be positive $m\times n$ matrices. $A$ is \textbf{cross ratio equivalent} to $B$, 
denoted by $A\overset{c.r.}{\sim} B$,
if all cross ratios of $A$ and $B$ are the same, i.e.
$$r_{ijkl}(A) := \frac{a_{ik} a_{jl}}{a_{il} a_{jk}} = \frac{b_{ik} b_{jl}}{b_{il} b_{jk}} := r_{ijkl}(B) $$
holds for any $i, j \in \{1, \dots, m\}$ and $k, l \in \{1, \dots, n\}$. 

\end{definition}

\begin{lemma}\label{lemma:cr_dr}
For two positive matrices $A, B$, 
$A \overset{c.r.}{\sim}B$ if and only if 
there exist positive diagonal matrices $D^r$ and $D^c$ such that $A = D^r B D^c$.
\end{lemma}



\begin{thm}\label{thm:IOT}
Let $T$ be an observed positive optimal coupling of dimension $m\times n$. 
Then $\Phi^{-1} (T)$ is a hyperplane of dimension 
$m+n-1$ embedded in $ (\mathbb{R}^*)^{m\times n}$, which consists all the cost matrices 
that of the form:
\begin{equation}\label{eq:cr_equiv}
 \Phi^{-1} (T) = \{C \in (\mathbb{R}^*)^{m\times n} | K= e^{-C} \overset{c.r.}{\sim} T\}.    
\end{equation}

\end{thm}

Cross ratio equivalence provides a strong connection between IOT and algebraic geometry.
Algebraically, cross ratios generate the set of algebraic invariants of matrix scaling.
Thus the set of all scale reachable matrices from a coupling $T$, 
i.e. $\Phi^{-1}_K(T) = \{K| D^{r}KD^{c}\} = \{K = e^{-C}| C\in \Phi^{-1}(T)\}$ forms an algebraic variety defined by the cross-ratios of $T$.
% For instance: the matrices $\tiny K = \begin{pmatrix} a & b \\ c & d \end{pmatrix} \in \mathcal{K}(T) $ for
% $\tiny T = \begin{pmatrix} 0.1 & 0.2 \\ 0.3 & 0.4 \end{pmatrix}$ (i.e. the set of possible negative exponential cost matrix) 
% are generic solutions to the equation $3ad-2bc=0$. 
Geometrically, the set $\Phi^{-1}_K(T)$ forms a special manifold \citep{fienberg1968geometry}.
$T$ is the unique intersection between $\Phi^{-1}_K(T)$ 
and the hyperplane determined by the linear marginal conditions.

\begin{remark}
Since a matrix $T$ and its normalization $T/\sum_{ij}(t_{ij})$ 
have the same cross ratios (hence have the same image under IOT),
we may relax the distribution constraint on the observed coupling $T$.
In this case, instead of probability, 
$t_{ij}$ represents the frequency of observing $x_i$ and $y_i$ simultaneously.
\end{remark}

\begin{example}\label{eg:hyperplane}
Let $\tiny T = \begin{pmatrix} 1 & 2 & 3\\ 2 & 3 & 1\end{pmatrix}$. 
$T$ has three cross ratios $r_{1212} (T) = \frac{3}{4}, r_{1213}(T) =\frac{1}{6} , r_{1223}=\frac{2}{9}$.
Only two are independent as $r_{1213}(T) = r_{1212}(T) * r_{1223} (T)$. Hence $\Phi^{-1}_K(T)$ 
is the solution set of the algebraic equation:
\begin{equation*}
\begin{aligned}[c]
\small
    \begin{cases}
      k_{11} k_{22}/ k_{12}k_{21} = 3/4\\
      k_{12} k_{23}/k_{13}k_{22} = 2/9
    \end{cases}
\end{aligned}
\Longleftrightarrow \qquad
\begin{aligned}[c]
\small
    \begin{cases}
      4 k_{11} k_{22} - 3 k_{12}k_{21} = 0\\
      9 k_{12} k_{23} - 2 k_{13}k_{22} = 0
    \end{cases}
\end{aligned}
\end{equation*}
Further as $k_{ij} = e^{-c_{ij}}$, we obtain that $\Phi^{-1}(T)$ is the 4-dim hyperplane defined by the linear equations:



% \begin{subequations} \label{eq:T_1}
% \small
%   \begin{align}
%     & c_{12}+c_{21} - c_{11}-c_{22} = \small{\ln 3/4} \label{eq:T_1a}\\
%     & c_{13}+ c_{21} - c_{11} - c_{23} = \ln 1/6 \label{eq:T_1b}
%   \end{align}
% \end{subequations}
\begin{subequations} \label{eq:T_1}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln (3/4) \label{eq:T_1a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_1b}
  \end{empheq}
\end{subequations}


% \begin{equation}\label{eq:T_1}
% \small
%     \begin{cases}
%       c_{12}+c_{21} - c_{11}-c_{22} = \ln\frac{3}{4}\\
%       c_{13}+ c_{21} - c_{11} - c_{23} = \ln \frac{1}{6}
%     \end{cases}
% \end{equation}
\end{example}


\begin{remark}\label{rmk:basis}
For a $m\times n$ matrix $A$, 
although there are $\binom{m}{2} \binom{n}{2}$ ways to choose $i,j,k,l$ to form cross ratios of $A$, 
not all are independent as seen in Example~\ref{eg:hyperplane}. 
A set of independent cross ratios that generates the entire collection of cross ratios is called a \textbf{basis}.
For example, it is easy to check that $\mathcal{B} = \{r_{1j1k}(A)| j = 2, \dots, m, k=2, \dots, n\}$ forms a basis for $A$.
\end{remark}

% \pw{The following paragraph may delete or simplified.}
% Another special case is when $T$ is a square matrix.
% Two square matrices are said to be \textit{\textbf{diagonal} ratio equivalent} 
% if the ratio between any two positive diagonals of the two matrices are the same (See definition and proofs in supplemental materials.).
% \citep{pei2019generalizing} showed that when $T$ is a square matrix, any $C \in \Phi^{-1} (T)$ is diagonal ratio equivalent to $T$.
% In the supplementary material, we prove that for positive square matrices, \textbf{diagonal} ratio equivalent coincides with cross ratio equivalent.
Observed $T$ is assumed to be a positive matrix for the rest of the paper,
the case when $T$ is non-negative can be derived using  machinery of \textit{maximal partial pattern} 
developed in \citep{pei2019generalizing}.

\textbf{Support manifold.} 
%Now we are ready to study the support manifold 
%of posterior distribution $P(C|T)$.
Since $\text{Supp}[P(C|T)] = \Phi^{-1} (T) \cap \text{Domain}[P_0(C)]$, 
different priors would add different constraints on $C$, which will result different submanifolds embeded in 
the hyperplane formed by $\Phi^{-1} (T)$.

For instance, suppose $P_0(C)$ follows a Dirichlet distribution over the entire matrix ~($\mathbf{P_1}$). 
Then 
$$\text{supp}[P(C|T)]  =\{C \in (\mathbb{R}^*)^{m\times n} | e^{-C} \overset{c.r}{\sim} T, \sum_{ij} c_{ij} = 1\}.$$
 

Notice that $K$ encodes the cross ratios of $T$, and to avoid the estimation of $\lambda$,
it is handy to directly put prior put over $K=e^{-C}$. 
For example, assume that $P_0(K)$ is the 
distribution where each column follows an independent Dirichlet distribution~($\mathbf{P_2}$) with hyperparameter $\alpha$.
% According to Proposition~\ref{prop:DAD}, we have:
% \[\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}\]
Then the domain of $P_0(K)$ is $\mathcal{P}(\mathbb{R}^{n})^{m}$. 
Therefore, based on Eq.~\eqref{eq:diag_equiv}, we have the intersection is of the form:
\begin{equation} \label{eq:supp_posterior}
    \text{supp}[P(C|T)] = \{ C | \exists D^{r} \text{ s.t. } K = \text{Col}(D^{r}T) \}
\end{equation}



% Since for any non-negative cost matrix $C$, elements in $K$ are in the range of $(0,1]$, which can be cross-ratio equivalently 
% converted into a $K$ in the prior by column normalization.
%\centerline{$\d
% %isplaystyle \text{supp}[P(C|T)] = \{ \widehat{C} \in (\mathbb{R}^{+})^{m\times n} | \exists D^{r} \text{ s.t. } \widehat{C} \text{ is column normalization of } D^{r}T \}$ }
\begin{remark}\label{rmk: one_free_column}
Eq.~\eqref{eq:supp_posterior} indicates that: \textbf{(i)} a known column of $K$ uniquely determines all the other columns. 
Indeed, denote the $j$-th column of $K, T$ by $\mathbf{k}_j, \mathbf{t}_j$. 
For a known column $\mathbf{k}_j$, let $d_i = k_{ij}/t_{ij} $ and $D^{r} = \diag\{d_1, \dots, d_m\}$. 
Then the $l$-th column $\mathbf{k}_l$ equals to the column normalization of $D^{r} \mathbf{t}_l$.
\textbf{(ii)} for any $\mathbf{v} \in \mathcal{P}((\R^+)^m)$, there exists a $K \in  \text{supp}[P(K|T)]$ such that $\mathbf{k}_j = \mathbf{v} $.
Therefore, we have:

\end{remark}

\begin{cor}\label{cor:proj_single_column}
Under prior $\mathbf{P_2}$,
the projection of $\text{supp}[P(K|T)]$ onto each column is a $(m-1)$-dimensional manifold that is homeomorphic to the simplex $\Delta_{m-1}$. 
\end{cor}
\textbf{Subspace of $\text{Supp}[P(C|T)]$.} 
\label{para:subspace}
Let $C_s$ be the submatrix of the cost $C$ 
that corresponds to $X_s\times Y_s$, where $X_s = \{x_1, \dots, x_{s_1}\} \subset X$, $Y_s = \{y_1, \dots, y_{s_2}\}\subset Y$.
In this section, we characterize the support of $P(C_s|T)$ as a subspace of $\text{Supp}[P(C|T)]$.

Denote the sub-coupling of $T$ corresponding to $C_s$ by $T_s$.
According to Eq.~\eqref{eq:diag_equiv} and Eq.~\eqref{eq:cr_equiv}, 
the projection of $\Phi^{-1}(T)$ onto the cost over $X_s\times Y_s$
is in form of:
\begin{align*}
 \Phi^{-1}_s(T) &:= \{C_s | C_{s} \text{ is submatrix of a } C \in \Phi^{-1}(T)\} \\
 & = \{C_s| \exists D^r_s, D^c_s \text{ s.t. } K_s = D^r_s T_s D^c_s \}\\
 & = \{C_s|  K_s=e^{-C_s},  K_s \overset{r.c.}{\sim} T_s\}
\end{align*}


$\text{Supp}[P(C_s|T)]$ is determined by  $\Phi^{-1}_s(T)$ and the prior $P_0(C)$.
Intuitively, $\text{supp}[P(C_s|T)]$ contains all the matrices $C_s \in  \Phi^{-1}_s(T) $ such that there exists a proper extension of 
$D^r_s, D^c_s$ to $D^r, D^c$ such that $D^rTD^c$ is in the domain of $P_0(C)$. 

Take prior $\mathbf{P_2}$ as an example. Since the domain for a column of $K$ is a copy of $\Delta_{m-1}$ as shown in Corollary~\ref{cor:proj_single_column}, 
the domain for a column of $K_s = e^{-C_s}$ is then
a copy of $\Sigma_{s_1} = \{\mathbf{k} = (k_1, \dots, k_{s_1}) \in (\mathbb{R}^+ )^{s_1}| k_{1}+\dots +k_{s_1} < 1\}$. 
Hence, $\text{supp}[P(C_s|T)] $ should be contained in the set :
\begin{align*}
\mathcal{W}&  = \{C^s |\exists \text{ diagonal matrices } D_s^r, D_s^c \text{ s.t. }  \\
& K_s = D_s^rT_sD_s^c  \text{ and } \mathbf{1}_{s_1} K_s = (\alpha_1, \dots, \alpha_{s_2}), \alpha_i < 1 \}    
\end{align*}

It is important to note that $\text{supp}[P(C_s|T)]$ is a proper subset of $\mathcal{W}$. 
As $K_s$ is a submatrix of $K$, the choice of $D_s^c$ must form a proper column normalizing constant of a $D^rT$. 
Thus, the choice of $D_s^c = \diag \{d^c_1, \dots, d^c_{s_2}\}$ must guarantee that there exist an extension of $D_s^r$, 
denoted by $D'^{r} = \diag\{D_s^r,d^r_{s_1 +1}, \dots, d^r_{m}\}$, with $d^r_{s_1 +1}, \dots, d^r_{m}>0$, 
such that the $j$-th column sum of $D'^{r} T$ is $1/d^c_j$.
Let $T_{m-s}$ be the submatrix of $T$ corresponding to $\{x_{s_1+1}, \dots, x_{m}\} \times Y^{s}$. We show that:
\begin{prop}\label{prop:submanifold}
$C_s \in \text{supp}[P(C_s|T)]$ if and only if there exists positive diagonal matrices $D_s^c, D_s^r$ such that $K_s = D_s^c T_s D_s^r$ and
the system of equations 
$(x_1, \dots, x_{m-s_1}) T_{m-s}  = (1/d^c_1, \dots, 1/d^c_{s_2}) - \mathbf{1}_s D_s^rT_s$ have a set positive solution for $\{x_1, \dots, x_{m-s_1}\}$.
\end{prop}



\textbf{Incomplete Observation.}
\label{para:missing_element}
%We characterize the support of $P(C|T)$, when $T$ has a missing element.
Say $T$ is observed with $t_{m1}$ missing. Then generically, we have: 

\centerline{$\text{supp}[P(C|T)] = \cup_{\widehat{T} \in U(T)} \text{supp}[P(C|\widehat{T})]$}

where $U(T)$ is the set of matrices with $T$ completed by a choice of $t_{m1}>0$.
Given a prior, say $\textbf{P1}$, we have: 

\vspace{0.5pc}

\centerline{$\text{supp}[P(C|T)]  =\{C | \exists t_{m1} >0 \text{ s.t. } K \overset{c.r}{\sim} \widehat{T}, \sum_{ij} c_{ij} = 1\}$}

where $\widehat{T}$ is $T$ with $t_{m1}$ as its $m1$-th element. With prior $\textbf{P2}$, according to \eqref{eq:supp_posterior} we have:
$$\text{supp}[P(C|T)] = \{ C | \exists D^{r}, t_{m1} >0, \text{ s.t. } K = \text{Col}(D^{r}\widehat{T}) \}$$


Moreover, according to Remark~\ref{rmk: one_free_column}, 
a known column $\mathbf{k}_l$ of $K$ completely determines 
another fully observed column. Hence with a missing element in the first column, 
$\mathbf{k}_l$ determines an one dimensional set $\mathcal{K}_1$ for $\mathbf{k}_1$.
% forms a line segment in $\Delta_{m-1}$.
In particular, let $D^{r} = \diag \{d_1, \dots, d_m\}$, where $d_i = k_{il}/t_{il}$.
We show that:
%$D^{r} = \diag \{k_{1l}/t_{1l}, \dots, k_{ml}/t_{ml}\}$
\begin{cor}\label{cor:missing_element}
Under prior $\mathbf{P_2}$, 
$\mathcal{K}_1$ is a line segment in $\Delta_{m-1}$ that can be parameterized as:
$\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} \in (0,\infty) \}$.
\end{cor}


% Then the line segment can be parameterized as 
% $\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} = \widehat{t}_{m1} \in (0,\infty) \}$.


Note that for different choice of priors, $\mathcal{K}_1$ could be a curve instead of a line segment. 
Denote the prior imposed constraint on $\mathbf{k}_1$ by $f_1(\mathbf{k}_1) = 0$,
the ratio imposed linear constraint on $\mathbf{k}_1$ by $f_i(\mathbf{k}_1) = 0$, where $f_i(\mathbf{k}_1) = k_{11}/k_{i1} - d_1*t_{11}/(d_i*t_{i1})$,
for $i = 2, \dots, m-1$.
Then $\mathcal{K}_1$ is the solution set for system of equations $\{f_1, f_2, \dots, f_{m-1}\}$.
With Dirichlet prior, $f_1$ is also linear, so $\mathcal{K}_1$ is a line segment. 




\subsection{With observation noise}
%In this section, we study the general case when there are observation noises. 

First, for any two observed couplings with the same dimension, we introduce a natural distance between 
their images under IOT.

\begin{cor}\label{cor:parallel}
Let $T_1, T_2$ be two positive matrices of dimension $m \times n$.
The hyperplanes $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
In particular, if $T_1 \overset{c.r.}{\sim}T_2$ then $\Phi^{-1}(T_1) = \Phi^{-1}(T_2)$.
Otherwise $\Phi^{-1}(T_1)$ is parallel to $\Phi^{-1}(T_2) $.
\end{cor}

Therefore, $\Phi^{-1}(T_1) , \Phi^{-1}(T_2)$ are either the same or parallel hyperplanes
embedded in $(\mathbb{R}^{+})^{m\times n}$. 
\textbf{The distance between IOT of $T_1$ and $T_2$}, denoted by $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$ 
is then well-defined to be the Euclidean distance between $\Phi^{-1}(T_1) $ and $\Phi^{-1}(T_2)$.

Moreover, $\Phi^{-1}(T) $ is completely determined by $T$'s cross ratios.
So $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$ can be expressed in term of cross ratios of $T_1$ and $T_2$.
We now illustrate how to obtain $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$.
\begin{example}
Let $T_1 = T$ in Example~\ref{eg:hyperplane}, 
$\tiny T_2 = \begin{pmatrix} 1 & 2 & 3\\ 3 & 2 & 1\end{pmatrix}$.
Then $\Phi^{-1}(T_1)$ is the hyperplane show in Eq.~\eqref{eq:T_1}.
Taking $r_{1212}, r_{1213}$ as $T$'s cross ratio basis, 
then we have $\Phi^{-1}(T_2)$ is: 

\begin{subequations} \label{eq: T_2}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln (1/3) \label{eq:T_2a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (1/3) \label{eq:T_2b}
  \end{empheq}
\end{subequations}


%Eq~\eqref{eq:T_1} and Eq~\eqref{eq:T_2} have the same coefficients, 
Both $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$ are intersections of two 5-dim hydroplanes 
(i.e. \eqref{eq:T_1a} $\cap$ \eqref{eq:T_1b} and \eqref{eq:T_2a} $\cap$ \eqref{eq:T_2b})
with the same coefficient, so they are are parallel. 
Let the Dihedral angle between \eqref{eq:T_1a} and \eqref{eq:T_1b} be $\theta$.
It is easy to check $\cos \theta = 1/2$. 
So %by law of cosines, 
we have \scalebox{0.9}{$d(\Phi^{-1}(T_1), \Phi^{-1}(T_1) ) = \sqrt{\ln^2 \frac{4}{9} + \ln^2 \frac{3}{2} -\ln \frac{3}{2} \ln \frac{4}{9}}$}.
%$d(\Phi^{-1}(T_1), \Phi^{-1}(T_1) ) = \sqrt{(\ln 1/3 - \ln3/4)^2 + (\ln 1/6 - \ln1/9)^2 - 2(\ln 1/3 - \ln3/4)(\ln 1/6 - \ln1/9) \cos \theta } $
\end{example}

\begin{remark}
The hyperparameter $\lambda$ in Eq.\eqref{eq:eot} can be viewed as a greedy data selection. 
For a forward EOT problem, $\lambda$ raises the cross ratios of $K=e^{-C}$ to a power of $\lambda$.
Hence, $\lambda$ either exaggerates or suppresses the cross ratios of $T$, 
depending on whether $\lambda$ is greater or less than $1$ \citep{wang2020mathematical}.
Conversely, given a backward IOT problem, for a fixed coupling $T$, the larger the $\lambda$ is assumed, 
the smaller the cross ratios of $K$ are. 
Moreover, for a pair of observed couplings $T_1$ and $T_2$, 
the equations for hyperplanes corresponding $\Phi^{-1} (T_1), \Phi^{-1} (T_2)$ with different choices of $\lambda$, only differ 
on the constants by a scalar, i.e. $d_{\lambda}(\Phi^{-1} (T_1), \Phi^{-1} (T_2)) = d(\Phi^{-1} (T_1), \Phi^{-1} (T_2))/\lambda$.
Therefore, the larger $\lambda$ is assumed, the smaller the distance between $\Phi^{-1} (T_1)$ and $\Phi^{-1} (T_1)$ are.
\end{remark}

Assuming uniform prior $P_0(C)$ over $(\mathbb{R}^*)^{m\times n}$, 
we now investigate $P(C|T)$ under two common noise types. 
Results for other specific priors can be obtained by restricting the generic results to the prior's domain.
Without loss, 
we will assume noise only occurs on one element of $T$, say $t_{11}$, 
as the general case may be treated as compositions of such.

\textbf{Bounded noise.} 
% Consider the case where elements of the noisy observation $T$ 
% is within a bounded distance away from the optimal coupling $T^*$.
Suppose that $t_{11}$ is perturbed 
by a uniform noise from $t^*_{11}$, i.e. $t^*_{11} = t_{11} + \epsilon$, 
where $\epsilon$ is a random variable with uniform distribution over $[-a, a]$, for $a>0$.
%Then according to Eq~\ref{eq: PIOT}, assuming uniform prior $P_{0}(C)$,
% $P(C|T)$ is a uniform distribution over it support.

Theorem~\ref{thm:IOT} and Corollary~\ref{cor:parallel} imply that 
$P(C|T)$ is supported on a collection of parallel hyperplanes 
within bounded distance away from $\Phi^{-1}(T)$. 
More precisely, we show:

\begin{prop} \label{prop: bounded_noise}
For a coupling $T$,  assume uniform observation noise on $t_{11}$ with bounded size $a$, 
$$\text{supp}[P(C|T)] = \cup_{T'\in \mathbb{B}_{a}(T)} \Phi^{-1}(T'),$$
where $\mathbb{B}_{a}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t'_{11}>0$, $|t'_{11} - t_{11}| \leq a$ and $t'_{ij} = t_{ij}$ for other $i, j$.
Moreover, $\Phi^{-1}(T')$ can be expressed as intersection of two hyperplanes (may be in different dimensions):
one with equation: $c_{11} + c_{22} - c_{21} - c_{12} = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$, 
and the other equation does not depend on the value of $t'_{11}$. Assume the angle between these two hyperplanes is $\theta$.
Then $d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \ln \frac{t_{11} + a}{t_{11} - a} /\sin \theta $, for $T_1', T_2' \in \mathbb{B}_{a}(T)$.
\end{prop}

\begin{example}\label{eg:bounded_noise}
Let $T$ be the same as Example~\ref{eg:hyperplane}.
Suppose there is a bounded noise $\epsilon$ on $t_{11}$ of size $a>0$.
Hence, $\text{supp}[P(C|T)]$ is the union of a collection of hyperplanes $\mathbb{B}_{a}(T)$ 
of the form for $\epsilon \in [-a, a]$:

\begin{subequations} \label{eq:T_1}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln [(3+3\epsilon)/4] \label{eq:T_3a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_3b}
  \end{empheq}
\end{subequations}

Let the angle between \eqref{eq:T_3a} and \eqref{eq:T_3b} be $\theta$.
Computation shows that $\sin \theta = \sqrt{3}/2$, Hence for $T_1', T_2' \in \mathbb{B}_{a}(T)$, 
$d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \sqrt{3}\ln (1+a)$.
\end{example}

\textbf{Gaussian noise.} Suppose that $t_{11}$ is perturbed 
by a Gaussian distribution from $t^*_{11}$ centered at zero, i.e. $t^*_{11} = t_{11} + \epsilon$, 
where $\epsilon \sim \mathcal{N}(0, \sigma^2)$ with standard deviation $\sigma >0$.

Gaussian distribution is defined over the entire real line, 
% $P(T^*|T)$ is supported on the set $\mathcal{L}(T)$ consists matrices $T'$ of the same dimension of $T$ 
% with the propriety that:
% $t'_{ij} = t_{ij}$ for $(i, j) \neq (1,1)$. 
so $\text{supp}[P(C|T)] = \cup_{T'\in \mathbb{L}_{a}(T)} \Phi^{-1}(T')$,
where $\mathbb{L}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t_{11}>0$ and $t'_{ij} = t_{ij}$ for $(i, j) \neq (1,1)$.
In particular, cross ratios of $T'$ that depend on $t_{11}$ can be any arbitrary number.
Hence, similar to the case of missing elements in $T$, 
$P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T^*)$.
In particular, we show:

\begin{prop} \label{prop: gaussian_noise}
Let $T$ be an observed coupling of dimension $m\times n$ with Gaussian noise on $t_{11}$.
Further, let $\mathcal{B}$ be a basis for cross ratios of $m\times n$ matrices, that contains only one cross ratio depending on $t_{11}$.
Eliminate the cross ratio depending on $t_{11}$ in $\mathcal{B}$, denote the new set by $ \mathcal{B}^{-}$. Then: 

\centerline{$\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$}
In particular, $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T')$ 
for any $T'\in \mathbb{L}(T)$.
\end{prop}

\begin{example}\label{eg:Gaussian_noise}
Let $T$ be the same as Example~\ref{eg:hyperplane}.
Suppose there is a Gaussian noise $\epsilon \sim \mathcal{N}(0, \sigma^2) $ on $t_{11}$.
Hence, $\text{supp}[P(C|T)]$ is the union of a collection of hyperplanes $\mathbb{L}(T)$ 
of the form:

\begin{subequations} \label{eq:T_4}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln [(3+3\epsilon)/4] \label{eq:T_4a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_4b}
  \end{empheq}
\end{subequations}

Here $3+3\epsilon >0$ and $\epsilon \sim \mathcal{N}(0, \sigma^2) $ imply that
$\epsilon \in (-1, \infty)$, which further suggests that Eq.~\eqref{eq:T_4a} does not put any restriction on 
$c_{12}+c_{21} - c_{11}-c_{22}$. Hence:
$$ \text{supp}[P(C|T)] = \{C| c_{13}+ c_{22} - c_{12} - c_{23} = \ln \frac{2}{9} \}.$$
\end{example}

\begin{remark}
In this case, $P(C|T)$ is not uniform over its support. 
According to Eq~\eqref{eq: PIOT}, $P(C|T) \propto P(T_C|T)$ where $T_C \in \mathbb{L}(T) $ and $K = e^{-C} \overset{c.r.}{\sim}T_C$.
In particular, $P(C|T)$ has the highest probability on the hyperplane $\Phi^{-1}(T)$. 
If further constraints are added to the cost matrix $C$ such that 
there is a unique $C \in \Phi^{-1}(T)$ that meets such constraints, 
then one may obtain a maximum a posteriori estimation of $C$.
This explains why the simulation for the general case~\footnote{\citet{stuart2020inverse} requires the diagonal elements of $C$ be zeros in the general case.} 
in Section~4.4 of \citep{stuart2020inverse} failed 
to identify a unique cost matrix: $P(C|T)$ is supported on an entire hyperplane. 
%In contrast, m
Maximum a posteriori estimations of $C$ were successfully obtained in both the 
graph and Toeplitz cases \citep{stuart2020inverse}. %\wt{Do they use MAP or just sampling the posterior?}
\end{remark}

% \pw{pictures within each subsection or all pictures in a simulation section?}
% \wt{Noise on marginals? Eg. when we do PIOT on NBA data, can we add noises on the original row marginals to make predictions? After we obtain the posterior distributions we samples sets of noisy row marginals, and then use the posterior as cost and noisy marginals to find OT plans. }

==> AISTATS_2022/3-experiment.tex <==

\section{Algorithm}

\textbf{Approximate inference via MCMC.}
%
Given a perfectly observed $T$ and $P_0(C)$, we propose a Markov Chain Monte Carlo (MCMC) method 
% based  on the Metropolis algorithm\citep{metropolis1953equation} 
for sampling $P(C|T)$ (see Algorithm 1).
%from the posterior distribution. 
%The cross-ratio of the generated cost matrices are the same as $T$. 
%
%The algorithm works as follows. %\footnote{We suppress the $\lambda$ superscript to simplify notation of iterations.} 
At iteration $i$, denote the current cost $C$ by $C^{(i)}$, $K^{(i)} = e^{-C^{(i)}}$.
We generate two vectors $D^r$ and $D^c$ with each element sampled from an exponential of a Gaussian distribution $\mathcal{N}(0,\sigma^2)$. 
$K^{(i+1)}$ is then obtained by $K^{(i+1)} = \diag{D^r}K^{(i)}\diag{D^c}$.
%and scale rows in $K^{(i)}$ by left multiplying $D^r$ and columns by right multiplying $D^n$ to give $K^{(i+1)}$. 
%We compute the probability of the cost matrix, $P($log$(K^{(i)} | \mu)$. 
The acceptance ratio, $r = \frac{P(-\ln (K^{(i+1)}) | T)}{P(-\ln(K^{(i)}|T)} \overset{(*)}{=} \frac{P_0(C^{i+1}, \beta)}{P_0(C^{i}, \beta)}$
%$r = \frac{P_0(C^{i+1})}{P_0(C^{i})} = \frac{P(\text{log}(K^{(i+1)}) | \theta)}{P(\text{log}(K^{(i)}) | \theta)}$, 
where $\beta$ is the hyperparameter of prior $P_0(C)$. %represents the parameters of the model. %\pw{check with wei-ting.}
Equality~$(*)$ holds because our proposal preserves the cross-ratios, so we are guaranteed to stay on the manifold of support. 
Therefore, $P(T|C)$ is always $1$ and is omitted (see Proposition~\ref{prop:piot}). 
We accept or reject the move by comparing the acceptance ratio to an uniform random variable, $u$, 
which concludes a single step of the MCMC algorithm. 
%
We refer this method as MetroMC.
%\pw{the algorithm should be on cost $C$, not $K$}
\begin{algorithm}\label{alg:MCMC}
\caption{ MetroMC } %for generating $K$}
Inputs: coupling $T$, variance $\sigma$, Prior parameters $\beta$, uniform random variable $u$ $\in$ [0, 1)\;
Initialization: $C^{(0)}=-\ln(K^{(0)})$; $K^{(0)}=T_{m\times n}$\;
\For{i = 1 to ITERMAX}{
    $D^{r} =$ exp$( N(0, \sigma * \mathbb{I}_{m}) )$\; %\text{ones}(m,n)$ \; 
    $D^{c} =$ exp$( N(0, \sigma * \mathbb{I}_{n}) ) $\;
    $K^{(i+1)}\leftarrow$ diag($D^r$) $K^{(i)}$ diag($D^c$)\;
    %$K^{\lambda}_{i+1}\leftarrow$ ColumnNormalize[diag($D^r$) $K^{\lambda}_i$ diag($D^c$)]\;
    $C^{(i+1)} = -\ln (K^{(i+1)})$\;
   $a$ $\leftarrow P(C^{(i+1)}| T) / P(C^{(i)}|T)$\;
    \eIf{a $>$ u}{
        Accept $C^{(i+1)}$\;
    }{
        Reject $C^{(i+1)}$\;
        $C^{(i+1)} \leftarrow C^{(i)}$
    }
}
Output: $\mathbf{C}$
\label{algo:MetroMC}
\end{algorithm}

\textbf{Metropolis-Hastings Monte Carlo method.}
%
We can avoid dealing with the parameter $\lambda$ by putting a prior on $K$. However, 
the MetroMC has long autocorrelation time for such priors. 
%does not work well for such priors. The inverse procedure involves scaling 
%the rows and columns of the observed coupling with exponential factors, and experiments show that symmetric proposal distribution used in MetroMC is not efficient (has very long autocorrelation time) 
%for $\mathbf{P}_2$. \pat{we should explain why this is so. it will not at all be obvious to the reader.} 
%\wt{Explain:} 
%The reason is that i
In each iteration, $K^{(i+1)}$ is obtained by \textit{multiplying} random factors on $K^{(i)}$, 
whereas $C^{(i+1)}$ is obtained by \textit{adding} random factors on $C^{(i)}$.
In more detail, rows of $K^{(i)}$ are scaled by exponential of Gaussian variables 
a lot of time only a few of rows are at the same scale. After the columns are normalized, 
the rows that have large scale will have most of the weight in a column, which means we will sample a lot on the boundaries of the support.
In order to improve the efficiency, we utilize the Metropolis-Hastings \citep{hastings1970monte} sampling method. 

Now we propose an algorithm to sample from $P({K|T})$ with a prior on $K$.
The sufficient condition for the ergodicity of the MCMC method is detailed balance, which is defined as
% \begin{equation}
% \pi(s)P(s'|s)=\pi(s')P(s|s'),
% \label{eq:detailed_balance}
% \end{equation}
% where $\pi$ is the equilibrium distribution and $P(s'|s)$ is the transition probability to any state s' given a state s. At the end of a MC simulation, we will have the target distribution $\pi(s)$. Eq.~\eqref{eq:detailed_balance} can be re-written as 
$\pi(K)Q(K'|K)A(K', K)=\pi(K')Q(K|K')A(K, K')$,
% \begin{equation}
% \pi(s)Q(s'|s)A(s', s)=\pi(s')Q(s|s')A(s, s'),
% \label{eq:detailed_balance_2}
% \end{equation}
where $\pi(K)$ is the stationary distribution, $Q(K'|K)$ is the proposal transition probability from a state $K$ to $K'$ and $A(K',K)$ is the acceptance probability which we choose
\begin{equation}
A(K', K)=\text{min} \left(1, \frac{P(K')}{P(K)}\frac{Q(K|K'))}{Q(K'|K)} \right).
\label{eq:acceptance_prob}
\end{equation}
We replace the acceptance probability $a$ in Alg.~\ref{algo:MetroMC} with Eq.~(\ref{eq:acceptance_prob}). We refer this algorithm as the MHMC.

The proposal transition probability $Q(K'|K)$ is defined as follows.
In each iteration of MHMC, we draw a random number $\epsilon_i$ from a Gaussian distribution $\mathcal{N}(0, \sigma^2)$, where $\sigma$ depends on the row sums of $K$.
More precisely, $\sigma=\sigma_0*s_i^{\gamma}+\delta$, where $\sigma_0$, $\gamma$, and $\delta$ are hyper-parameters for the model and $s_i = \sum_j K_{ij}$. 
$K' = \text{diag}(D_i^r) K$, where $D_i^r = e^{[0,..,0,\epsilon_i,0,...,0]}$.

We %use the Gibbs sampling method to 
scale a row at once, so in each step the acceptance ratio is reduced to $A(s_i'|s_i)$. To compute it we need 
$Q(s_i'|s_i)=F_N(x=\ln(s_i'/s_i), \mu, \sigma) $ and 
$Q(s_i|s_i')=F_N(x=\ln(s_i/s_i'), \mu', \sigma')$,
% \begin{align*}
% Q(s'|s)=&F_N(x=\ln\frac{s'}{s}, \mu=0, \sigma) \\
% Q(s|s')=&F_N(x=\ln\frac{s}{s'}, \mu'=0, \sigma'),
% \end{align*}
where $F_N(x, \mu, \sigma)$ is the Gaussian probability density function.% $\mathcal{N}(\mu, \sigma^2)$.
%Gaussian probability density function with mean = $\mu$ and standard deviation = $\sigma$ at $x$. Namely, 
% \begin{equation}
% F_N(x, \mu, \sigma) = \frac{1}{\sqrt{2\pi}}e^{-\frac{1}{2}\frac{(x-\mu)^2}{\sigma^2}}
% \label{eq:Gaussian_pdf}
% \end{equation}

% In our simulations, we sample the next state $s'$ based on the current state $s$. We take s to be the sum of the row/column being scaled, $\mu=\mu'=0$, the standard deviation $\sigma=\sigma_0*s^k+\delta$ where $\sigma_0$, $k$, and $\delta$ are hyper-parameters.
%

% Move to supplements
% \subsection{Auto-correlation function.}

% To monitor the efficiency of our MCMC method, we compute the auto-correlation function during the burn-in phase and choose the lags accordingly.

% The auto-correlation function is defined as
% \begin{equation}
% R(t)=\frac{1}{(N-t)\sigma^2}\sum_{l=1}^{N-t}\sum_{i,j}(K_{i,j}^{(l)}-\bar{K}_{i,j})\cdot(K^{(l+t)}_{i,j}-\bar{K}_{i,j}),
% \label{eq:autocorrelation}
% \end{equation}
% where $N$ is the total number of samples generated, (i,j) runs over all indices of the matrices $K$, $\bar{K}$ is the mean averaging over all the samples, and $\sigma_K^2=\sum_{i,j}\sigma_{K,i,j}^2$ is the variance. 


\section{Simulations on synthetic data}\label{sec:simulations}

%\subsection{Effects of matrix size on manifold behavior.}

\paragraph{Visualizing subspaces of $\text{supp}[P(K|T)]$.} Fig~\ref{fig:2x2_subspace}(a-c) illustrates 
support of $2\times 2$ subspaces $\text{supp}[P(K^s|T)]$, for a $4\times 4$ coupling $T$ under prior $\mathbf{P}_2$.
In each plot, a $T$ is sampled from a Dirichlet distribution \footnote{All observed coupling $T$ in this section are presented in the supplement material.}.
Consider submatrix %$\tiny K^s=\begin{pmatrix} k_{11}& k_{12} \\ k_{21} & k_{22}\end{pmatrix}$ 
$K_s = [[k_{11}, k_{12}],[k_{21}, k_{22}]]$ of $K$. 
According to section~\ref{para:subspace}, both columns $\mathbf{k}_1, \mathbf{k}_2$ of $K_s$ lie in a copy of $\Sigma_2$. 
Each colored triangle mark represents a uniformly sampled $\mathbf{k}_1$ from $\Sigma_2$. 
A sampled $\mathbf{k}_1$ determines a $D^r_s = \diag\{k_{11}/t_{11}, k_{21}/t_{21}\}$, 
which further determines a set $\mathcal{K}_2 $ for $\mathbf{k}_2$  shown by solid segment with the same color.
% the corresponding $\mathcal{K}^s_2$, the set of $\mathbf{k}^s_2$, is shown by solid segment with the same color,
Projection of $\mathcal{W}$ into the simplex corresponding to $\mathbf{k}_2$, denoted by $\mathcal{W}_2$, is shown by the dashed ray.
Here, $\mathcal{K}_2$ is obtained by: fix $\mathbf{k}_1 = (k_{11}, k_{21})^T$, 
further sample $k_{31}$ and $k_{41}$ to form the first column of $K$.
Then compute and plot the uniquely determined $\mathbf{k}_2$. 
As predicted in section~\ref{para:subspace}, $\mathcal{K}_2$ is only a subset of $\mathcal{W}_2$. 
The sizes and locations of $\mathcal{K}_2$ in $\mathcal{W}_2$ vary according to cross ratios of $T$.

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c c}
    \hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_1.png}}
            \put(60,60){\textbf{a.}}
        \end{picture}
        %\textbf{a.}\includegraphics[width=0.2\textwidth]{figs/submat_1.png}
        &\hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_2.png}}
            \put(60,60){\textbf{b.}}
        \end{picture}
    %\end{tabular}
    %\begin{tabular}{c c}
        &\hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_3.png}}
            \put(60,60){\textbf{c.}}
        \end{picture}
    %     &\hspace{-7pt}
    %     \begin{picture}(50,50)% width and height of the picture
    %         \put(0,0){\includegraphics[width=0.12\textwidth]{figs/submat_4.png}}
    %         \put(40,40){\textbf{d.}}
    %     \end{picture}
    \end{tabular}
    \caption{
    Visualization of $2\times 2$ subspaces of $\text{supp}[P(K|T)]$. 
    In each plot, a $T$ is sampled from a Dirichlet distribution. 
    Each colored mark represents a uniformly sampled $\mathbf{k}_1 = (k_{11}, k_{21})^T$.
    Solid segment with the same color plots the corresponding set $\mathcal{K}_2$ for the second column, and
    the dashed ray plots $\mathcal{W}_2$. 
     }%Randomly generates the elements of first column of $K$ with $\sum_{i} K_{i,j} = 1$. Three sets of points are sampled for each plot and represented in different colors. Triangular points are ($K_{1,1}$, $K_{2,1}$) of first column; Lines are sets of points ($K_{2,1}$, $K_{2,2}$) of column 2.}
    \label{fig:2x2_subspace}
    \label{fig:subspace}
\end{figure}



%\subsection{Inferring censored values.}
\paragraph{Visualizing $\text{supp}[P(K|T)]$ with incomplete observations.} 

Fig.~\ref{fig:missing_element_T} illustrates the 
$\text{supp}[P(K|T)]$ for a $3\times 3$ observation $T$ with $t_{31}$ missing under prior $\mathbf{P}_2$. % \hl{FIXME}
%$T = [[5.84, 4.32, 4.10],[5.90, 9.00, 4.29],[t_{31}, 5.49, 7.18]]$ is constructed by sampling each element uniformly from $[0,10]$.
Columns of three sampled $K \in \text{supp}[P(K|T)]$ are plotted in three colored copies $\Delta_2$ as shown.
Here, three $\mathbf{k}_2$ are sampled uniformly from the middle $\Delta_2$. The uniquely determined $\mathbf{k}_3$ are shown in the right $\Delta_2$.
The corresponding set for $\mathbf{k}_1$ ($\mathcal{K}_1$) is plotted in the left $\Delta_2$.
$\mathcal{K}_1$ is obtained by uniformly sample a thousand $t_{31}$ from $[0,10]$. 
Each $t_{31}$ uniquely determines a $\mathbf{k}_1$.
As explained in Corollary~\ref{cor:missing_element}, 
each $\mathcal{K}_1$ forms a line segments. 
The slope of each line is determined by $T$'s cross ratios. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/missing_value_2.png}
    \caption{Visualization of $\text{supp}[P(K|T)]$ for a $3\times 3$ observed $T$ with $t_{31}$ missing.
    Three sampled $K \in \text{supp}[P(K|T)]$ are shown here with 
    each column is plotted in a copy of $\Delta_2$ as shown.
    Colored dots in the middle $\Delta_2$ represents uniformly sampled $\mathbf{k}_2$'s. 
    The uniquely determined $\mathbf{k}_3$'s are shown on the right, 
    the set $\mathcal{K}_1$ for the corresponding $\mathbf{k}_1$'s is shown on the left.}
    \label{fig:missing_element_T}
\end{figure}

%\subsection{Tests of MC samplers.}
% Supplement
% \pw{let's shorten?} \pat{move the whole section with the figure to supplement?}
% \textbf{Validation of MHMC.} In this section, we validate our MHMC algorithm by apply it to an uniform $T$, i.e $T_{m,n}=1/m$ 
% under prior $\mathbf{P}_2$.
% %on uniform matrices, e.g. $T_{m,n}=1/m$ for the column-wise Dirichlet prior case. 
% The cross-ratios of $T$ are all 1 and stay the same for all inferred sample $K^{(i)}$. 
% Thus, each $K^{(i)}$ has same copies of $n$ columns. 
% We compare posterior sample by MHMC to a 
% $m$-dimensional uniform symmetric Dirichlet distribution generated by the SciPy package \citep{2020SciPy-NMeth}.  

% %\footnote{Cite SciPy: https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.dirichlet.html}


% Fig.~\ref{fig:uniform_3x3} shows the results the 3x3 case.
% are the same for every element. We choose $\alpha=1$ for the Dirichlet prior, 
% $\sigma_0=0.5$, $k=3$, and $\delta=1.0$. 
% We run for 10,000 burn-in steps and take 10,000 samples 
% with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. 
% We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps.
% Also, the running averages of the row sums are stable at taking 10,000 samples, 
% which means 10,000 samples can effectively represent the posterior distribution. The plots for autocorrelation and running average are in appendix.

% % We perform our MHMC algorithm on a 3x3 uniform matrix with a symmetric column-wise Dirichlet prior, i.e. $\sum_i K^{(i)}_{i,j}=1$ and the Dirichlet concentration parameter $\alpha$ are the same for every element. We choose $\alpha=1$ for the Dirichlet parameter, $\sigma_0=0.5$, $k=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps. Also, the running averages of the row sums are stable at taking 10,000 samples, which means 10,000 samples can effectively represent the posterior distribution. The plots for autocorrelation and running average are in appendix.

% The posterior distribution is compared to the distribution $P(K|T)$ of three-dimensional vectors generated by Dirichlet vector sampler \citep{2020SciPy-NMeth} with symmetric $\alpha=1$ in Fig.~\ref{fig:uniform_3x3}. The results are comparable, which suggests that our MHMC method is able to generate distributions which well represent the support of the posterior distributions.


% \begin{figure}[h!]
%     \centering
%     \begin{tabular}{c c}
%         \hspace{-4pt}\includegraphics[width=0.235\textwidth]{figs/dirichlet_3.png}
%         \hspace{-6pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3.png}
%     \end{tabular}
%     % \begin{tabular}{c c}
%     %     \hspace{-4pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3_autocorr.png}
%     %     \hspace{-6pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3_running_avg.png}
%     % \end{tabular}
    
%     \caption{\textbf{(Left.)} \pat{row rather than square?} The distributions of each component of three-dimensional Dirichlet vectors with symmetric $\alpha=1$ generated using SciPy package. \textbf{(Right.)} The distributions of each component of the first column of $P(K|T)$ sampled by the MHMC method. %\textbf{(Lower left.)} The auto-correlation function of the MHMC simulation. The black dashed lines indicate the range [$-1/e$, $1/e$]. \textbf{(Lower right.)} The running average of the row sums of the MHMC simulation.
%     }
%     \label{fig:uniform_3x3}
% \end{figure}

\textbf{Visualizing $\text{supp}[P(K|T)]$ through MHMC.} Now we utilize MHMC to visualize supp[$P(K|T)$] and see the effect of cross-ratios. 
Under prior $\mathbf{P}_2$ with $\alpha =1$, Fig.~\ref{fig:sample_supp} illustrates the posterior distributions $P(K|T)$ of $3\times 3$ coupling $T$. 
% Here couplings $T$ are generated by solving an OT problem with uniform marginals $\mu, \nu$, and random column Dirichlet matrices $K^g$. 
% \pw{what is $K^g$}.

%We simulate $P(K|T)$ using MHMC with the same parameters as in the previous uniform matrix case 
%\pw{fix}. \wt{fixed}
We choose $\alpha=1$ for the Dirichlet prior $P_0(K)$, $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. 
The choices of these numbers are validated in Supplemental Material. 
Three columns (\textcolor{red}{red}, \textcolor{green}{green}, and \textcolor{blue}{blue} colors, respectively) 
of each $T$ are plotted on a one single simplex in the left of Fig.~\ref{fig:sample_supp}. 
Locations of these points illustrate the relations between each column encoded by the cross ratios of $T$. 
The right of Fig.~\ref{fig:sample_supp} plots columns of sampled $K$ from $P(K|T)$ with corresponding $T$ to the left. 
We clearly see how the cross-ratio of $T$ affects $P(K|T)$. 
If one column of $T$ is close to one edge, then the posterior distribution of that column will be denser on that edge; on the other hand, if a column of $T$ is located near the center, then the posterior is more evenly distributed on a simplex. 
%Since the relative location of each column should be kept to retain the cross-ratio equivalence for all inferred samples.
E.g. in the top case, the effects on red and blue are exaggerated because the effect depends on relative position (and similarly for the red in the middle panel). 

\begin{figure}[h!]
    \centering
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_1.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_1_1.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_1_2.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_1_3.png}
    \end{tabular}
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_2.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_2_1.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_2_2.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_2_3.png} 
    \end{tabular}
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_3.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_3_1.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_3_2.png} &
        \includegraphics[width=0.1\textwidth]{figs/random_3x3_simplex_3_3.png} 
    \end{tabular}
    \caption{\textbf{(Left.)} The columns of three $T$ matrices plotted on the same simplex: $\mathbf{t}_1,\mathbf{t}_2, \mathbf{t}_3 $ are shown in
    \textcolor{red}{Red}, \textcolor{green}{green} for , \textcolor{blue}{blue}. 
\textbf{(Right.)} Samples from posterior distribution $P(K|T)$. Each column of inferred matrices $K$ are plotted in a separate simplex, indicated by corresponding color.}
    \label{fig:sample_supp}
\end{figure}

% T_1 = [[0.1104, 0.0684, 0.1545],
%         [0.0505, 0.2401, 0.0428],
%         [0.1725, 0.0249, 0.1360]]

% T_2 = [[0.0950, 0.1100, 0.1283],
%         [0.1155, 0.0343, 0.1835],
%         [0.1228, 0.1890, 0.0215]]

%  T_3 = [[0.1053, 0.1193, 0.1088],
%         [0.2148, 0.0090, 0.1096],
%         [0.0133, 0.2051, 0.1150]]

% Appendix
% \textbf{MetroMC on uniform matrix.} We test MetroMC on 3x3 uniform $T$, where $T_{i,j}=1/(m*n)$, and assume the prior is put on $C$, i.e. $\sum_{i,j}C_{i,j}=1$. For this method, we need to first re-normalize $T$ so that $K^{(0)} = F(T)$ is on the support of the posterior manifold. F(T) is defined as
% \begin{equation}
%     F(T) = \text{exp}\left({\frac{1+\sum_{i=1}^{m}\sum_{j=1}^{n}\text{log}(T_{i,j})}{m*n}}\right).
% \end{equation}
% For each MC iteration we sample $m+n-1$ Gaussian random numbers with standard deviations of 0.02 for the diagonal matrices $D^r$ and $D^c$ satisfying the condition 
% \begin{equation}
% \sum_{i,j}\text{log}(D^r_{i})+\text{log}(D^c_j)=0. 
% \label{eq:condition_bounded_noises}
% \end{equation}
% We burn in 10,000 steps and take 100,000 samples with 100 lags in between. The Gaussian Kernel density estimation (KDE) of each component of $P(C|T)$ is demonstrated in Fig.~\ref{fig:uniform_3x3_2}. We use bandwidths of 0.05 for all the Gaussian KDE in this article. There are a few notable features. First, we assume a Dirichlet prior on the whole $C$ matrix, the distributions will be smaller at large values because each large value will suppress the value of the other elements. Second, since we have cross-ratio = 1 everywhere in $T$ and matrix-wise symmetric Dirichlet prior on $C$, there will not be a single element with value close to one. Otherwise, the cross-ratio involving that element could never be 1 anymore. Also, for the same reason all distributions should be similar.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/pdf_unifrm_T_3x3.png}
%     \caption{\pat{move to supplement?} The KDE of each matrix element of $P(C|T)$ with a uniform $T$ and a symmetric Dirichlet prior over the whole $C$ matrix.}
%     \label{fig:uniform_3x3_2}
% \end{figure}


\paragraph{Bounded noise on observed plan.}
Given an observed noisy $T$, 
we assume $t_{11}$ was perturbed by a bounded noise $\epsilon$ sampled uniformly 
from distribution $[-a, a]$ with $a=0.01$. 
Assuming prior $\mathbf{P}_1$ for $P_0(C)$ with symmetric Dirichlet parameter equals to $1$, 
we use MetroMC to sample $\text{supp}[P(C|T)]$.

% To see the effects of noise on the inferred cost we take five evenly spaced values within the range. A ground truth probability cost matrix $C^g$, whose elements are randomly rolled from a uniform distribution [0, 1] and normalized to $\sum_{i,j}C^g_{i,j}=1$, is generated and a OT problem is solved to obtain a plan $T^g$ with even marginals $\mu, \nu$ and $C^g$. For simplicity we do not add a random noise on $T^g$ to obtain the observed plan $T$, so $T=T^g$. 
%For the PIOT inference, the noise is added to the (1,1)-th element of the  observed plan $T$. 

% In order to make $-log(T)$ lie on the support of the posterior we re-normalize the plans upon performing the MCMC method by a factor $F(T)$.
% \pw{how about swap to }

Notice that initializing $K^{(0)} = T$ may cause the corresponding $C^{(0)}$ lies outside the domain of $P_0(C)$ as 
$\sum_{ij} c^{(0)}_{ij} = \sum_{ij} -\ln(t_{ij})$ is not guaranteed be $1$. This will cause an extremely 
long burning time. In order fix this issue, we scale $K^{(0)}$ by a constant when necessary.
Scaling does not change the cross-ratios, hence it equivalent to a move within $\Phi^{-1}(T)$. 

%We assume a symmetric Dirichlet prior on $P_0(C)$, where $\sum_{i,j}C_{i,j}=1$ and the Dirichlet parameters = 1 everywhere. 
For each iteration in the MCMC method we generate $m+n-1$ (rather than $m+n$) independent Gaussian random numbers 
with $\sigma = 0.02$ to construct vectors $D^r$ and $D^c$ 
satisfying $\sum_{i,j}\ln(d^r_{i})+\ln(d^c_j)=0$.
%eq.~\ref{eq:condition_bounded_noises}.
The purpose of the above condition is to ensure that the newly generated sample lies on the support of the posterior. Otherwise, the acceptance rate will be extremely low. Because $C$ is a positive matrix, the MetroMC method rejects any sample of $K$ if $\max_{(i,j)}k_{i,j}\ge 1$. 

Fig.~\ref{fig:bounded noise} shows the MetroMC results on the inferred cost matrices $C$ for a given $3\times 3$ coupling 
$T$. For each simulation we burn in 10,000 steps and take 100,000 samples with lags of 100. 
The acceptance rates range from 0.51 to 0.58.  Noise level $\epsilon$ is indicated by colors.
The \textbf{Left} panel plots components for a cross-ratio depend on $t_{11}$: $(c_{11}+c_{22})$ by solid curves and plots $(c_{21}+c_{12})$ by dashed curves.
The \textbf{Right} panel plots components for a cross-ratio dose not depend on $t_{11}$: 
$(c_{12}+c_{23})$ by solid curves and plots $(c_{13}+c_{22})$ by dashed curves.
All the curves are broadened using the Gaussian kernel density estimation (KDE) method with a bandwidth of 0.05. 
Fig.~\ref{fig:bounded noise} illustrates that curves for $(c_{11} + c_{22})$ and $ (c_{21} + c_{12})$ with a fixed $\epsilon$, i.e. curves in the same color, are in the same shape.
The off-set of curves varies as the noisy level changes. 
Whereas off-set between curves for $c_{12}+c_{23}$ and $(c_{13}+c_{22})$ on the right panel remains a constant for any choice of $\epsilon$.
This is consistent with our theoretical result in Prop.~\ref{prop: bounded_noise} that:
$(c_{11} + c_{22}) - (c_{21} + c_{12}) = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$ depends on $\epsilon$
where as $(c_{12}+c_{23}) - (c_{13}+c_{22}) = - \ln\frac{t_{12} t_{23}}{t_{13}t_{22}}$ is a constant.
%\wt{Dies $t_{12}$ has a prime?}
%The cross-ratio pair including the (1,1)-th element.
% Hence curves for $(c_{11} + c_{22})$ and $ (c_{21} + c_{12})$ with a fixed $\epsilon$, i.e. curves in the same color, should be in the same shape.
% And their off-set varies as the noisy level changes. 
% Whereas curves for $c_{12}+c_{23}$ and $(c_{13}+c_{22})$) should be in the same shape with a fixed off-set.



% so only the difference between cross-ratio pairs of pairs of elements of $C$ which involve the element with noise changes as the value of the noise alters. E.g. the difference between the cross-ratio pair ($c_{11} + c_{22}$) and ($c_{21} + c_{12}$) is controlled by the noise added to $t'_{11}$ while the difference between another pair ($c_{12} + c_{23}$) and ($c_{13} + c_{22}$) is not, see 

% C = [[0.1626, 0.0279, 0.1071],
%       [0.1047, 0.1477, 0.1628],
%       [0.1358, 0.0265, 0.1249]]
% T = [[0.1067, 0.1141, 0.1125],[0.1175, 0.1052, 0.1106],[0.1092, 0.1139, 0.1102]]
% noises = [-0.01, -0.005, 0.0, 0.005, 0.01]

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
    \hspace{-8pt}\includegraphics[width=0.25\textwidth]{figs/random_T_bonded_noise_1.png} &
    \hspace{-18pt}\includegraphics[width=0.25\textwidth]{figs/random_T_bonded_noise_2.png}  
    \end{tabular}
    \caption{Results on infered cost $C$ given a $T$ with bounded noise $\epsilon$ on $t_{11}$.
    $\epsilon$ varies in $[-0.01, -0.005, 0.0, 0.005, 0.01]$, indicated by [\textcolor{blue}{blue}, \textcolor{cyan}{cyan}, \textcolor{black}{black},  
    \textcolor{magenta}{magenta}, \textcolor{red}{red}] in order.
    %The KDE of the distributions of cross-ratio pairs of pair of elements of $C$ with various noise added to $t_{11}$. 
    %The colors represent the noise, \textcolor{blue}{blue}: -0.01, \textcolor{cyan}{cyan}: -0.005, \textcolor{black}{black}: 0.0,  \textcolor{magenta}{magenta}: 0.005, and \textcolor{red}{red}: 0.01.
    \textbf{(Left.)} Solid curves are for ($c_{11}+c_{22}$), and dashed for $(c_{21}+c_{12})$. 
    \textbf{(Right.)} The solid curves are for ($c_{12}+c_{23}$), and dashed for $(c_{13}+c_{22})$.
    }
    \label{fig:bounded noise}
\end{figure}


%\subsection{Gaussian noise on observed plan.}
\textbf{Gaussian noise on observed plan.} We start with a Toeplitz ground truth cost function $C^g$ and obtain a OT plan, $T^g$, with $C^g$ and uniform $\mu, \nu$. A random Gaussian noise $\epsilon \sim \mathcal{N}(0, 0.004^2)$, about 4\% of the average value of $T$, is added to $t^g_{1,2}$, and the corrupted plan $T=T^g+\epsilon$. We then infer the posterior distribution $P(C|T)$. We put a $\mathbf{P}_1$ prior on $C$ with the hyperparameters follows toeplitz matrix format. 
%The prior of $P_0(C)$ is assumed to be toeplitz Dirichlet, where the matrix of the Dirichlet parameters is diagonal-constant and $\sum_{i,j}{C_{i,j}}=1$. 
Inference is done by first generating 10 random numbers $\epsilon_i^{*}\sim \mathcal{N}(0, 0.004^2)$ and apply the noise on $t_{12}$ to get $T_i^{*}=T+\epsilon_i^{*}$. Then, we utilize MHMC on every $T_i^{*}$ to obtain $P(C|T_i^{*}$), and finally $P(C|T)\approx\sum_i P(C|T_i^{*})$. %\wt{Confirm notation with paragraph after remark 3.16.}

For the MHMC method, we burn in 10,000 steps and then take 10,000 samples with lags of 200 steps for each $P(C|T_i^{*})$. For each step, we use the same sampling procedure as described in the bounded noise case but use a Gaussian standard deviation of 0.003. The acceptance rates are around 0.52-0.70.

The posterior distributions of each element of the inferred $C$ are shown in Fig.~\ref{fig:Gaussian noise}. The inferred distributions are close to the ground truth costs which are indicated by blue dashed lines. We demonstrate that our method successfully make accurate inferences using soft constraints, $P_0(C)$, with the results comparable to hard constraints imposed by \citep{stuart2020inverse}. 

% C^g  =[[0.2604, 0.0521, 0.0104],
        % [0.0208, 0.2604, 0.0521],
        % [0.0625, 0.0208, 0.2604]]

% T^g = [[0.0952, 0.1168, 0.1214],
        % [0.1214, 0.0952, 0.1168],
        % [0.1168, 0.1214, 0.0952]]
        
% corruption noise = -0.0011

% noises = [ 0.0004, -0.0008,  0.0029,  0.0002, -0.0056, -0.0005,  0.0006, -0.0023,0.0041,  0.0076]

% d, e, f, g, h = 25., 5., 1.9, 3., 6.
% alpha = torch.tensor([[d, e, f],\
%                       [g, d, e],\
%                       [h, g, d]])


\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_11.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_12.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_13.png} 
    \end{tabular}
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_21.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_22.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_23.png} 
    \end{tabular}
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_31.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_32.png} &
        \hspace{-8pt}\includegraphics[width=0.155\textwidth]{figs/Gaussian_noise_33.png} 
    \end{tabular}

    \caption{The KDE of each element of inferred cost $C$ with Gaussian noise on $t_{12}$. The blue dashed vertical lines indicate the ground truth cost $C^g$.
    }
    \label{fig:Gaussian noise}
\end{figure}

\paragraph{Application on European Migration data.}

%\pw{what plot for real data?}

==> AISTATS_2022/4-conclusion.tex <==
\section{Conclusion}
%In conclusion, we presented an analysis of probabilistic Inverse Optimal Transport which infers latent costs from observed couplings. 
%In contrast with prior work on IOT, we consider the geometric foundations inherited from Sinkhorn scaling of entropy-regularized Optimal Transport. We analyze the support of the cost matrices associated with an observed coupling, the implications of prior distributions on costs, and introduce MCMC algorithms for posterior inference. Our models perform well on synthesis data and the results are comparable to previous works. \wt{Do we need to include a short discussion on the limitations of our model?}
We have generalized prior treatments of IOT by defining and studying the underlying support manifold and associated inference problems. 
We provide general MCMC methods for inference over general priors on discrete costs and induced kernels. 
Simulations illustrate underlying geometric structure and show the feasibility and effectiveness of the inference. 
%\pat{FIXME: one last thing?}

==> AISTATS_2022/customized_command.tex <==
% \usepackage[utf8]{inputenc}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{fullpage}

\usepackage{graphicx}
\usepackage{color,soul}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amstext}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{pictexwd,dcpic}
\usepackage{enumitem}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{empheq,etoolbox}
% Update display of subequation numbering (Xy) > (X.y)
\usepackage{cases}
\usepackage{cleveref} 



\usepackage{tikz}
\usetikzlibrary{calc,intersections,through}
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

%\usepackage{pgfplots}

\newcommand{\pat}[1]{\textcolor[rgb]{.7,0,.2}{#1}}
\newcommand{\pw}[1]{\textcolor[rgb]{0.6,0.6,0}{#1}}
\newcommand{\wt}[1]{\textcolor[rgb]{0,0,0.7}{#1}}
%theorem styles



\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
\def\rep@title{#2 \ref{##1}}%
\begin{rep@theorem}}%
{\end{rep@theorem}}}
\makeatother

\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}

\newreptheorem{lemma}{Lemma}
\newreptheorem{prop}{Proposition}
\newreptheorem{thm}{Theorem}
\newreptheorem{cor}{Corollary}

\newtheorem{exercise}{Exercise}
\newtheorem{question}{Question}


\theoremstyle{definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{problem}[thm]{Problem}
\newtheorem{remark}[thm]{Remark}
\newtheorem{example}[thm]{Example}
\newtheorem*{example*}{Example}
\newtheorem{examples}[thm]{Examples}
\newtheorem{notation}[thm]{Notation}
\newtheorem*{framework*}{Unifying OT Framework}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

% \newtheorem{theorem}{Theorem}[section]
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{note}[theorem]{Note}
% \newtheorem{remark}[theorem]{Remark}



% Notations
\newcommand{\D}{\mathcal{D}} % data space
\newcommand{\hp}{\mathcal{H}} % hypothesis space
\newcommand{\R}{\mathbb{R}} % all real numbers.
\newcommand{\e}{\epsilon} % a small parameter
\newcommand{\E}{\mathbb{E}}%  expectation
\newcommand{\kl}{\text{KL}}%  
\newcommand{\diag}{\text{diag}}%  
\newcommand{\CR}{\text{CR}}%  
\newcommand{\parallelsum}{\mathbin{\!/\mkern-5mu/\!}}

% \usepackage[
% backend=biber,
% style=alphabetic,
% sorting=ynt
% ]{biblatex}


==> AISTATS_2022/supp_algs.tex <==
\section{Additional details of experiments} \label{supsec: alg}


\subsection{Auto-correlation function.}

To monitor the efficiency of our MC methods, we compute the auto-correlation function during the burn-in phase and choose the lags accordingly.

The auto-correlation function is defined as
\begin{equation}
R(t)=\frac{1}{(N-t)\sigma^2}\sum_{l=1}^{N-t}\sum_{i,j}(K_{i,j}^{(l)}-\bar{K}_{i,j})\cdot(K^{(l+t)}_{i,j}-\bar{K}_{i,j}),
\label{eq:autocorrelation}
\end{equation}
where $N$ is the total number of samples generated, (i,j) runs over all indices of the matrices $K$, $\bar{K}$ is the mean averaging over all the samples, and $\sigma_K^2=\sum_{i,j}\sigma_{K,i,j}^2$ is the variance. 

\subsection{Re-normalization of $T$ for MetroMC over prior $\mathbf{P}_1$.}

For using this method, not every random $T$ satisfies the condition such that $C^{(0)}=-\text{ln}(K^{(0)})=-\text{ln}(T)$ lies on the support of the posterior, therefore, we need to re-normalize $T$ so that $C^{(0)}-\text{ln}[T/F(T)]$ is on the support. $F(T)$ is defined as
\begin{equation}\label{eq:renormal_T}
    F(T) = \text{exp}\left({\frac{1+\sum_{i=1}^{m}\sum_{j=1}^{n}\text{log}(T_{i,j})}{m*n}}\right).
\end{equation}

\subsection{MHMC on uniform matrix.}

In this section, we validate our MHMC algorithm by apply it to an uniform $T$, i.e $T_{m,n}=1/m$ 
under prior $\mathbf{P}_2$.
%on uniform matrices, e.g. $T_{m,n}=1/m$ for the column-wise Dirichlet prior case. 
The cross-ratios of $T$ are all 1 and stay the same for all inferred sample $K^{(i)}$. 
Thus, each $K^{(i)}$ has same copies of $n$ columns. 
We compare posterior sampled by MHMC to a 
$m$-dimensional uniform symmetric Dirichlet distribution generated by the SciPy package \citep{2020SciPy-NMeth}.  


% Fig.~\ref{fig:uniform_3x3} shows the results the 3x3 case.
% are the same for every element. We choose $\alpha=1$ for the Dirichlet prior, 
% $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. 
% We run for 10,000 burn-in steps and take 10,000 samples 
% with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. 
% We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps.
% Also, the running averages of the row sums are stable at taking 10,000 samples, 
% which means 10,000 samples can effectively represent the posterior distribution. 

We perform our MHMC algorithm on a $3\times 3$ uniform matrix with prior $P_2$ and the Dirichlet concentration parameter $\alpha$ are the same for every element. We choose $\alpha=1$ for the Dirichlet parameter, $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps. Also, the running averages of the row sums are stable at taking 10,000 samples, which means 10,000 samples can effectively represent the posterior distribution. 

The posterior distribution (Shown in top right of Fig.~\ref{fig:uniform_3x3}.) is compared to the distribution $P(K|T)$ of three-dimensional vectors generated by Dirichlet vector sampler \citep{2020SciPy-NMeth} with symmetric $\alpha=1$ in top left of  Fig.~\ref{fig:uniform_3x3}. The results are comparable, which suggests that our MHMC method is able to generate distributions which well represent the support of the posterior distributions.


\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
        \hspace{-4pt}\includegraphics[width=0.45\textwidth]{figs/dirichlet_3.png}
        \hspace{-6pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3.png}
    \end{tabular}
    \begin{tabular}{c c}
        \hspace{-4pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3_autocorr.png}
        \hspace{-6pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3_running_avg.png}
    \end{tabular}
    
    \caption{\textbf{(Top left.)} The distributions of each component of three-dimensional Dirichlet vectors with symmetric $\alpha=1$ generated using SciPy package. \textbf{(Top right.)} The distributions of each component of the first column of $P(K|T)$ sampled by the MHMC method. \textbf{(Lower left.)} The auto-correlation function of the MHMC simulation. The black dashed lines indicate the range [$-1/e$, $1/e$]. \textbf{(Lower right.)} The running average of the row sums of the MHMC simulation.
    }
    \label{fig:uniform_3x3}
\end{figure}

\subsection{MetroMC on uniform matrix.} We test MetroMC on 3x3 uniform $T$, where $T_{i,j}=1/(m*n)$, and assume the prior $\mathbf{P}_1$ is put on $C$. We take $K^{(0)}=T/F(T)$.
For each MC iteration we sample $m+n-1$ Gaussian random numbers with standard deviations of 0.02 for the diagonal matrices $D^r$ and $D^c$ satisfying the condition 
\begin{equation}
\sum_{i,j}\text{ln}(d^r_{i})+\text{ln}(d^c_j)=0. 
\label{eq:condition_bounded_noises}
\end{equation}
We burn in 10,000 steps and take 100,000 samples with 100 lags in between. The Gaussian Kernel density estimation (KDE) of each component of $P(C|T)$ is demonstrated in Fig.~\ref{fig:uniform_3x3_2}. We use bandwidths of 0.05 for all the Gaussian KDE in this article. There are a few notable features. First, we assume a Dirichlet prior on the whole $C$ matrix, the distributions will be smaller at large values because each large value will suppress the value of the other elements. Second, since we have cross-ratio = 1 everywhere in $T$ and prior $\mathbf{P}_1$ on $C$, there will not be a single element with value close to one. Otherwise, the cross-ratio involving that element could never be 1 anymore. Also, for the same reason all distributions should be similar.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.50\textwidth]{figs/pdf_unifrm_T_3x3.png}
    \begin{tabular}{c c}
        \includegraphics[width=0.45\textwidth]{figs/autocor_uniform_T_P2.png}
        \includegraphics[width=0.45\textwidth]{figs/running_average_uniform_T_P2.png}
    \end{tabular}
    \caption{\textbf{(Top.)} The distribution of each matrix element of $P(C|T)$ with a uniform $T$ and a prior $\mathbf{P}_1$ over $C$ matrix. \textbf{(Bottom left.)} The autocorrelation function of the simulation. \textbf{(Bottom right.)} The running averages of the row sums.}
    \label{fig:uniform_3x3_2}
\end{figure}

\newpage

\subsection{Supporting plots for the MetroMC method on noisy T.}

In this section, we provide data for diagnostics of the MetroMC simulations on the noise models in section 5 of the main text.

\textbf{Bounded noise on observed plan.} The autocorrelation function and the running averages of row sums of the samples for each noise are plotted in Fig.~\ref{fig:MC_details_bounded_noise}. In the simulation we set 100 for the lags by observing that the chains become uncorrelated after $\sim$ 100 steps for all cases. We take 100,000 samples in total for all cases since the running averages are stable at (or before) 100,000 MC steps, which means the samples reaches a stationary distribution.

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.44\textwidth]{figs/autocor_bounded_noise.png}
            \put(-30,125){\textbf{a.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_1.png}
            \put(-30,125){\textbf{b.}}
        \end{picture}

    \end{tabular}
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_2.png}
            \put(-30,125){\textbf{c.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_3.png}
            \put(-30,125){\textbf{d.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_4.png}
            \put(-30,125){\textbf{e.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_5.png}
            \put(-30,125){\textbf{f.}}
        \end{picture}
    \end{tabular}
    \caption{MC diagnostics for the Bounded noise example. \textbf{(a.)} The autocorrelation funciton for all noises. \textbf{(b.)-(f.)} The running averages of row sums of the samples for noises -0.01, -0.005, 0.0, 0.005, and 0.01 added to $t_{11}$, respectively.
    }
    \label{fig:MC_details_bounded_noise}
\end{figure}

\textbf{Gaussian noise on observed plan.}
The autocorrelation function and the running averages of row sums of the samples for the 10 Gaussian noises are plotted in Fig.~\ref{fig:MC_details_running_average_gaussian_noise}. We set 200 for the lags since the chains become uncorrelated after $\sim$ 180 steps for all cases. 10,000 samples are taken for all cases since the running averages of the row sums are stable at 10,000 MC steps.

\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c c c}
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/autocor_gaussian_noise.png}
            \put(-30,80){\textbf{a.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_1.png}
            \put(-30,30){\textbf{b.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_2.png}
            \put(-30,30){\textbf{c.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}   
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_3.png}
            \put(-30,30){\textbf{d.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_4.png}
            \put(-30,30){\textbf{e.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_5.png}
        \put(-30,30){\textbf{f.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}  
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_6.png}
            \put(-30,30){\textbf{g.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_7.png}
            \put(-30,30){\textbf{h.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_8.png} 
            \put(-30,30){\textbf{i.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}  
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_9.png}
        \put(-30,30){\textbf{j.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_10.png}      
            \put(-30,30){\textbf{k.}}
        \end{picture}
    \end{tabular}

    \caption{MC diagnostics for the Bounded noise example. \textbf{(a.)} The autocorrelation funciton for all noises. \textbf{(b.)-(k.)} The running averages of row sums of the samples for the 10 random Gaussian noises added to $t_{12}$.
    }
    \label{fig:MC_details_running_average_gaussian_noise}
\end{figure}

\newpage

\subsection{Matrices.}

We list the matrices used in section 5: \textbf{Simulations on synthetic data} below.

The three $T$ matrices in Fig.~\ref{fig:2x2_subspace} are

\begin{align*}
T_a = 
\begin{bmatrix}
0.3096 & 0.3785 & 0.0544 & 0.2575 \\
0.2522 & 0.3203 & 0.1860 & 0.2415 \\
0.4318 & 0.1433 & 0.4196 & 0.0053 \\
0.0064 & 0.1579 & 0.3400 & 0.4957 \\
\end{bmatrix},
\end{align*}

\begin{align*}
T_b = 
\begin{bmatrix}
0.2532 & 0.4143 & 0.2894 & 0.0431\\
0.1925 & 0.0548 & 0.0958 & 0.6569\\
0.4459 & 0.0905 & 0.3480 & 0.1156\\
0.1083 & 0.4404 & 0.2669 & 0.1844
\end{bmatrix},
\end{align*}

\begin{align*}
T_c = 
\begin{bmatrix}
0.4790 & 0.0994 & 0.0838 & 0.3378\\
0.1343 & 0.1514 & 0.1920 & 0.5224\\
0.1678 & 0.6182 & 0.1963 & 0.0177\\
0.2189 & 0.1310 & 0.5279 & 0.1222
\end{bmatrix}.
\end{align*}

The matrix $T$ in Fig.~\ref{fig:missing_element_T} is
\begin{align*}
T = 
\begin{bmatrix}
0.4583 & 0.2297 & 0.2633\\
0.4631 & 0.4785 & 0.2755\\
0.0785 & 0.2919 & 0.4611
\end{bmatrix}.
\end{align*}


The matrices $T$ in Fig.~\ref{fig:sample_supp} are

\begin{align*}
T_1 = 
\begin{bmatrix}
0.1104 & 0.0684 & 0.1545 \\
0.0505 & 0.2401 & 0.0428 \\
0.1725 & 0.0249 & 0.1360
\end{bmatrix},
\end{align*}

\begin{align*}
T_2 = 
\begin{bmatrix}
0.0950 & 0.1100 & 0.1283\\
0.1155 & 0.0343 & 0.1835\\
0.1228 & 0.1890 & 0.0215
\end{bmatrix},
\end{align*}

\begin{align*}
T_3 =
\begin{bmatrix}
0.1053 & 0.1193 & 0.1088\\
0.2148 & 0.0090 & 0.1096\\
0.0133 & 0.2051 & 0.1150
\end{bmatrix}.
\end{align*}

The matrix $T$ for the bounded noise case is

\begin{align*}
T =
\begin{bmatrix}
0.1067 & 0.1141 & 0.1125\\
0.1175 & 0.1052 & 0.1106\\
0.1092 & 0.1139 & 0.1102
\end{bmatrix}.
\end{align*}

The ground truth $C^g$ in the Gaussian noise example is
\begin{align*}
C^g = 
\begin{bmatrix}
0.2604 & 0.0521 & 0.0104\\
0.0208 & 0.2604 & 0.0521\\
0.0625 & 0.0208 & 0.2604
\end{bmatrix},
\end{align*}
and the hyperparameter matrix for the prior is
\begin{align*}
\alpha =
\begin{bmatrix}
25.0  & 5.0     & 1.9\\
3.0   & 25.0    & 5.0\\
6.0   & 3.0     & 25.0
\end{bmatrix}.
\end{align*}

==> AISTATS_2022/supp_proofs.tex <==
\section{Proofs and Definitions for Section~\ref{sec:piot}}
\begin{repprop}{prop:piot}
When $T = T^*$, $ P(C|T)$ is supported on the intersection between $\Phi^{-1} (T)$ and the domain of $ P_0(C)$, moreover, we have that
$\displaystyle P(C|T) = \frac{P_0(C)}{\int_{\Phi^{-1} (T)} P_0(C) \text{d} C}$.
\end{repprop}

\begin{proof}
When $T = T^*$, Eq~\eqref{eq: PIOT} and Eq~\eqref{eq: bayes} imply that:
$P(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$. $P(T) >0$ is the normalizing constant, 
so $\text{Supp}[P(C|T)] = \text{Supp}[P(T|C)] \cap \text{Domain}[P_0(C)] $.
Note that $P(T|C) P_0(C) = P_0(C)$ for $C \in \Phi^{-1}(T)$, otherwise $P(T|C) P_0(C) =0$.
Hence the proposition holds.
\end{proof}




\begin{repprop}{prop:DAD}
Let $T$ be a non-negative optimal coupling of dimension $m\times n$. $C \in \Phi^{-1} (T)$ if and only if for every $\epsilon > 0$,
there exist two positive diagonal matrices $D^r = \diag\{d^r_1, \dots, d^r_m\}$ and $D^c =\diag \{d^c_1,\dots, d^c_n\}$ such that: 
$\displaystyle |D^r K D^c - T| < \epsilon$, where $K = e^{-C}$ and $|\cdot|$ is the $L^1$ norm. 
In particular, if $T$ is a positive matrix, then $C \in \Phi^{-1} (T)$ 
if and only if there exist positive diagonal matrices $D^r,D^c$ such that $D^r K D^c = T$, i.e.
\begin{equation*}
\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}    
\end{equation*}
\end{repprop}

\begin{proof}
Let the row and column of marginals of $T$ be $\mu$ and $\nu$.
Then $C \in \Phi^{-1} (T)$ if and only if $(\mu, \nu)$-Sinkhorn scaling of $K$ converges to $T$ in $L^1$ norm 
(for finite matrices, convergence in all $L^k$ norms are equivalent).
Notice that a row (column) normalization step in the Sinkhorn scaling is equivalent to a left(right) matrix multiplication of a positive diagonal matrix. 
Indeed, let $K_0 = {K}$, $\mathbf{r}_0 = K_0 \mathbf{I}_n$ (vector for row sums of $K_0$), $D_0^{r} = \diag(\mu /\mathbf{r}_0)$.
Here $\mu /\mathbf{r}_0$ represents element-wise division. 
Let $K'_0$ be the matrix obtained by row normalization of $K_0$ with respect to $\mu$. Then $K'_0 = D_0^{r} K_0$.
Similarly, let $K_1$ be the matrix obtained by column normalization of $K'_0$ with respect to $\nu$.
Then $K_1 = K'_0 D_0^c$, where $D_0^c = \diag (\nu/ \mathbf{I}_m^T K'_0)$.
Iteratively, we have $K_s = \Pi_{i=1}^{s} D_i^r \cdot K_0 \cdot \Pi_{i=1}^{s} D_i^c$.

The \textbf{only if direction} [${C} \in \Phi^{-1} (T) \Longrightarrow$ existence of $D^r$ and $D^c$ for any $\epsilon$]: 
${C} \in \Phi^{-1} (T) \Longrightarrow $ $(\mu, \nu)$-Sinkhorn scaling of ${K}$ converges to $T$
$\Longrightarrow $, for any $\epsilon >0$, there exists $N>0$ such that for any $s>N$, $|K_s - T| < \epsilon$, 
where $K_s = \Pi_{i=1}^{s} D_i^r \cdot {K} \cdot \Pi_{i=1}^{s} D_i^c$.
Let $D^r = \Pi_{i=1}^{s} D_i^r$, $D^c = \Pi_{i=1}^{s} D_i^c$, the only if direction is complete.

The \textbf{if direction} [existence of $D^r$ and $D^c$ for any $\epsilon$ $\Longrightarrow$ ${C} \in \Phi^{-1} (T)$]: 
Let the limit of $(\mu, \nu)$-Sinkhorn scaling on ${K}$ be $K^{*}$.
Hence $K^{*}$ and $T$ have the same marginals and pattern. 
According to Lemma~A.3 of \citep{pei2019generalizing}, $K^{*}$ and $T$ are diagonally equivalent. 
Further by Proposition~1 of \citep{pretzel1980convergence} $K^{*} = T$.


In particular, when $T$ is a positive matrix, ${K}$ must also be a positive matrix.
Then $T$ and ${K}$ have the same pattern. 
$T = \lim_{s\to \infty} \Pi_{i=1}^{s} D_i^r \cdot {K} \cdot \Pi_{i=1}^{s} D_i^c$
implies that $\lim_{s\to \infty} \Pi_{i=1}^{s} D_i^r$ and $\lim_{s\to \infty} \Pi_{i=1}^{s} D_i^c$ exist. 
Hence the claim. \citep{rothblum1989scalings, idel2016review}

\end{proof}



\begin{replemma}{lemma:cr_dr}
For two positive matrices $A, B$, 
$A \overset{c.r.}{\sim}B$ if and only if 
there exist positive diagonal matrices $D^r$ and $D^c$ such that $A = D^r B D^c$.
\end{replemma}
\begin{proof}
The \textbf{if direction}:
$A = D^r B D^c$  $\Longrightarrow$ 
$\displaystyle \frac{a_{ik}a_{jl}}{a_{il}a_{jk}} = \frac{d^r_ib_{ik}d^{c}_{k} \cdot d^{r}_{j}b_{jl}d^{c}_l}{d^{r}_ib_{il}d^{c}_{l} \cdot d^{r}_jb_{jk}d^{c}_k} 
=  \frac{b_{ik}b_{jl}}{b_{il}b_{jk}}$  $\Longrightarrow$  $A \overset{c.r.}{\sim}B$.

The \textbf{only if direction}: Let the dimension of $A, B$ be $m\times n$, we will prove by induction on $m+n$. 
\textit{Step1.} Assume the dimension of $A, B$ is $2\times 2$.
Let the marginal of $A$ be $\mu_A$ and $\nu_A$, and  $B^* = \Phi (B, \mu_A, \nu_A)$. Then $A$ and $B^*$ 
have the same marginals and cross ratios, which put four same independent constraints on elements of $A$ and $B$,
hence $A =  B^* = D^r B D^c$  for some $D^r, D^c$.
\textit{step2.} Assume the statement holds for $m+n< N$. 

\newpage
Now assume that $m+n = N$. 
Denote the submatrices of $A$ and $B$ consisted by their first $n-1$ by $A_{1}$ and $B_{1}$.
$A\overset{c.r.}{\sim} B \Longrightarrow A_{1}\overset{c.r.}{\sim} B_{1}$. By the inductive assumption, there exist
diagonal matrices $D^r_1$ and $D^{c}_1$ such that $A_{1} = D^r_1 B_1 D^c_1$. 
Further $\frac{a_{11}a_{1n}}{a_{i1}}a_{in} = \frac{b_{11}b_{1n}}{b_{i1}}b_{in}$ holds for any $i\in \{1,\dots, m\}$ imply that
there exists an $d>0$ such that $\mathbf{a}_{n} = d \cdot \mathbf{b}_{n}$. Let $D^r = D^r_1$, $D^{c} = \diag{D^c_1, d}$, 
we have $A = D^rB D^c$ holds. Hence the only if direction is completed.
\end{proof}


\begin{repthm}{thm:IOT}
Let $T$ be an observed positive optimal coupling of dimension $m\times n$. 
Then $\Phi^{-1} (T)$ is a hyperplane of dimension 
$m+n-1$ embedded in $ (\mathbb{R}^*)^{m\times n}$, which consists all the cost matrices 
that of the form:
\begin{equation}\label{supeq:cr_equiv}
 \Phi^{-1} (T) = \{C \in (\mathbb{R}^*)^{m\times n} | K= e^{-C} \overset{c.r.}{\sim} T\}.    
\end{equation}
\end{repthm}

\begin{proof}
Combining Proposition~\ref{prop:DAD} and Lemma~\ref{lemma:cr_dr}, we have Eq.~\eqref{supeq:cr_equiv} holds.
Hence $\Phi^{-1} (T)$ contains all the matrices $C$ satisfying the following set of equations:
$\frac{k_{ik} k_{jl}}{k_{il} k_{jk}} = \frac{t_{ik} t_{jl}}{t_{il} t_{jk}} $ 
for any $i, j \in \{1, \dots, m\}$ and $k, l \in \{1, \dots, n\}$, where $K = e^{-C}$, i.e. $k_{ik} = e^{-c_{ik}}$.
Thus $\Phi^{-1} (T)$ is the solution set of the system of linear equations:
\begin{equation} \label{supeq:linear_sys}
    c_{il}+c_{jk} - c_{ik}-c_{jl} = \ln (t_{ik} t_{jl}) - \ln (t_{il} t_{jk})
\end{equation}
Further Remark~\ref{rmk:basis} shows that there are only $(m-1)(n-1)$ independent equations in the system \eqref{supeq:linear_sys}.
Hence $\Phi^{-1} (T)$ is a hyperplane of dimension $mn - (m-1)(n-1) = m+n-1$.
\end{proof}




\begin{repcor}{cor:proj_single_column}
Under prior $\mathbf{P_2}$,
the projection of $\text{supp}[P(K|T)]$ onto each column is a $(m-1)$-dimensional manifold that is homeomorphic to the simplex $\Delta_{m-1}$. 
\end{repcor}

\begin{proof}
According to prior $\mathbf{P_2}$, for any $K \in \text{supp}[P(K|T)]$, each column of $K$ sums to $1$. 
Hence the projection of $\text{supp}[P(K|T)]$ onto any $j$-th column is embedded in the simplex $\Delta_{m-1}$. 
To show `homeomorphic ', 
we only need to show that for each $v \in \Delta_{m-1}$, there exists a $K \in \text{supp}[P(K|T)$ such that $\mathbf{k}_{j} =v$.
As discussed in Remark~\ref{rmk: one_free_column}, let $D'^{r} = \diag(v/\mathbf{t}_{j})$, 
$K' = \text{Col}( D'^{r}T)$. It's easy to check that $K'\in \text{supp}[P(K|T)]$, and $\mathbf{k'}_{j} = v$.
Hence the corollary holds.
\end{proof}
% \textit{Cross ratio equivalent} is defined in \citep{pei2019generalizing} as following:
% \begin{definition}
% Let $A = (a_{ij})_{n\times n}$ be a square matrix and $S_n$ be the set of all permutations of length~$n$.
% For any $\sigma \in S_n$, the set of $n$-elements $\{a_{1,\sigma(1)}, a_{2,\sigma(2)}, \dots,a_{t,\sigma(n)}\}$
% is called a \textbf{diagonal} of $A$.
% If every $a_{k, \sigma(k)} > 0$, then the diagonal is said to be \textbf{positive}.
% \end{definition}


% \begin{definition}\label{def:cross ratios}
% Let $A, B$ be two $n\times n$ matrices and $D^A_1=\{a_{1,\sigma(1)},\dots, a_{n, \sigma(n)}\}$ and $D^A_2=\{a_{1,\sigma'(1)},\dots, a_{n, \sigma'(n)}\}$ be two positive diagonals of $A$ determined by permutations $\sigma, \sigma'\in S_n$. 
% Denote the products of elements on $D^A_1$ and $D^A_2$ by $d^A_1=\Pi_{i=1}^{n}a_{i, \sigma(i)}, d^A_2=\Pi_{i=1}^{n}a_{i, \sigma'(i)}$ respectively. Then $\CR(D^A_1, D^A_2)=d^A_1/d^A_2$ is called the \textbf{cross ratio} between $D^A_1$ and $D^A_2$ of $A$. Further, let the diagonals in $B$ determined by the same $\sigma$ and $\sigma'$ be 
% $D^B_1=\{b_{1,\sigma(1)},\dots, b_{n, \sigma(n)}\}$ and $D^B_2=\{b_{1,\sigma'(1)},\dots, b_{n, \sigma'(n)}\}$. We say $A$ is \textbf{cross ratio equivalent} to $B$, denoted by $A\overset{cr}{\sim} B$, if $d_i^A\neq 0 \Longleftrightarrow d_i^B\neq 0$
% and $\CR(D^A_1, D^A_2)=\CR(D^B_1, D^B_2)$ holds for 
% any $D^A_1$ and $D^A_2$.
% \end{definition}

\begin{repprop}{prop:submanifold}
$C_s \in \text{supp}[P(C_s|T)]$ if and only if there exists positive diagonal matrices $D_s^c, D_s^r$ such that $K_s = D_s^c T_s D_s^r$ and
the system of equations shown below have a set positive solution for $\{x_1, \dots, x_{m-s_1}\}$.
\begin{equation}\label{supeq: submainfold}
  (x_1, \dots, x_{m-s_1}) T_{m-s}  = (1/d^c_1, \dots, 1/d^c_{s_2}) - \mathbf{1}_s D_s^rT_s  
\end{equation}

\end{repprop}

\begin{proof}
The \textbf{if direction}: Let $(x_1, \dots, x_{m-s_1})$ be a positive solution of Eq.~\eqref{supeq: submainfold}, 
let $D'^{r} = \diag (D^{r}_s, x_1, \dots, x_{m-s_1})$ be an extension of $D^r_s$.
Denote the column sum of $D'^{r} T$ by $\nu'$. Then Eq.~\eqref{supeq: submainfold} implies that $\nu'_i = d^c_i$ for 
$i \in \{1, \dots, s_2\}$. Let $D'^c = \diag(D^c_s, \nu'_{s_2+1}, \dots,\nu'_{n})$. 
It is clear that $K' = D'^r T D'^c \in \text{supp}[P(K|T)]$, and $K_s$ is $K'$'s submatrix corresponding to $X_s\times Y_s$.

The \textbf{only if direction}: for $C_s \in \text{supp}[P(C_s|T)]$, let $K_s = e^{-C_s}$ be the submatrix of $K'\in text{supp}[P(K|T)$.
Then there exists $D'^r, D'^c$ such that $K' = D'^r T D'^c $. Let the corresponding submatrices of $D'^r, D'^c$ be $D^r_s, D^c_s$. 
We have $K_s = D_s^c T_s D_s^r$ hold. Further it is easy to verify that $(d'^r_{s_1+1}, \dots d'^r_{n})$ is a positive solution for 
Eq.~\eqref{supeq: submainfold}. Hence the proof is completed.
\end{proof}


\begin{repcor}{cor:missing_element}
Under prior $\mathbf{P_2}$, 
$\mathcal{K}_1$ is a line segment in $\Delta_{m-1}$ that can be parameterized as:
$\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} \in (0,\infty) \}$.
\end{repcor}

\begin{proof}
Corollary~\ref{cor:proj_single_column} implies that $\mathcal{K}_1 \subset \Delta_{m-1}$. 
Further Remark~\ref{rmk: one_free_column} implies that for each choice of $t_{m1} >1$, 
a known $\mathbf{k}_l$ uniquely determines a point in form of $(d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}$ 
in $\mathcal{K}_1$. Hence the corollary holds.
\end{proof}


\begin{repcor}{cor:parallel}
Let $T_1, T_2$ be two positive matrices of dimension $m \times n$.
The hyperplanes $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
In particular, if $T_1 \overset{c.r.}{\sim}T_2$ then $\Phi^{-1}(T_1) = \Phi^{-1}(T_2)$.
Otherwise $\Phi^{-1}(T_1)$ is parallel to $\Phi^{-1}(T_2) $.
\end{repcor}

\begin{proof}
According to the proof of Theorem~\ref{thm:IOT} above, 
both $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$ are defined by system of equations in form of
Eq.~\eqref{supeq:linear_sys}. In particular, they have the same coefficients, 
only the constants on the right side of the equations are different.
Hence, $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
\end{proof}


\begin{repprop} {prop: bounded_noise}
For a coupling $T$,  assume uniform observation noise on $t_{11}$ with bounded size $a$, 
\begin{equation}\label{supeq: bounded_noise}
 \text{supp}[P(C|T)] = \cup_{T'\in \mathbb{B}_{a}(T)} \Phi^{-1}(T'),   
\end{equation}

where $\mathbb{B}_{a}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t'_{11}>0$, $|t'_{11} - t_{11}| \leq a$ and $t'_{ij} = t_{ij}$ for other $i, j$.
Moreover, $\Phi^{-1}(T')$ can be expressed as intersection of two hyperplanes (may be in different dimensions):
one with equation: $c_{11} + c_{22} - c_{21} - c_{12} = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$, 
and the other equation does not depend on the value of $t'_{11}$. Assume the angle between these two hyperplanes is $\theta$.
Then $d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \ln \frac{t_{11} + a}{t_{11} - a} /\sin \theta $ for $T_1', T_2' \in \mathbb{B}_{a}(T)$.
\end{repprop}

\begin{proof}
With bounded noise on $t_{11}$, the domain for $t^*_{11}$ is $[t_{11}-a, t_{11}+a] \cap \{t^*_{11} > 0\}$.
Hence Eq.~\eqref{supeq: bounded_noise} holds. $\Phi^{-1}(T')$ is defined by the cross ratios of $T$ as shown in 
Eq.~\ref{supeq:linear_sys}. Using cross-ratio basis say $\mathcal{B} =\{r_{mjnk}(T')| j = 1, \dots, m-1, k=1,\dots, n-1 \}$, Eq.~\ref{supeq:linear_sys} 
can be simplified into a system with only independent $(m-1)(n-1)$, where only the equation defined by $r_{m1n1}(T')$ involves $t'_{11}$,
the other equations can be combined into one equation by substitutions.
Each of these two equations determines a hyperplane,
hence $\Phi^{-1}(T')$ can be expressed as the intersection of two hyperplanes.
Moreover, let the defining hyperplanes for $T^1, T^2 \in \mathbf{B}_a(T)$ be $\{H^1_1, H^1_2\}$ and  $\{H^2_1, H^2_2\}$ respectively,
where $H^i_1$ is the one defined by $ c_{11}+c_{mn} - c_{m1}-c_{1n} = \ln (t_{m1} t_{1n}) - \ln (t^i_{11} t_{mn})$, where $i =1,2$.
Then the Euclidean distance between $H^1_1, H^1_1$ is $d(H^1_1, H^1_1) = |\ln t^1_{1,1} - \ln t^2_{1,1}| \leq |\ln (t_11 +a) - \ln (t_11 -a)|$.
Notice that $H^1_2 = H^2_2$. So the distance between $\Phi^{-1}(T^1), \Phi^{-1}(T^2)$ is bounded by $(\ln (t_{11} +a) - \ln (t_{11} -a))/\sin\theta$.
\end{proof}


\begin{repprop}{prop: gaussian_noise}
Let $T$ be an observed coupling of dimension $m\times n$ with Gaussian noise on $t_{11}$.
Further, let $\mathcal{B}$ be a basis for cross ratios of $m\times n$ matrices, that contains only one cross ratio depending on $t_{11}$.
Eliminate the cross ratio depending on $t_{11}$ in $\mathcal{B}$, denote the new set by $ \mathcal{B}^{-}$. Then: 

\centerline{$\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$}
In particular, $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T')$ 
for any $T'\in \mathbb{L}(T)$.
\end{repprop}

\begin{proof}
Since the domain for $\epsilon \sim \mathcal{N}(0,\sigma^2)$ is $(-\infty, \infty)$, 
hence the domain for possible $t^*_{11}$ is $(0, \infty)$. 
Thus the observation $T$ essentially put no constraint on the cross ratio of $T^*$ depends on $t^*_{11}$.
Hence $\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$. 
As only one equation was eliminated, so $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T')$ 
for any $T'\in \mathbb{L}(T)$.
\end{proof}

==> ICML-sumission/1-intro_ICML.tex <==
\section{Introduction}

%A common goal in machine learning is to infer, given some observations, estimate the model(s) that may have generated the observations. 
%Suppose, however, that the observed data are not the outcome of a single model, but a collection of models and the observed data they produce are an efficient assignment of models to instances. Such situations commonly occur among collections of individuals, where the possible outcomes are a constrained set, all of which must be covered. See
%In such situations, we may also wish to draw inferences about the underlying models, but in order to do so we must account for the interactions among individuals arising from the coupling process. This class of problems is naturally formalized via Inverse Optimal Transport (IOT). 

%\pat{set up the paper against prior work. assume squared noise on plan. do not understand underlying geometric structure}
%
%\pat{our contributions: 
%(1) describe geometry of underlying manifold 
%(2) Geometry provides insight into missing value problems
%(3) Algorithm for inference based on geometry (current algorithm, show it works for randomly generated matrix)
%(4) standardly assumed noise model iteracts with support (claim: high CR means more concentrated posterior, due to "fewer" manifolds in the same gaussian ball.)
%(5) improved inference for standard noise model based on cross ratios??? 
%-- Clever way for thinking about which manifolds are nearby, avoids computing sinkhorn over and over
%(6) Geometry provides insight into behavior of different possible noise models (multiple agents, noise on perceived costs)
%}

%A common goal in machine learning is to infer, given some observations, estimate the costs that underlie the observations. 
%Given a coupling of two discrete probability distributions, can we infer the underlying costs that explain the observed joint density? Such couplings appear commonly when one set is matched with a second set. Examples include inferring the underlying distances given transportation patterns, affinity between matched pairs \cite{}, and  \pat{FIXME}. The forward problem of computing stochastic couplings is typically formulated as Entropy regularized optimal transport. Here we investigate the problem of inferring underlying costs via Inverse entropy regularized Optimal Transport.  

Inverse Optimal Transport (IOT)  involves inferring latent costs from stochastic couplings, a problem that arises across many domains where matching or movement of distributions arises \citep{stuart2020inverse,li2019learning,paty2020regularized}. 
%has received less systematic attention than (entropy-regularized) Optimal Transport (OT) \citep{villani2008optimal,cuturi2013sinkhorn}. 
%Although researchers have studied IOT in migration \citep{stuart2020inverse} and matching problems \citep{li2019learning}, and through adversarial robustness \citep{paty2020regularized} formulation and investigation of the general problem of probabilistic inference of latent costs from stochastic couplings given priors has not been systematically undertaken. 
%Formulation and investigation of the general problem of probabilistic inference of latent costs from stochastic couplings given priors has not been systematically undertaken.
Unlike (Entropy-regualrized) Optimal Transport \citep{villani2008optimal,cuturi2013sinkhorn}, mathematical foundations and computational implications have not been systematically investigated. 
IOT inherits interesting geometric structure from Sinkhorn scaling \citep{sinkhorn1964relationship}, which gives rise to natural questions about the nature of posterior distributions, the existence of samplers, and questions about the feasibility of inferences from observed couplings to underlying costs. 

IOT problems has been applied in many areas. Practical examples include: (1) inferring the cost criterion of international migration (Stuart and Wolfram, 2020); (2) estimating the marriage matching affinity (Dupuy \textit{et al.}, 2019); (3) learning interaction cost function from noisy and incomplete matching matrix and make prediction on new matching (Li \textit{et al.}, 2019). These works provide methodologies to solve \textit{specific} IOT problems with extra hard constraints on latent costs. In this paper we provide a framework to analyze the \textit{general} probabilistic inverse optimal transport (PIOT) problem, and to understand the geometric properties of the space of latent costs.
%while in this paper we provide a framework for analyzing the general problem to understand the geometric properties of probabilistic inverse optimal transport (PIOT).

Our contributions include: (1) formulating the PIOT problem and identify the support manifold for latent costs; 
(2) characterizing the geometry of the support manifold along with the implications of prior distributions on posterior inference; 
(3) analyzing the support manifold for noisy and incomplete observations.
(4) developing MCMC algorithms for posterior inference which derives directly from geometric properties
of Sinkhorn scaling; 
(5) demonstrating PIOT through simulations on general examples 
including visualizations of latent cost manifold and  missing/noisy value predictions for migration data. 
%\pw{need some help on item (5).}
%We investigate properties of PIOT with several contributions. We formalize the general problem and proving basic results; characterize the manifold of support of the posterior distribution along with the implications of prior distributions on posterior inference; and present MCMC algorithms for posterior inference which derives directly from properties of Sinkhorn scaling, and show by simulation that samplers are effective on synthetic problems.  
%Our third contribution is to explore the feasibility of inference in this model by simulation and by demonstration on a real-world performance of NBA basketball teams. We conclude by discussing implications of the approach and interesting directions for extending the work. 

\textbf{Notation:} $\mathbb{R}^+$ denotes positive reals, $\mathbb{R}^*$ denotes non-negative reals.
$\overline{\mathbb{R}^*}$ denotes the extended non-negative reals $ \mathbb{R}^* \cup \{+\infty\}$. 
$\Delta_k$ is the $k$-dimensional simplex.
For a space $X$, $\mathcal{P}(X)$ denotes the set of distributions over $X$. 
%All matrices are assumed to be non-negative, and have no zero rows or zero columns unless otherwise stated. 
Matrices are in uppercase and their elements are in the corresponding lowercase.
For a matrix $A_{m\times n}$, $\mathbf{a}_1, \dots,\mathbf{a}_{n}$ denotes columns of $A$. %$\text{Col}(M)$ denotes column normalization of $M$.
Column normalizing a matrix $A_{m\times n}$
with respect to a $n$-dim row vector $\nu$ is defined as 
$\text{Col}(A, \nu) = A \text{diag} (\frac{\nu}{\mathbf{1}_{m} A})$, 
where $\mathbf{1}_{m}$ is a $m$-dim row vector with each element equals to~$1$. 
`with respect to $\nu$' is omitted when $\nu = \mathbf{1}_{n}$. 
Row normalization is defined in the same fashion.

==> ICML-sumission/2-theory_ICML.tex <==


\section{Background and Related Work}
%Consider the situation where data from a collection of models were observed and the inference needs to be made on the underlying interactions between those models.
%In this section we formalize such inference as probabilistic inverse optimal transport. 
%\pw{discuss, notations, name for H,  T and C, $t_{ij}, c_{ij}$}
%\pat{pull out all details about column normalization to make it fully general to dirichlet prior on cost}

Given two spaces $X = \{x_1, \dots, x_m\}$ and $Y = \{y_1, \dots, y_n\}$, 
let $T = (t_{ij})_{m\times n} \in (\mathbb{R}^*)^{m\times n}$ 
be a \textit{coupling} that records the co-occurrence distribution between $X$ and $Y$.
Note that $t_{ij}$ is allowed to be zero here.
%Each column of $P$ is indexed by an $h$ and each row of $P$ is indexed by a $d$.
Each element $t_{ij}$ represents the probability of observing $x_i$ and $y_j$ simultaneously. 
The interaction between $X$ and $Y$ can be captured by a \textit{cost matrix} 
$C = (c_{ij})_{m\times n} \in (\overline{\mathbb{R}^*})^{m\times n}$, 
where $c_{ij}$ measures the underlying cost of coupling $x_i$ and $y_j$. 
Hence, the probabilistic inference on the underlying structure over $X$ and $Y$ is then to obtain $P(C|T)$, 
the distribution over all possible $C$ given an observed coupling $T$.

%The total cost of a plan $T$ is defined to be $\langle C, T\rangle = \sum_{i\in \D, j\in \hp} c_{ij}t_{ij}$, the Frobenius inner product.
%Let the prior of $C$ be $P_0(C)$, a distribution over $(\mathbb{R}^*)^{m\times n}$. %($\mathbb{R}^*$ is the set of non-negative real numbers). 
%Then the inference on $C$ 
%can be concluded using Bayes Rule: $P_t(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$.

% \pw{How do we justify the assumption that $T$ is optimal, by assuming the underlying model is cooperative?}
% \pw{directly go for EOT or OT}

%Assuming the $T$ is obtained by minimizing the total cost, we may 
\textbf{Entropy regularized optimal transport} is an fundamental building block in modelling $P(C|T)$. 
Given a cost matrix $C$ and distributions $\mu,\nu$ over $X$ and $Y$ respectively, 
\textit{Entropy regularized optimal transport} (EOT) \citep{cuturi2013sinkhorn,peyre2019computational} solves the optimal coupling $T^{\lambda}$ that 
minimizes the entropy regularized cost of transfer $X$ with distribution $\mu$ into $Y$ with distribution $\nu$. 
Thus for a parameter $\lambda >0$: 
\begin{equation}\label{eq:eot}
T^{\lambda} = \text{argmin}_{T\in U(\mu, \nu)} \{\langle C, T\rangle - \frac{1}{\lambda} H(T)\},
\end{equation}
\noindent where $U(\mu, \nu)$ is the set of all couplings between 
between $\mu$ and $\nu$ (i.e. joint distributions with marginals $\mu$ and $\nu$), $\langle C, T\rangle = \sum_{i\in X, j\in Y} c_{ij}t_{ij}$ is 
the Frobenius inner product between $C$ and $T$, and $H(T) := - \sum_{i=1}^{m}\sum_{j=1}^{n} t_{ij} \log t_{ij}$ 
is the \textit{entropy} of $T$. $T^{\lambda}$ is called an \textit{optimal coupling} with parameter $\lambda$. 

\textbf{Sinkhorn scaling} is used to efficiently compute optimal couplings.
$(\mu,\nu)$-\textit{Sinkhorn Scaling (SK)} \citep{sinkhorn1964relationship} of a matrix M 
is the iterated alternation between row normalization of $M$ with respect to $\mu$ and 
column normalization of $M$ with respect to $\nu$. \citep{cuturi2013sinkhorn} proved that: 
given a cost matrix $C$, the optimal coupling $T^{\lambda}$ between $\mu$ and $\nu$ 
can be solved by applying $(\mu, \nu)$-Sinkhorn scaling on 
the \textit{negative exponential cost matrix} $K^{\lambda}$,
where $K^{\lambda} = e^{-\lambda C} = (e^{-\lambda\cdot c_{ij}})_{m\times n}$ (See Example~\ref{eg: sk}).
% \pw{include an example of Sinkhorn?}
% \pat{yeah. i think this will help when we need to define the inverse.}

% \begin{example}\label{eg: sk}
% Let $\mu =\nu=(\frac{3}{8},\frac{5}{8})$, 
% $\tiny C = \begin{pmatrix} \ln 1 & \ln 2 \\
%  \ln 4 & \ln 1 \end{pmatrix}$. 
% For $\lambda=1$, we may obtain $T$ by applying SK scaling on
% $\tiny K^{\lambda} = e^{-C} = \begin{pmatrix} 1 & 1/2\\ 1/4 & 1 \end{pmatrix}$:
% first, row normalize $K^{\lambda} $ with respect to $\mu$ results:
% $\tiny K_1^{\lambda} =  \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
% Then column normalization of $ K_1^{\lambda}$ with respect to $\nu$ outputs 
% $\tiny K_2^{\lambda} = \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
% As $K_1^{\lambda}= K_2^{\lambda}$, the SK scaling has converged with $T = K_1^{\lambda}$.
% In general, multiple iterations may be required to reach the limit. \pw{may move to apdx}
% \end{example} 

Given a coupling $T$, the inference on the cost matrix $C$
can be formulated as an inverse entropy regularized optimal transport problem. 
%can be interpreted as map from an optimal coupling $T^{\lambda}$ to the set of all possible triples of cost and marginals $\{(\widehat{C}, \widehat{\mu},\widehat{\nu})\}$. 
Given $\lambda$, EOT is the map $\Phi$:$(\overline{\mathbb{R}^*})^{m\times n} \times \mathcal{P} (\mathbb{R}^{m}) \times 
\mathcal{P} (\mathbb{R}^{n}) \to \mathcal{P} ((\mathbb{R}^*)^{m\times n})$ with $\Phi(C, \mu, \nu) = T^{\lambda}$.
Therefore \textbf{inverse entropy regularized optimal transport (IOT)} can be defined as $\Phi^{-1}: T^{\lambda} \to \{(C, \mu,\nu)\}$,
where $\{(C, \mu,\nu)\}$ represents the preimage set of $T^{\lambda}$ under $\Phi$.


\begin{remark}
In IOT, when $T^{\lambda}$ is observed without any noise,
$T^{\lambda}$ completely determines $\mu$ and $\nu$. 
Indeed $(C, \mu,\nu) \in \Phi^{-1}(T^{\lambda})$ implies that
$T^{\lambda} \in U(\mu,\nu)$. Thus $\mu$ and $\nu$ must equal the row and column marginals of $T^{\lambda}$.
Hence we may reduce IOT into $\Phi^{-1}: T^{\lambda} \to \{C\}$. 

Further, note that $\Phi^{-1}: T^{\lambda} \to \{C\}$ 
is not well-defined as a function, 
since $T^{\lambda}$ does not uniquely determine cost $C$. 
For instance, 
any two cost matrices differ by an additive constant 
output the same optimal coupling.
% For instance, any matrix $C'$ in form of 
% $\tiny C' = \begin{pmatrix} \ln \alpha \cdot 1 & \ln \alpha \cdot 2 \\
%  \ln \beta \cdot 4 & \ln \beta \cdot 1 \end{pmatrix}$, for $\alpha, \beta>0$
% outputs the same optimal coupling $T$ as $C$ in Example~\ref{eg: sk} \pw{need to modify if example is moved.}
%\pat{insert example here too? build off the SK one}
\end{remark}

%\pw{we probably may move the next two paragraphs into intro.}

\textbf{Related Work.} 
The forward OT problem has a long history and is an active field of research 
\citep{kantorovich1942translocation, villani2008optimal,peyre2019computational,genvay2016stochastic}.
Applications in machine learning include: 
supervised learning \citep{frogner2015learning}, Bayesian inference \citep{el2012bayesian}, generative models \citep{salimans2018improving},
Transfer learning \citep{courty2016optimal}, and NLP \citep{alaux2018unsupervised}. 

However, the inverse OT problem is much less studied. The few existing inverse OT papers \citep{dupuy2019estimating, li2019learning, stuart2020inverse}, 
to our best knowledge, all 
focused on obtaining a unique approximation of the `ground truth' $C^*$, even though $\Phi^{-1}(T)$ contains a set of cost matrices.
To output an estimate of $C^*$, existing approaches place constraints on the cost matrix. 
For example in \citet{stuart2020inverse}, $C$ has to be either a Toeplitz matrix or
determined by a given graph structure.
In \citet{li2019learning}, $C$ must be constructed from a metric over a space where both $X$ and $Y$ are able to embedded in, plus $X$ and $Y$ need to have the same dimensionality. In \citet{dupuy2019estimating}, the affinity matrix has a low-rank constraint.
However, these assumptions do not hold in general.

Rather than adding another constraint, 
We aim to analyze the intrinsic properties and 
the underlying geometric structure of the set $ \{C\} = \Phi^{-1} (T^{\lambda})$ 
for the general case in the following sections.
%
% Other related approaches, largely the lovely work of Curturi and colleagues, formulate the problem as ground metric learning. 
% \citep{cuturi2014ground} proposed algorithms for Ground Metric Learning (GML) which learns a distance from labeled normalized histograms given a criterion.
% \citep{heitz2021ground} extended the work of GML to learn the ground metric where only a geodesic distance on a graph is considered.
% \citep{paty2020regularized} re-interpreted regularized OT problems as ground cost adversarial and solved for robust solutions under different regularization. 
%
To simplify the notation, we will omit the superscript $\lambda$,
and fix $\lambda = 1$ unless otherwise stated.
% Some results will be described in term of negative exponential cost matrix $K$. 
% Corresponding statements in terms of $C$ can be obtained by $K = e^{-C}$.
% % Prior $P_0(K)$ is set to be the distribution where each column is follows symmetric Dirichlet distribution with hyperparameter $\alpha$ independently.
% Since for any non-negative cost matrix $C$, elements in $K$ are in the range of $(0,1]$, which can be cross-ratio equivalently 
% converted into a $K$ in the prior by column normalization.
% Observed $T$ is assumed to be a positive matrix, the case when $T$ is non-negative can be derived using  machinery of \textit{maximal partial pattern} 
% developed in \citep{pei2019generalizing}.









\section{Probabilistic inverse optimal transport} \label{sec:piot}

%\pat{remind people of our goal?}-\pw{added}
%In this section, we formalize the general IOT problem through Bayesian inference, 
%analyze key properties of $\Phi^{-1}(T)$ and reveal its underlying geometric structure. 


\begin{definition}\label{def: PIOT}
Let $T$ be a noisy observation of the optimal coupling~$T^*$.
\textbf{Probabilistic inverse optimal transport} is defined as: 
\begin{equation} \label{eq: PIOT}
 P(C|T) = \int _{T^* \in (\mathbb{R}^*)^{m\times n}} P(C|T^*) P(T^*|T) d T^*,    
\end{equation}
where $\displaystyle P(C|T^*) $ is obtained through Bayes' Rule:
\begin{equation} \label{eq: bayes}
 P(C|T^*)  = \frac{P(T^*|C) P_0(C)}{P(T^*)},   
\end{equation}
$P_0(C)$ is the prior of cost $C$; 
%over $(\overline{\mathbb{R}^*})^{m\times n}$; 
Likelihood $P(T|C) = 1$ if $C\in \Phi^{-1}(T)$, otherwise $P(T|C) = 0$;
$P(T^*) = \int P(T^*|C) P_0(C) \text{d} C$ is the normalizing constant;
$P(K|T)$ is used to denote the induced posterior on $K = e^{-C}$.
\end{definition}


\subsection{No observation noise}
In this section, we study the case when $T^* = T$.
As a direct application of Definition~\ref{def: PIOT}, we have:
\begin{proposition}\label{prop:piot}\footnote{Proofs for all results are included in Appendix \ref{apdx:proofs}.}
$ P(C|T)$ is supported on the intersection between $\Phi^{-1} (T)$ and the domain of $ P_0(C)$. Moreover, we have that 
$\displaystyle P(C|T) = \frac{P_0(C)}{\int_{\Phi^{-1} (T)} P_0(C) \text{d} C}$.
\end{proposition}

Therefore, characterization of $\Phi^{-1} (T)$ is essential to understand
the manifold on which the posterior distribution $P(C|T)$ is supported.

Notice that for any $C \in \Phi^{-1} (T)$, 
a Sinkhorn scaling of $K = e^{-C}$ results in $T$, and 
each step of Sinkhorn Scaling is a normalization which equivalent to 
multiplication of a diagonal matrix. %We show that: 

\begin{proposition}\label{prop:DAD}
Let $T$ be a non-negative optimal coupling of dimension $m\times n$. $C \in \Phi^{-1} (T)$ if and only if for every $\epsilon > 0$,
there exist two positive diagonal matrices $D^r = \diag\{d^r_1, \dots, d^r_m\}$ and $D^c =\diag \{d^c_1,\dots, d^c_n\}$ such that: 
$\displaystyle |D^r K D^c - T| < \epsilon$, where $K = e^{-C}$ and $|\cdot|$ is the $L^1$ norm. 
In particular, if $T$ is a positive matrix, then $C \in \Phi^{-1} (T)$ 
if and only if there exist positive diagonal matrices $D^r,D^c$ such that $D^r K D^c = T$, i.e.
\begin{equation}\label{eq:diag_equiv}
\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}.   
\end{equation}

\end{proposition}

Proposition~\ref{prop:DAD} identifies a key feature of matrices in $\Phi^{-1} (T)$. 
However, it is not easy to
verify whether an arbitrary matrix belongs to $\Phi^{-1} (T)$ nor reveal any underlying 
geometric structure of $\Phi^{-1} (T)$.

Towards these goals, we now introduce an equivalent condition: \textit{cross ratio equivalence} between \textit{positive} matrices, 
and show that the IOT set $\Phi^{-1} (T)$ can be completely characterized by $T$'s \textit{cross ratios}. 

\begin{definition}
Let $A, B$ be positive $m\times n$ matrices. $A$ is \textbf{cross ratio equivalent} to $B$, 
denoted by $A\overset{c.r.}{\sim} B$,
if all cross ratios of $A$ and $B$ are the same, i.e.
$$r_{ijkl}(A) := \frac{a_{ik} a_{jl}}{a_{il} a_{jk}} = \frac{b_{ik} b_{jl}}{b_{il} b_{jk}} := r_{ijkl}(B) $$
holds for any $i, j \in \{1, \dots, m\}$ and $k, l \in \{1, \dots, n\}$. 

\end{definition}

\begin{lemma}\label{lemma:cr_dr}
For two positive matrices $A, B$, 
$A \overset{c.r.}{\sim}B$ if and only if 
there exist positive diagonal matrices $D^r$ and $D^c$ such that $A = D^r B D^c$.
\end{lemma}



\begin{theorem}\label{thm:IOT}
Let $T$ be an observed positive optimal coupling of dimension $m\times n$. 
Then $\Phi^{-1} (T)$ is a hyperplane of dimension 
$m+n-1$ embedded in $ (\mathbb{R}^*)^{m\times n}$, which consists all the cost matrices 
that of the form:
\begin{equation}\label{eq:cr_equiv}
 \Phi^{-1} (T) = \{C \in (\mathbb{R}^*)^{m\times n} | K= e^{-C} \overset{c.r.}{\sim} T\}.    
\end{equation}

\end{theorem}

Cross ratio equivalence provides a strong connection between IOT and algebraic geometry.
Algebraically, cross ratios generate the set of algebraic invariants of matrix scaling.
The set of all scale reachable matrices from a coupling $T$, 
i.e. $\Phi^{-1}_K(T) \coloneqq \{K| D^{r}TD^{c}\} = \{K = e^{-C}| C\in \Phi^{-1}(T)\}$ forms an algebraic variety defined by the cross-ratios of $T$.
% For instance: the matrices $\tiny K = \begin{pmatrix} a & b \\ c & d \end{pmatrix} \in \mathcal{K}(T) $ for
% $\tiny T = \begin{pmatrix} 0.1 & 0.2 \\ 0.3 & 0.4 \end{pmatrix}$ (i.e. the set of possible negative exponential cost matrix) 
% are generic solutions to the equation $3ad-2bc=0$. 
Geometrically, the set $\Phi^{-1}_K(T)$ forms a special manifold \citep{fienberg1968geometry}.
$T$ is the unique intersection between $\Phi^{-1}_K(T)$ 
and the hyperplane determined by the linear marginal conditions.

\begin{remark}
Since a matrix $T$ and its normalization $T/\sum_{ij}(t_{ij})$ 
have the same cross ratios (hence have the same image under IOT),
we may relax the distribution constraint on the observed coupling $T$.
In this case, instead of probability, 
$t_{ij}$ represents the frequency of observing $x_i$ and $y_i$ simultaneously.
\end{remark}

\begin{example}\label{eg:hyperplane}
Let $\tiny T = \begin{pmatrix} 1 & 2 & 3\\ 2 & 3 & 1\end{pmatrix}$. 
$T$ has three cross ratios $r_{1212} (T) = \frac{3}{4}, r_{1213}(T) =\frac{1}{6} , r_{1223}=\frac{2}{9}$.
Only two are independent as $r_{1213}(T) = r_{1212}(T) * r_{1223} (T)$. Hence $\Phi^{-1}_K(T)$ 
is the solution set of the algebraic equation:
\begin{equation*}
\begin{aligned}[c]
\footnotesize
    \begin{cases}
      k_{11} k_{22}/ k_{12}k_{21} = 3/4\\
      k_{12} k_{23}/k_{13}k_{22} = 2/9
    \end{cases}
\end{aligned}
\Longleftrightarrow \hspace{0.08in}
\begin{aligned}[c]
\footnotesize
    \begin{cases}
      4 k_{11} k_{22} - 3 k_{12}k_{21} = 0\\
      9 k_{12} k_{23} - 2 k_{13}k_{22} = 0.
    \end{cases}
\end{aligned}
\end{equation*}
Further as $k_{ij} = e^{-c_{ij}}$, we obtain that $\Phi^{-1}(T)$ is the 4-dim hyperplane defined by the linear equations:
% \begin{subequations} \label{eq:T_1}
% \small
%   \begin{align}
%     & c_{12}+c_{21} - c_{11}-c_{22} = \small{\ln 3/4} \label{eq:T_1a}\\
%     & c_{13}+ c_{21} - c_{11} - c_{23} = \ln 1/6 \label{eq:T_1b}
%   \end{align}
% \end{subequations}
\begin{subequations} \label{eq:T_1}
\footnotesize
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln (3/4) \label{eq:T_1a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_1b}.
  \end{empheq}
\end{subequations}


% \begin{equation}\label{eq:T_1}
% \small
%     \begin{cases}
%       c_{12}+c_{21} - c_{11}-c_{22} = \ln\frac{3}{4}\\
%       c_{13}+ c_{21} - c_{11} - c_{23} = \ln \frac{1}{6}
%     \end{cases}
% \end{equation}
\end{example}


\begin{remark}\label{rmk:basis}
For a $m\times n$ matrix $A$, 
although there are $\binom{m}{2} \binom{n}{2}$ ways to choose $i,j,k,l$ to form cross ratios of $A$, 
not all are independent as seen in Example~\ref{eg:hyperplane}. 
A set of independent cross ratios that generates the entire collection of cross ratios is called a \textbf{basis}.
For example, it is easy to check that $\mathcal{B} = \{r_{1j1k}(A)| j = 2, \dots, m, k=2, \dots, n\}$ forms a basis for $A$.
\end{remark}

% \pw{The following paragraph may delete or simplified.}
% Another special case is when $T$ is a square matrix.
% Two square matrices are said to be \textit{\textbf{diagonal} ratio equivalent} 
% if the ratio between any two positive diagonals of the two matrices are the same (See definition and proofs in supplemental materials.).
% \citep{pei2019generalizing} showed that when $T$ is a square matrix, any $C \in \Phi^{-1} (T)$ is diagonal ratio equivalent to $T$.
% In the supplementary material, we prove that for positive square matrices, \textbf{diagonal} ratio equivalent coincides with cross ratio equivalent.
Observed $T$ is assumed to be a positive matrix for the rest of the paper,
the case when $T$ is non-negative can be derived using  machinery of \textit{maximal partial pattern} 
developed in \citep{pei2019generalizing}.

\textbf{Support manifold.} 
%Now we are ready to study the support manifold 
%of posterior distribution $P(C|T)$.
Since $\text{Supp}[P(C|T)] = \Phi^{-1} (T) \cap \text{Domain}[P_0(C)]$, 
different priors would add different constraints on $C$, which will result different submanifolds embeded in 
the hyperplane formed by $\Phi^{-1} (T)$.

For instance, suppose $P_0(C)$ follows a Dirichlet distribution over the entire matrix ~($\mathbf{P_1}$). 
Then 
$$\small \text{supp}[P(C|T)]  =\{C \in (\mathbb{R}^*)^{m\times n} | e^{-C} \overset{c.r}{\sim} T, \sum_{ij} c_{ij} = 1\}.$$
Notice that $K$ encodes the cross ratios of $T$, and to avoid the estimation of $\lambda$,
it is handy to directly put prior put over $K=e^{-C}$. 
For example, assume that $P_0(K)$ is the 
distribution where each column follows an independent Dirichlet distribution~($\mathbf{P_2}$) with hyperparameter $\alpha$.
% According to Proposition~\ref{prop:DAD}, we have:
% \[\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}\]
Then the domain of $P_0(K)$ is $\mathcal{P}(\mathbb{R}^{n})^{m}$. 
Therefore, based on Eq.~\eqref{eq:diag_equiv}, we have the intersection is of the form:
\begin{equation} \label{eq:supp_posterior}
    \text{supp}[P(C|T)] = \{ C | \exists D^{r} \text{ s.t. } K = \text{Col}(D^{r}T) \}.
\end{equation}



% Since for any non-negative cost matrix $C$, elements in $K$ are in the range of $(0,1]$, which can be cross-ratio equivalently 
% converted into a $K$ in the prior by column normalization.
%\centerline{$\d
% %isplaystyle \text{supp}[P(C|T)] = \{ \widehat{C} \in (\mathbb{R}^{+})^{m\times n} | \exists D^{r} \text{ s.t. } \widehat{C} \text{ is column normalization of } D^{r}T \}$ }
\begin{remark}\label{rmk: one_free_column}
Eq.~\eqref{eq:supp_posterior} indicates that: \textbf{(i)} a known column of $K$ uniquely determines all the other columns. 
Indeed, denote the $j$-th column of $K, T$ by $\mathbf{k}_j, \mathbf{t}_j$. 
For a known column $\mathbf{k}_j$, let $d_i = k_{ij}/t_{ij} $ and $D^{r} = \diag\{d_1, \dots, d_m\}$. 
Then the $l$-th column $\mathbf{k}_l$ equals to the column normalization of $D^{r} \mathbf{t}_l$.
\textbf{(ii)} for any $\mathbf{v} \in \mathcal{P}((\R^+)^m)$, there exists a $K \in  \text{supp}[P(K|T)]$ such that $\mathbf{k}_j = \mathbf{v} $.
Therefore, we have:

\end{remark}

\begin{corollary}\label{cor:proj_single_column}
Under prior $\mathbf{P_2}$,
the projection of $\text{supp}[P(K|T)]$ onto each column is a $(m-1)$-dimensional manifold that is homeomorphic to the simplex $\Delta_{m-1}$. 
\end{corollary}
\textbf{Subspace of $\text{Supp}[P(C|T)]$.} \label{para:subspace}
Let $C_s$ be the submatrix of the cost $C$ 
that corresponds to $X_s\times Y_s$, where $X_s = \{x_1, \dots, x_{s_1}\} \subset X$, $Y_s = \{y_1, \dots, y_{s_2}\}\subset Y$.
In this section, we characterize the support of $P(C_s|T)$ as a subspace of $\text{Supp}[P(C|T)]$.

Denote the sub-coupling of $T$ corresponding to $C_s$ by $T_s$.
According to Eq.~\eqref{eq:diag_equiv} and Eq.~\eqref{eq:cr_equiv}, 
the projection of $\Phi^{-1}(T)$ onto the cost over $X_s\times Y_s$
is in form of:
\begin{align*}
 \Phi^{-1}_s(T) &:= \{C_s | C_{s} \text{ is submatrix of a } C \in \Phi^{-1}(T)\} \\
 & = \{C_s| \exists D^r_s, D^c_s \text{ s.t. } K_s = D^r_s T_s D^c_s \}\\
 & = \{C_s|  K_s=e^{-C_s},  K_s \overset{r.c.}{\sim} T_s\}.
\end{align*}
$\text{Supp}[P(C_s|T)]$ is determined by  $\Phi^{-1}_s(T)$ and $P_0(C)$.
Intuitively, $\text{supp}[P(C_s|T)]$ contains all the matrices $C_s \in  \Phi^{-1}_s(T) $ such that there exists a proper extension of 
$D^r_s, D^c_s$ to $D^r, D^c$ such that $D^rTD^c$ is in the domain of $P_0(C)$. 

Take prior $\mathbf{P_2}$ as an example. Since the domain for a column of $K$ is a copy of $\Delta_{m-1}$ as shown in Corollary~\ref{cor:proj_single_column}, 
the domain for a column of $K_s = e^{-C_s}$ is then
a copy of $\Sigma_{s_1} = \{\mathbf{k} = (k_1, \dots, k_{s_1}) \in (\mathbb{R}^+ )^{s_1}| k_{1}+\dots +k_{s_1} < 1\}$. 
Hence, $\text{supp}[P(C_s|T)] $ should be contained in the set :
\begin{align*}
\mathcal{W}&  = \{C^s |\exists \text{ diagonal matrices } D_s^r, D_s^c \text{ s.t. }  \\
& K_s = D_s^rT_sD_s^c  \text{ and } \mathbf{1}_{s_1} K_s = (\alpha_1, \dots, \alpha_{s_2}), \alpha_i < 1 \}.   
\end{align*}

It is important to note that $\text{supp}[P(C_s|T)]$ is a proper subset of $\mathcal{W}$. 
As $K_s$ is a submatrix of $K$, the choice of $D_s^c$ must form a proper column normalizing constant of a $D^rT$. 
Thus, the choice of $D_s^c = \diag \{d^c_1, \dots, d^c_{s_2}\}$ must guarantee that there exist an extension of $D_s^r$, 
denoted by $D'^{r} = \diag\{D_s^r,d^r_{s_1 +1}, \dots, d^r_{m}\}$, with $d^r_{s_1 +1}, \dots, d^r_{m}>0$, 
such that the $j$-th column sum of $D'^{r} T$ is $1/d^c_j$.
Let $T_{m-s}$ be the submatrix of $T$ corresponding to $\{x_{s_1+1}, \dots, x_{m}\} \times Y^{s}$.  %We show that:
\begin{proposition}\label{prop:submanifold}
$C_s \in \text{supp}[P(C_s|T)]$ if and only if there exists positive diagonal matrices $D_s^c, D_s^r$ such that $K_s = D_s^c T_s D_s^r$ and
the system of equations 
$(x_1, \dots, x_{m-s_1}) T_{m-s}  = (1/d^c_1, \dots, 1/d^c_{s_2}) - \mathbf{1}_s D_s^rT_s$ have a positive solution for $\{x_1, \dots, x_{m-s_1}\}$.
\end{proposition}



\textbf{Incomplete Observation.}
\label{para:missing_element}
%We characterize the support of $P(C|T)$, when $T$ has a missing element.
Say $T$ is observed with $t_{m1}$ missing. Then generically, we have: 

\centerline{$\text{supp}[P(C|T)] = \cup_{\widehat{T} \in U(T)} \text{supp}[P(C|\widehat{T})]$,}
where $U(T)$ is the set of matrices with $T$ completed by a choice of $t_{m1}>0$.
Given a prior, say $\textbf{P1}$, we have: 

\vspace{0.1in}
\centerline{$\text{supp}[P(C|T)]  =\{C | \exists t_{m1} >0 \text{ s.t. } K \overset{c.r}{\sim} \widehat{T}, \sum_{ij} c_{ij} = 1\}$,}

where $\widehat{T}$ is $T$ with $t_{m1}$ as its $m1$-th element. With prior $\textbf{P2}$, according to \eqref{eq:supp_posterior} we have:
$$\text{supp}[P(C|T)] = \{ C | \exists D^{r}, t_{m1} >0, \text{ s.t. } K = \text{Col}(D^{r}\widehat{T}) \}.$$

Moreover, according to Remark~\ref{rmk: one_free_column}, 
a known column $\mathbf{k}_l$ of $K$ completely determines 
other fully observed columns. Whereas, for a column with a missing element, say the first column, 
$\mathbf{k}_l$ determines an 1-dim set $\mathcal{K}_1$ for $\mathbf{k}_1$.
% forms a line segment in $\Delta_{m-1}$.
In particular, let $D^{r} = \diag \{d_1, \dots, d_m\}$, where $d_i = k_{il}/t_{il}$.
%We show:
%$D^{r} = \diag \{k_{1l}/t_{1l}, \dots, k_{ml}/t_{ml}\}$
\begin{corollary}\label{cor:missing_element}
Under prior $\mathbf{P_2}$, 
$\mathcal{K}_1$ is a line segment in $\Delta_{m-1}$ that can be parameterized as:
\centerline{$\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} \in (0,\infty) \}$.}
\end{corollary}


% Then the line segment can be parameterized as 
% $\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} = \widehat{t}_{m1} \in (0,\infty) \}$.


Note that for different choice of priors, $\mathcal{K}_1$ could be a curve instead of a line segment. 
Denote the prior imposed constraint on $\mathbf{k}_1$ by $f_1(\mathbf{k}_1) = 0$,
the ratio imposed linear constraint on $\mathbf{k}_1$ by $f_i(\mathbf{k}_1) = 0$, where $f_i(\mathbf{k}_1) = k_{11}/k_{i1} - d_1*t_{11}/(d_i*t_{i1})$,
for $i = 2, \dots, m-1$.
Then $\mathcal{K}_1$ is the solution set for system of equations $\{f_1, f_2, \dots, f_{m-1}\}$.
With Dirichlet prior, $f_1$ is also linear, so $\mathcal{K}_1$ is a segment. 




\subsection{With observation noise}
%In this section, we study the general case when there are observation noises. 

%First, f
For any two observed couplings with the same dimension, we introduce a natural distance between 
their images under IOT.

\begin{corollary}\label{cor:parallel}
Let $T_1, T_2$ be two positive matrices of dimension $m \times n$.
The hyperplanes $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
In particular, if $T_1 \overset{c.r.}{\sim}T_2$ then $\Phi^{-1}(T_1) = \Phi^{-1}(T_2)$.
Otherwise $\Phi^{-1}(T_1)$ is parallel to $\Phi^{-1}(T_2) $.
\end{corollary}

Therefore, $\Phi^{-1}(T_1) , \Phi^{-1}(T_2)$ are the same or parallel hyperplanes
embedded in $(\mathbb{R}^{+})^{m\times n}$. \textbf{The distance between IOT of $T_1$ and $T_2$}, 
denoted by $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$ 
is then well-defined to be the Euclidean distance between $\Phi^{-1}(T_1) $ and $\Phi^{-1}(T_2)$.

Moreover, $\Phi^{-1}(T) $ is completely determined by $T$'s cross ratios.
So $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$ can be expressed in term of cross ratios of $T_1$ and $T_2$.
We now illustrate how to obtain $d(\Phi^{-1}(T_1) , \Phi^{-1}(T_2))$.
\begin{example}
Let $T_1 = T$ in Example~\ref{eg:hyperplane}, 
$\tiny T_2 = \begin{pmatrix} 1 & 2 & 3\\ 3 & 2 & 1\end{pmatrix}$.
Then $\Phi^{-1}(T_1)$ is the hyperplane show in~Eq.~\eqref{eq:T_1}.
Taking $r_{1212}, r_{1213}$ as $T$'s cross ratio basis, 
then we have $\Phi^{-1}(T_2)$ is: 
\begin{subequations} \label{eq: T_2}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln (1/3) \label{eq:T_2a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (1/3) \label{eq:T_2b}.
  \end{empheq}
\end{subequations}
%Eq~\eqref{eq:T_1} and Eq~\eqref{eq:T_2} have the same coefficients, 
Both $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$ are intersections of two 5-dim hydroplanes 
(i.e.\eqref{eq:T_1a} $\cap$ \eqref{eq:T_1b}, \eqref{eq:T_2a} $\cap$ \eqref{eq:T_2b})
with the same coefficient, so they are are parallel. 
Let the Dihedral angle between \eqref{eq:T_1a} and \eqref{eq:T_1b} be $\theta$.
It is easy to check $\cos \theta = 1/2$. 
So %by law of cosines, 
we have \scalebox{0.9}{$d(\Phi^{-1}(T_1), \Phi^{-1}(T_1) ) = \sqrt{\ln^2 \frac{4}{9} + \ln^2 \frac{3}{2} -\ln \frac{3}{2} \ln \frac{4}{9}}$}.
%$d(\Phi^{-1}(T_1), \Phi^{-1}(T_1) ) = \sqrt{(\ln 1/3 - \ln3/4)^2 + (\ln 1/6 - \ln1/9)^2 - 2(\ln 1/3 - \ln3/4)(\ln 1/6 - \ln1/9) \cos \theta } $
\end{example}

\begin{remark}
The hyperparameter $\lambda$ in Eq.\eqref{eq:eot} can be viewed as a greedy data selection. 
For a forward EOT problem, $\lambda$ raises the cross ratios of $K=e^{-C}$ to a power of $\lambda$.
Hence, $\lambda$ either exaggerates or suppresses the cross ratios of $T$, 
depending on whether $\lambda$ is greater or less than $1$ \citep{wang2020mathematical}.
Conversely, given a backward IOT problem, for a fixed coupling $T$, the larger the $\lambda$ is assumed, 
the smaller the cross ratios of $K$ are. 
Moreover, for a pair of observed couplings $T_1$ and $T_2$, 
the equations for hyperplanes corresponding $\Phi^{-1} (T_1), \Phi^{-1} (T_2)$ with different choices of $\lambda$, only differ 
on the constants by a scalar, i.e. $d_{\lambda}(\Phi^{-1} (T_1), \Phi^{-1} (T_2)) = d(\Phi^{-1} (T_1), \Phi^{-1} (T_2))/\lambda$.
Therefore, the larger $\lambda$ is assumed, the smaller the distance between $\Phi^{-1} (T_1)$ and $\Phi^{-1} (T_2)$ are.
\end{remark}

Assuming uniform prior $P_0(C)$ over $(\mathbb{R}^*)^{m\times n}$, 
we now investigate $P(C|T)$ under two common noise types. 
Results for other specific priors can be obtained by restricting the generic results to the prior's domain.
Without loss, 
we will assume noise only occurs on one element of $T$, say $t_{11}$, 
as the general case may be treated as compositions of such.

\textbf{Bounded noise.} 
% Consider the case where elements of the noisy observation $T$ 
% is within a bounded distance away from the optimal coupling $T^*$.
Suppose that $t_{11}$ is perturbed 
by a uniform noise from $t^*_{11}$, i.e. $t^*_{11} = t_{11} + \epsilon$, 
where $\epsilon$ is a random variable with uniform distribution over $[-a, a]$, for $a>0$.
%Then according to Eq~\ref{eq: PIOT}, assuming uniform prior $P_{0}(C)$,
% $P(C|T)$ is a uniform distribution over it support.

Theorem~\ref{thm:IOT} and Corollary~\ref{cor:parallel} imply that 
$P(C|T)$ is supported on a collection of parallel hyperplanes 
within bounded distance from $\Phi^{-1}(T)$. 
%More precisely, we show:

\begin{proposition} \label{prop: bounded_noise}
For a coupling $T$,  assume uniform observation noise on $t_{11}$ with bounded size $a$, then
$$\text{supp}[P(C|T)] = \cup_{T'\in \mathbb{B}_{a}(T)} \Phi^{-1}(T'),$$
where $\mathbb{B}_{a}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t'_{11}>0$, $|t'_{11} - t_{11}| \leq a$ and $t'_{ij} = t_{ij}$ for other $i, j$.
Moreover, $\Phi^{-1}(T')$ can be expressed as intersection of two hyperplanes (may be in different dimensions):
one with equation: $c_{11} + c_{22} - c_{21} - c_{12} = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$, 
and the other equation does not depend on the value of $t'_{11}$. Assume the angle between these two hyperplanes is $\theta$.
Then $d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \ln \frac{t_{11} + a}{t_{11} - a} /\sin \theta $, for $T_1', T_2' \in \mathbb{B}_{a}(T)$.
\end{proposition}

\begin{example}\label{eg:bounded_noise}
Let $T$ be the same as Example~\ref{eg:hyperplane}.
Suppose there is a bounded noise $\epsilon$ on $t_{11}$ of size $a>0$.
Hence, $\text{supp}[P(C|T)]$ is the union of a collection of hyperplanes $\mathbb{B}_{a}(T)$ 
of the following form, where $\epsilon \in [-a, a]$.
\begin{subequations} \label{eq:T_3}
\small
  \begin{empheq}[left=\empheqlbrace]{align}
    c_{12}+c_{21} - c_{11}-c_{22} &= \ln [(3+3\epsilon)/4] \label{eq:T_3a}\\
    c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_3b}
  \end{empheq}
\end{subequations}
Let the angle between \eqref{eq:T_3a} and \eqref{eq:T_3b} be $\theta$.
Computation shows that $\sin \theta = \sqrt{3}/2$, Hence for $T_1', T_2' \in \mathbb{B}_{a}(T)$, 
$d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \sqrt{3}\ln (1+a)$.
\end{example}

\textbf{Gaussian noise.} Suppose that $t_{11}$ is perturbed 
by a Gaussian noise from the ground truth $t^*_{11}$, i.e. $t^*_{11} = t_{11} + \epsilon$, 
where $\epsilon \sim \mathcal{N}(0, \sigma^2)$ with standard deviation $\sigma >0$.

Gaussian distribution is defined over the entire real line, 
% $P(T^*|T)$ is supported on the set $\mathcal{L}(T)$ consists matrices $T'$ of the same dimension of $T$ 
% with the propriety that:
% $t'_{ij} = t_{ij}$ for $(i, j) \neq (1,1)$. 
so $\text{supp}[P(C|T)] = \cup_{T'\in \mathbb{L}_{a}(T)} \Phi^{-1}(T')$,
where $\mathbb{L}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t_{11}>0$ and $t'_{ij} = t_{ij}$ for $(i, j) \neq (1,1)$.
Therefore, cross ratios of $T'$ that depend on $t_{11}$ can be any arbitrary number.
So similar to the case of missing elements in $T$, 
$P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T^*)$.
%In particular, we show:

\begin{proposition} \label{prop: gaussian_noise}
Let $T$ be an observed coupling of dimension $m\times n$ with Gaussian noise on $t_{11}$.
Further, let $\mathcal{B}$ be a basis for cross ratios of $m\times n$ matrices, that contains only one cross ratio depending on $t_{11}$.
Eliminate the cross ratio depending on $t_{11}$ in $\mathcal{B}$, denote the new set by $ \mathcal{B}^{-}$. Then: 

\centerline{$\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$}
In particular, $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T^*)$.
\end{proposition}

\begin{example}\label{eg:Gaussian_noise}
Let $T$ be the same as Example~\ref{eg:hyperplane}.
Suppose there is a Gaussian noise $\epsilon \sim \mathcal{N}(0, \sigma^2) $ on $t_{11}$.
Hence, $\text{supp}[P(C|T)]$ is the union of a collection of hyperplanes in $\mathbb{L}(T)$,
which are in the same form as Eq~\ref{eq:T_3}, with constraint on $\epsilon$ being:
% \begin{subequations} \label{eq:T_4}
% \small
%   \begin{empheq}[left=\empheqlbrace]{align}
%     c_{12}+c_{21} - c_{11}-c_{22} &= \ln [(3+3\epsilon)/4] \label{eq:T_4a}\\
%     c_{13}+ c_{22} - c_{12} - c_{23} &= \ln (2/9) \label{eq:T_4b}
%   \end{empheq}
% \end{subequations}
$3+3\epsilon >0$ and $\epsilon \sim \mathcal{N}(0, \sigma^2) $. Thus,
$\epsilon \in (-1, \infty)$, which further suggests no restriction is put on 
$c_{12}+c_{21} - c_{11}-c_{22}$. Hence:
\vspace{0.1in}
\centerline{$\text{supp}[P(C|T)] = \{C| c_{13}+ c_{22} - c_{12} - c_{23} = \ln \frac{2}{9} \}.$}
\end{example}

\begin{remark}
In this case, $P(C|T)$ is not uniform over its support. 
According to Eq~\eqref{eq: PIOT}, $P(C|T) \propto P(T_C|T)$ where $T_C \in \mathbb{L}(T) $ and $K = e^{-C} \overset{c.r.}{\sim}T_C$.
In particular, $P(C|T)$ has the highest probability on the hyperplane $\Phi^{-1}(T)$. 
If further constraints are added to the cost matrix $C$ such that 
there is a unique $C \in \Phi^{-1}(T)$ that meets such constraints, 
then one may obtain a maximum a posteriori estimation of $C$.
This explains why the simulations in \citep{stuart2020inverse}, failed to identify a unique cost matrix
for the general case:
 $P(C|T)$ is supported on an entire hyperplane. 
%In contrast, m
Whereas, maximum a posteriori estimations of $C$ were successfully obtained in both the 
graph and Toeplitz cases.% \citep{stuart2020inverse}. %\wt{Do they use MAP or just sampling the posterior?}
\end{remark}
% \pw{pictures within each subsection or all pictures in a simulation section?}
% \wt{Noise on marginals? Eg. when we do PIOT on NBA data, can we add noises on the original row marginals to make predictions? After we obtain the posterior distributions we samples sets of noisy row marginals, and then use the posterior as cost and noisy marginals to find OT plans. }

==> ICML-sumission/3-experiment_ICML.tex <==

\section{Algorithm}

\textbf{Approximate inference via MCMC.}
%
Given a perfectly observed $T$ and $P_0(C)$, we propose a Markov Chain Monte Carlo (MCMC) method 
% based  on the Metropolis algorithm\citep{metropolis1953equation} 
for sampling $P(C|T)$ (see Algorithm 1).
%from the posterior distribution. 
%The cross-ratio of the generated cost matrices are the same as $T$. 
%
%The algorithm works as follows. %\footnote{We suppress the $\lambda$ superscript to simplify notation of iterations.} 
At iteration $i$, denote the current cost $C$ by $C^{(i)}$, $K^{(i)} = e^{-C^{(i)}}$.
We generate two vectors $D^r$ and $D^c$ with each element sampled from an exponential of a Gaussian distribution $\mathcal{N}(0,\sigma^2)$. 
$K^{(i+1)}$ is then obtained by $K^{(i+1)} = \diag{D^r}K^{(i)}\diag{D^c}$.
%and scale rows in $K^{(i)}$ by left multiplying $D^r$ and columns by right multiplying $D^n$ to give $K^{(i+1)}$. 
%We compute the probability of the cost matrix, $P($log$(K^{(i)} | \mu)$. 
The acceptance ratio, $r = \frac{P(-\ln (K^{(i+1)}) | T)}{P(-\ln(K^{(i)}|T)} \overset{(*)}{=} \frac{P_0(C^{i+1}, \beta)}{P_0(C^{i}, \beta)}$
%$r = \frac{P_0(C^{i+1})}{P_0(C^{i})} = \frac{P(\text{log}(K^{(i+1)}) | \theta)}{P(\text{log}(K^{(i)}) | \theta)}$, 
where $\beta$ is the hyperparameter of prior $P_0(C)$. %represents the parameters of the model. %\pw{check with wei-ting.}
Equality~$(*)$ holds because our proposal preserves the cross-ratios, so we are guaranteed to stay on the manifold of support. 
Therefore, $P(T|C)$ is always $1$ and is omitted (see Proposition~\ref{prop:piot}). 
We accept or reject the move by comparing the acceptance ratio to an uniform random variable, $u$, 
which concludes a single step of the MCMC algorithm. 
%
We refer this method as MetroMC.
%\pw{the algorithm should be on cost $C$, not $K$}
\begin{algorithm}[tb]
\caption{ MetroMC }\label{algo:MetroMC}
\begin{algorithmic}
\INPUT{: coupling $T$, variance $\sigma$, Prior parameters $\beta$, uniform random variable $u$ $\in$ [0, 1)}
\SET{: $C^{(0)}=-\ln(K^{(0)})$; $K^{(0)}=T_{m\times n}$}
\FOR{ i = 1 to ITERMAX} 
    \STATE $D^{r} =$ exp$( N(0, \sigma * \mathbb{I}_{m}) )$
    \STATE $D^{c} =$ exp$( N(0, \sigma * \mathbb{I}_{n}) ) $
    \STATE $K^{(i+1)}\leftarrow$ diag($D^r$) $K^{(i)}$ diag($D^c$)
    \STATE $C^{(i+1)} = -\ln (K^{(i+1)})$
    \STATE $a$ $\leftarrow P(C^{(i+1)}| T) / P(C^{(i)}|T)$
    \IF{ a $>$ u}
        \STATE Accept $C^{(i+1)}$
    \ELSE
        \STATE Reject $C^{(i+1)}$
        \STATE $C^{(i+1)} \leftarrow C^{(i)}$
    \ENDIF
\ENDFOR
\OUTPUT{: $\mathbf{C}$}
\end{algorithmic}
\end{algorithm}

\textbf{Metropolis-Hastings Monte Carlo method.}
%
We can avoid dealing with the parameter $\lambda$ by putting a prior on $K$. However, 
the MetroMC has long autocorrelation time for such priors. 
%does not work well for such priors. The inverse procedure involves scaling 
%the rows and columns of the observed coupling with exponential factors, and experiments show that symmetric proposal distribution used in MetroMC is not efficient (has very long autocorrelation time) 
%for $\mathbf{P}_2$. \pat{we should explain why this is so. it will not at all be obvious to the reader.} 
%\wt{Explain:} 
%The reason is that i
In each iteration, $K^{(i+1)}$ is obtained by \textit{multiplying} random factors on $K^{(i)}$, 
whereas $C^{(i+1)}$ is obtained by \textit{adding} random factors on $C^{(i)}$.
In more detail, rows of $K^{(i)}$ are scaled by exponential of Gaussian variables 
a lot of time only a few of rows are at the same scale. After the columns are normalized, 
the rows that have large scale will have most of the weight in a column, which means we will sample a lot on the boundaries of the support.
In order to improve the efficiency, we utilize the Metropolis-Hastings \citep{hastings1970monte} sampling method. 

Now we propose an algorithm to sample from $P({K|T})$ with a prior on $K$.
The sufficient condition for the ergodicity of the MCMC method is detailed balance, which is defined as
% \begin{equation}
% \pi(s)P(s'|s)=\pi(s')P(s|s'),
% \label{eq:detailed_balance}
% \end{equation}
% where $\pi$ is the equilibrium distribution and $P(s'|s)$ is the transition probability to any state s' given a state s. At the end of a MC simulation, we will have the target distribution $\pi(s)$. Eq.~\eqref{eq:detailed_balance} can be re-written as 
$\pi(K)Q(K'|K)A(K', K)=\pi(K')Q(K|K')A(K, K')$,
% \begin{equation}
% \pi(s)Q(s'|s)A(s', s)=\pi(s')Q(s|s')A(s, s'),
% \label{eq:detailed_balance_2}
% \end{equation}
where $\pi(K)$ is the stationary distribution, $Q(K'|K)$ is the proposal transition probability from a state $K$ to $K'$ and $A(K',K)$ is the acceptance probability which we choose
\begin{equation}
A(K', K)=\text{min} \left(1, \frac{P(K')}{P(K)}\frac{Q(K|K'))}{Q(K'|K)} \right).
\label{eq:acceptance_prob}
\end{equation}
We replace the acceptance probability $a$ in Alg.~\ref{algo:MetroMC} with Eq.~(\ref{eq:acceptance_prob}). We refer this algorithm as the MHMC.

The proposal transition probability $Q(K'|K)$ is defined as follows.
In each iteration of MHMC, we draw a random number $\epsilon_i$ from a Gaussian distribution $\mathcal{N}(0, \sigma^2)$, where $\sigma$ depends on the row sums of $K$.
More precisely, $\sigma=\sigma_0*s_i^{\gamma}+\delta$, where $\sigma_0$, $\gamma$, and $\delta$ are hyper-parameters for the model and $s_i = \sum_j K_{ij}$. 
$K' = \text{diag}(D_i^r) K$, where $D_i^r = e^{[0,..,0,\epsilon_i,0,...,0]}$.

We %use the Gibbs sampling method to 
scale a row at once, so in each step the acceptance ratio is reduced to $A(s_i'|s_i)$. To compute it we need 
$Q(s_i'|s_i)=F_N(x=\ln(s_i'/s_i), \mu, \sigma) $ and 
$Q(s_i|s_i')=F_N(x=\ln(s_i/s_i'), \mu', \sigma')$,
% \begin{align*}
% Q(s'|s)=&F_N(x=\ln\frac{s'}{s}, \mu=0, \sigma) \\
% Q(s|s')=&F_N(x=\ln\frac{s}{s'}, \mu'=0, \sigma'),
% \end{align*}
where $F_N(x, \mu, \sigma)$ is the Gaussian probability density function.% $\mathcal{N}(\mu, \sigma^2)$.
%Gaussian probability density function with mean = $\mu$ and standard deviation = $\sigma$ at $x$. Namely, 
% \begin{equation}
% F_N(x, \mu, \sigma) = \frac{1}{\sqrt{2\pi}}e^{-\frac{1}{2}\frac{(x-\mu)^2}{\sigma^2}}
% \label{eq:Gaussian_pdf}
% \end{equation}

% In our simulations, we sample the next state $s'$ based on the current state $s$. We take s to be the sum of the row/column being scaled, $\mu=\mu'=0$, the standard deviation $\sigma=\sigma_0*s^k+\delta$ where $\sigma_0$, $k$, and $\delta$ are hyper-parameters.
%

% Move to supplements
% \subsection{Auto-correlation function.}

% To monitor the efficiency of our MCMC method, we compute the auto-correlation function during the burn-in phase and choose the lags accordingly.

% The auto-correlation function is defined as
% \begin{equation}
% R(t)=\frac{1}{(N-t)\sigma^2}\sum_{l=1}^{N-t}\sum_{i,j}(K_{i,j}^{(l)}-\bar{K}_{i,j})\cdot(K^{(l+t)}_{i,j}-\bar{K}_{i,j}),
% \label{eq:autocorrelation}
% \end{equation}
% where $N$ is the total number of samples generated, (i,j) runs over all indices of the matrices $K$, $\bar{K}$ is the mean averaging over all the samples, and $\sigma_K^2=\sum_{i,j}\sigma_{K,i,j}^2$ is the variance. 


\section{Experiments}\label{sec:simulations}

%\subsection{Effects of matrix size on manifold behavior.}

\textbf{Visualizing subspaces of $\text{supp}[P(K|T)]$.} Fig~\ref{fig:2x2_subspace}(a-c) illustrates 
support of $2\times 2$ subspaces $\text{supp}[P(K^s|T)]$, for a $4\times 4$ coupling $T$ under prior $\mathbf{P}_2$.
In each plot, a $T$ is sampled from a Dirichlet distribution \footnote{All coupling $T$s in this section are reported in Appendix~\ref{apd:sec:matrices}.}.
Consider submatrix %$\tiny K^s=\begin{pmatrix} k_{11}& k_{12} \\ k_{21} & k_{22}\end{pmatrix}$ 
$K_s = [[k_{11}, k_{12}],[k_{21}, k_{22}]]$ of $K$. 
According to section~\ref{para:subspace}, both columns $\mathbf{k}_1, \mathbf{k}_2$ of $K_s$ lie in a copy of $\Sigma_2$. 
Each colored triangle mark represents a uniformly sampled $\mathbf{k}_1$ from $\Sigma_2$. 
A sampled $\mathbf{k}_1$ determines a $D^r_s = \diag\{k_{11}/t_{11}, k_{21}/t_{21}\}$, 
which further determines a set $\mathcal{K}_2 $ for $\mathbf{k}_2$  shown by solid segment with the same color.
% the corresponding $\mathcal{K}^s_2$, the set of $\mathbf{k}^s_2$, is shown by solid segment with the same color,
Projection of $\mathcal{W}$ into the simplex corresponding to $\mathbf{k}_2$, denoted by $\mathcal{W}_2$, is shown by the dashed ray.
Here, $\mathcal{K}_2$ is obtained by: fix $\mathbf{k}_1 = (k_{11}, k_{21})^T$, 
further sample $k_{31}$ and $k_{41}$ to form the first column of $K$.
Then compute and plot the uniquely determined $\mathbf{k}_2$. 
As predicted in section~\ref{para:subspace}, $\mathcal{K}_2$ is only a subset of $\mathcal{W}_2$. 
The sizes and locations of $\mathcal{K}_2$ in $\mathcal{W}_2$ vary according to cross ratios of $T$.

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c c}
    \hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_1.png}}
            \put(60,60){\textbf{a.}}
        \end{picture}
        %\textbf{a.}\includegraphics[width=0.2\textwidth]{figs/submat_1.png}
        &\hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_2.png}}
            \put(60,60){\textbf{b.}}
        \end{picture}
    %\end{tabular}
    %\begin{tabular}{c c}
        &\hspace{-7pt}
        \begin{picture}(70,70)% width and height of the picture
            \put(0,0){\includegraphics[width=0.16\textwidth]{figs/submat_3.png}}
            \put(60,60){\textbf{c.}}
        \end{picture}
    %     &\hspace{-7pt}
    %     \begin{picture}(50,50)% width and height of the picture
    %         \put(0,0){\includegraphics[width=0.12\textwidth]{figs/submat_4.png}}
    %         \put(40,40){\textbf{d.}}
    %     \end{picture}
    \end{tabular}
    \caption{
    Visualization of $2\times 2$ subspaces of $\text{supp}[P(K|T)]$. 
    In each plot, a $T$ is sampled from a Dirichlet distribution. 
    Each colored mark represents a uniformly sampled $\mathbf{k}_1 = (k_{11}, k_{21})^T$.
    Solid segment with the same color plots the corresponding set $\mathcal{K}_2$ for the second column, and
    the dashed ray plots $\mathcal{W}_2$. 
     }%Randomly generates the elements of first column of $K$ with $\sum_{i} K_{i,j} = 1$. Three sets of points are sampled for each plot and represented in different colors. Triangular points are ($K_{1,1}$, $K_{2,1}$) of first column; Lines are sets of points ($K_{2,1}$, $K_{2,2}$) of column 2.}
    \label{fig:2x2_subspace}
    \label{fig:subspace}
\end{figure}



%\subsection{Inferring censored values.}
%\subsection{Tests of MC samplers.}
% Supplement
% \pw{let's shorten?} \pat{move the whole section with the figure to supplement?}
% \textbf{Validation of MHMC.} In this section, we validate our MHMC algorithm by apply it to an uniform $T$, i.e $T_{m,n}=1/m$ 
% under prior $\mathbf{P}_2$.
% %on uniform matrices, e.g. $T_{m,n}=1/m$ for the column-wise Dirichlet prior case. 
% The cross-ratios of $T$ are all 1 and stay the same for all inferred sample $K^{(i)}$. 
% Thus, each $K^{(i)}$ has same copies of $n$ columns. 
% We compare posterior sample by MHMC to a 
% $m$-dimensional uniform symmetric Dirichlet distribution generated by the SciPy package \citep{2020SciPy-NMeth}.  
% %\footnote{Cite SciPy: https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.dirichlet.html}
% Fig.~\ref{fig:uniform_3x3} shows the results the 3x3 case.
% are the same for every element. We choose $\alpha=1$ for the Dirichlet prior, 
% $\sigma_0=0.5$, $k=3$, and $\delta=1.0$. 
% We run for 10,000 burn-in steps and take 10,000 samples 
% with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. 
% We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps.
% Also, the running averages of the row sums are stable at taking 10,000 samples, 
% which means 10,000 samples can effectively represent the posterior distribution. The plots for autocorrelation and running average are in appendix.

% % We perform our MHMC algorithm on a 3x3 uniform matrix with a symmetric column-wise Dirichlet prior, i.e. $\sum_i K^{(i)}_{i,j}=1$ and the Dirichlet concentration parameter $\alpha$ are the same for every element. We choose $\alpha=1$ for the Dirichlet parameter, $\sigma_0=0.5$, $k=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps. Also, the running averages of the row sums are stable at taking 10,000 samples, which means 10,000 samples can effectively represent the posterior distribution. The plots for autocorrelation and running average are in appendix.

% The posterior distribution is compared to the distribution $P(K|T)$ of three-dimensional vectors generated by Dirichlet vector sampler \citep{2020SciPy-NMeth} with symmetric $\alpha=1$ in Fig.~\ref{fig:uniform_3x3}. The results are comparable, which suggests that our MHMC method is able to generate distributions which well represent the support of the posterior distributions.


% \begin{figure}[h!]
%     \centering
%     \begin{tabular}{c c}
%         \hspace{-4pt}\includegraphics[width=0.235\textwidth]{figs/dirichlet_3.png}
%         \hspace{-6pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3.png}
%     \end{tabular}
%     % \begin{tabular}{c c}
%     %     \hspace{-4pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3_autocorr.png}
%     %     \hspace{-6pt}\includegraphics[width=0.235\textwidth]{figs/uniform_posterior_3x3_running_avg.png}
%     % \end{tabular}
    
%     \caption{\textbf{(Left.)} \pat{row rather than square?} The distributions of each component of three-dimensional Dirichlet vectors with symmetric $\alpha=1$ generated using SciPy package. \textbf{(Right.)} The distributions of each component of the first column of $P(K|T)$ sampled by the MHMC method. %\textbf{(Lower left.)} The auto-correlation function of the MHMC simulation. The black dashed lines indicate the range [$-1/e$, $1/e$]. \textbf{(Lower right.)} The running average of the row sums of the MHMC simulation.
%     }
%     \label{fig:uniform_3x3}
% \end{figure}

\textbf{Visualizing $\text{supp}[P(K|T)]$ through MHMC.} Now we utilize MHMC to visualize supp[$P(K|T)$] and see the effect of cross-ratios. 
Under prior $\mathbf{P}_2$ with $\alpha =1$, Fig.~\ref{fig:sample_supp} illustrates the posterior distributions $P(K|T)$ of three $3\times 3$ couplings. 
% Here couplings $T$ are generated by solving an OT problem with uniform marginals $\mu, \nu$, and random column Dirichlet matrices $K^g$. 
% \pw{what is $K^g$}.

%We simulate $P(K|T)$ using MHMC with the same parameters as in the previous uniform matrix case 
%\pw{fix}. \wt{fixed}
We choose $\alpha=1$ for the Dirichlet prior $P_0(K)$, $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. 
The choices of these numbers are validated in Appendix~\ref{apd:sec:MHMC}. 
Three columns (\textcolor{red}{red}, \textcolor{green}{green}, and \textcolor{blue}{blue} colors, respectively) 
of each $T$ are plotted in the simplex on the left of Fig.~\ref{fig:sample_supp}. 
Locations of these points illustrate the relations between each column encoded by the cross ratios of $T$. 
The right of Fig.~\ref{fig:sample_supp} plots columns of sampled $K$ from $P(K|T)$ with corresponding $T$ to the left. 
We clearly see how the cross-ratio of $T$ affects $P(K|T)$. 
If one column of $T$ is close to one edge, then the posterior distribution of that column will be denser on that edge; on the other hand, if a column of $T$ is located near the center, then the posterior is more evenly distributed on a simplex. 
%Since the relative location of each column should be kept to retain the cross-ratio equivalence for all inferred samples.
E.g. in the top case, the effects on red and blue are exaggerated because the effect depends on relative position (and similarly for the red in the middle panel). 

\begin{figure}[h!]
    \centering
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_1.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_1_1.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_1_2.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_1_3.png}
    \end{tabular}
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_2.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_2_1.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_2_2.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_2_3.png} 
    \end{tabular}
    \begin{tabular}{c | c c c}
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_3.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_3_1.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_3_2.png} &
        \includegraphics[width=0.09\textwidth]{figs/random_3x3_simplex_3_3.png} 
    \end{tabular}
    \caption{\textbf{(Left.)} The columns of three $T$ matrices plotted on the same simplex: $\mathbf{t}_1,\mathbf{t}_2, \mathbf{t}_3 $ are shown in
    \textcolor{red}{Red}, \textcolor{green}{green} for , \textcolor{blue}{blue}. 
\textbf{(Right.)} Samples from posterior distribution $P(K|T)$. Each column of inferred matrices $K$ are plotted in a separate simplex, indicated by corresponding color.}
    \label{fig:sample_supp}
\end{figure}

% T_1 = [[0.1104, 0.0684, 0.1545],
%         [0.0505, 0.2401, 0.0428],
%         [0.1725, 0.0249, 0.1360]]

% T_2 = [[0.0950, 0.1100, 0.1283],
%         [0.1155, 0.0343, 0.1835],
%         [0.1228, 0.1890, 0.0215]]

%  T_3 = [[0.1053, 0.1193, 0.1088],
%         [0.2148, 0.0090, 0.1096],
%         [0.0133, 0.2051, 0.1150]]

% Appendix
% \textbf{MetroMC on uniform matrix.} We test MetroMC on 3x3 uniform $T$, where $T_{i,j}=1/(m*n)$, and assume the prior is put on $C$, i.e. $\sum_{i,j}C_{i,j}=1$. For this method, we need to first re-normalize $T$ so that $K^{(0)} = F(T)$ is on the support of the posterior manifold. F(T) is defined as
% \begin{equation}
%     F(T) = \text{exp}\left({\frac{1+\sum_{i=1}^{m}\sum_{j=1}^{n}\text{log}(T_{i,j})}{m*n}}\right).
% \end{equation}
% For each MC iteration we sample $m+n-1$ Gaussian random numbers with standard deviations of 0.02 for the diagonal matrices $D^r$ and $D^c$ satisfying the condition 
% \begin{equation}
% \sum_{i,j}\text{log}(D^r_{i})+\text{log}(D^c_j)=0. 
% \label{eq:condition_bounded_noises}
% \end{equation}
% We burn in 10,000 steps and take 100,000 samples with 100 lags in between. The Gaussian Kernel density estimation (KDE) of each component of $P(C|T)$ is demonstrated in Fig.~\ref{fig:uniform_3x3_2}. We use bandwidths of 0.05 for all the Gaussian KDE in this article. There are a few notable features. First, we assume a Dirichlet prior on the whole $C$ matrix, the distributions will be smaller at large values because each large value will suppress the value of the other elements. Second, since we have cross-ratio = 1 everywhere in $T$ and matrix-wise symmetric Dirichlet prior on $C$, there will not be a single element with value close to one. Otherwise, the cross-ratio involving that element could never be 1 anymore. Also, for the same reason all distributions should be similar.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/pdf_unifrm_T_3x3.png}
%     \caption{\pat{move to supplement?} The KDE of each matrix element of $P(C|T)$ with a uniform $T$ and a symmetric Dirichlet prior over the whole $C$ matrix.}
%     \label{fig:uniform_3x3_2}
% \end{figure}

Visualization of $\text{supp}[P(K|T)]$ with 
incomplete observations is included in Appendix~\ref{apd:sec:missing_value}.

\textbf{Bounded noise on observed plan.}
Given an observed noisy $T$, 
we assume $t_{11}$ was perturbed by a bounded noise $\epsilon$ sampled uniformly 
from distribution $[-a, a]$ with $a=0.01$. 
Assuming prior $\mathbf{P}_1$ for $P_0(C)$ with symmetric Dirichlet parameter equals to $1$, 
we use MetroMC to sample $\text{supp}[P(C|T)]$.

% To see the effects of noise on the inferred cost we take five evenly spaced values within the range. A ground truth probability cost matrix $C^g$, whose elements are randomly rolled from a uniform distribution [0, 1] and normalized to $\sum_{i,j}C^g_{i,j}=1$, is generated and a OT problem is solved to obtain a plan $T^g$ with even marginals $\mu, \nu$ and $C^g$. For simplicity we do not add a random noise on $T^g$ to obtain the observed plan $T$, so $T=T^g$. 
%For the PIOT inference, the noise is added to the (1,1)-th element of the  observed plan $T$. 

% In order to make $-log(T)$ lie on the support of the posterior we re-normalize the plans upon performing the MCMC method by a factor $F(T)$.
% \pw{how about swap to }

Notice that initializing $K^{(0)} = T$ may cause the corresponding $C^{(0)}$ lies outside the domain of $P_0(C)$ as 
$\sum_{ij} c^{(0)}_{ij} = \sum_{ij} -\ln(t_{ij})$ is not guaranteed be $1$. This will cause an extremely 
long burning time. In order fix to this issue, we scale $K^{(0)}$ by a constant when necessary.
Scaling does not change the cross-ratios, hence it equivalent to a move within the support of $\Phi^{-1}(T)$. 

%We assume a symmetric Dirichlet prior on $P_0(C)$, where $\sum_{i,j}C_{i,j}=1$ and the Dirichlet parameters = 1 everywhere. 
For each iteration in the MCMC method we generate $m+n-1$ (rather than $m+n$) independent Gaussian random numbers 
with $\sigma = 0.02$ to construct vectors $D^r$ and $D^c$ 
satisfying $\sum_{i,j}\ln(d^r_{i})+\ln(d^c_j)=0$.
%eq.~\ref{eq:condition_bounded_noises}.
The purpose of the above condition is to ensure that the newly generated sample lies on the support of the posterior. Otherwise, the acceptance rate will be extremely low. Because $C$ is a positive matrix, the MetroMC method rejects any sample of $K$ if $\max_{(i,j)}k_{i,j}\ge 1$. 

Fig.~\ref{fig:bounded noise} shows the MetroMC results on the inferred cost matrices $C$ for a given $3\times 3$ coupling 
$T$. For each simulation we burn in 10,000 steps and take 100,000 samples with lags of 100. 
The acceptance rates range from 0.51 to 0.58. The MCMC method is validated by checking the autocorrelation function and the running averages. (See Appendix~\ref{supsec: alg}.)
Noise level $\epsilon$ is indicated by colors.
The \textbf{Left} panel plots components for a cross-ratio depend on $t_{11}$: $(c_{11}+c_{22})$ by solid curves and $(c_{21}+c_{12})$ by dashed curves.
The \textbf{Right} panel plots components for a cross-ratio dose not depend on $t_{11}$: 
$(c_{12}+c_{23})$ by solid curves and $(c_{13}+c_{22})$ by dashed curves.
All the curves are broadened using the Gaussian kernel density estimation (KDE) method with a bandwidth of 0.05. 
Fig.~\ref{fig:bounded noise} illustrates that curves for $(c_{11} + c_{22})$ and $ (c_{21} + c_{12})$ with the same $\epsilon$ (i.e. curves in the same color) are in the same shape.
The off-set between them varies as the noisy level changes. 
Whereas off-set between curves for $(c_{12}+c_{23})$ and $(c_{13}+c_{22})$ on the right panel remains a constant for any choice of $\epsilon$.
This is consistent with our theoretical result in Prop.~\ref{prop: bounded_noise} that:
$(c_{11} + c_{22}) - (c_{21} + c_{12}) = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$ depends on $\epsilon$,
whereas $(c_{12}+c_{23}) - (c_{13}+c_{22}) = - \ln\frac{t_{12} t_{23}}{t_{13}t_{22}}$ is a constant.
%\wt{Dies $t_{12}$ has a prime?}
%The cross-ratio pair including the (1,1)-th element.
% Hence curves for $(c_{11} + c_{22})$ and $ (c_{21} + c_{12})$ with a fixed $\epsilon$, i.e. curves in the same color, should be in the same shape.
% And their off-set varies as the noisy level changes. 
% Whereas curves for $c_{12}+c_{23}$ and $(c_{13}+c_{22})$) should be in the same shape with a fixed off-set.



% so only the difference between cross-ratio pairs of pairs of elements of $C$ which involve the element with noise changes as the value of the noise alters. E.g. the difference between the cross-ratio pair ($c_{11} + c_{22}$) and ($c_{21} + c_{12}$) is controlled by the noise added to $t'_{11}$ while the difference between another pair ($c_{12} + c_{23}$) and ($c_{13} + c_{22}$) is not, see 

% C = [[0.1626, 0.0279, 0.1071],
%       [0.1047, 0.1477, 0.1628],
%       [0.1358, 0.0265, 0.1249]]
% T = [[0.1067, 0.1141, 0.1125],[0.1175, 0.1052, 0.1106],[0.1092, 0.1139, 0.1102]]
% noises = [-0.01, -0.005, 0.0, 0.005, 0.01]

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
    \hspace{-8pt}\includegraphics[width=0.25\textwidth]{figs/random_T_bonded_noise_1.png} &
    \hspace{-18pt}\includegraphics[width=0.25\textwidth]{figs/random_T_bonded_noise_2.png}  
    \end{tabular}
    \caption{Results on infered cost $C$ given a $T$ with bounded noise $\epsilon$ on $t_{11}$.
    $\epsilon$ varies in $[-0.01, -0.005, 0.0, 0.005, 0.01]$, indicated by [\textcolor{blue}{blue}, \textcolor{cyan}{cyan}, \textcolor{black}{black},  
    \textcolor{magenta}{magenta}, \textcolor{red}{red}] in order.
    %The KDE of the distributions of cross-ratio pairs of pair of elements of $C$ with various noise added to $t_{11}$. 
    %The colors represent the noise, \textcolor{blue}{blue}: -0.01, \textcolor{cyan}{cyan}: -0.005, \textcolor{black}{black}: 0.0,  \textcolor{magenta}{magenta}: 0.005, and \textcolor{red}{red}: 0.01.
    \textbf{(Left)} Solid curves are for ($c_{11}+c_{22}$), and dashed for $(c_{21}+c_{12})$. 
    \textbf{(Right)} The solid curves are for ($c_{12}+c_{23}$), and dashed for $(c_{13}+c_{22})$.
    }
    \label{fig:bounded noise}
\end{figure}


%\subsection{Gaussian noise on observed plan.}
\textbf{Gaussian noise on observed plan.}\label{sec:gaussian_noise} We start with a Toeplitz ground truth cost function $C^g$ and obtain an OT plan, $T^g$, with $C^g$ and uniform $\mu, \nu$. A random Gaussian noise $\epsilon \sim \mathcal{N}(0, 0.004^2)$, about 4\% of the average value of $T$, is added to $t^g_{1,2}$, and the corrupted plan $T=T^g+\epsilon$. We then infer the posterior distribution $P(C|T)$. We put a $\mathbf{P}_1$ prior on $C$ with the hyperparameters follows toeplitz matrix format. 
%The prior of $P_0(C)$ is assumed to be toeplitz Dirichlet, where the matrix of the Dirichlet parameters is diagonal-constant and $\sum_{i,j}{C_{i,j}}=1$. 
Inference is done by first generating 10 random numbers $\epsilon_i^{*}\sim \mathcal{N}(0, 0.004^2)$ and apply the noise on $t_{12}$ to get $T_i^{*}=T+\epsilon_i^{*}$. Then, we utilize MetroMC on every $T_i^{*}$ to obtain $P(C|T_i^{*}$), and finally $P(C|T)\approx\sum_i P(C|T_i^{*})$. %\wt{Confirm notation with paragraph after remark 3.16.}

For the MetroMC method, we burn in 10,000 steps and then take 10,000 samples with lags of 200 steps for each $P(C|T_i^{*})$. For each step, we use the same sampling procedure as described in the bounded noise case but use a Gaussian standard deviation of 0.003. The acceptance rates are around 0.52-0.70.

The posterior distributions of each element of the inferred $C$ are shown in Fig.~\ref{fig:Gaussian noise}. The inferred distributions are close to the ground truth costs which are indicated by blue dashed lines. This experiment demonstrates that our method successfully make accurate inferences using soft constraints $P_0(C)$, with the results comparable to hard constraints imposed by \citep{stuart2020inverse}. 

% C^g  =[[0.2604, 0.0521, 0.0104],
        % [0.0208, 0.2604, 0.0521],
        % [0.0625, 0.0208, 0.2604]]

% T^g = [[0.0952, 0.1168, 0.1214],
        % [0.1214, 0.0952, 0.1168],
        % [0.1168, 0.1214, 0.0952]]
        
% corruption noise = -0.0011

% noises = [ 0.0004, -0.0008,  0.0029,  0.0002, -0.0056, -0.0005,  0.0006, -0.0023,0.0041,  0.0076]

% d, e, f, g, h = 25., 5., 1.9, 3., 6.
% alpha = torch.tensor([[d, e, f],\
%                       [g, d, e],\
%                       [h, g, d]])


\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_11.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_12.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_13.png} 
    \end{tabular}
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_21.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_22.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_23.png} 
    \end{tabular}
    \begin{tabular}{c c c}
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_31.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_32.png} &
        \hspace{-8pt}\includegraphics[width=0.14\textwidth]{figs/Gaussian_noise_33.png} 
    \end{tabular}
    \caption{The KDE of each element of inferred cost $C$ with Gaussian noise on $t_{12}$. The blue dashed vertical lines indicate the ground truth cost $C^g$.
    }
    \label{fig:Gaussian noise}
\end{figure}

\textbf{Application on European Migration data.}
We apply PIOT to analyze European migration flow. %as proposed in \citep{stuart2020inverse}.
The observed migration data $T^g$ between 9 European countries for the period 2002- 2007 is shown in Fig.~\ref{fig:heatmap_migration_and_cost}.top-left \citep{raymer2013integrated}. 
% In this section we apply the PIOT method to investigate the cost function of the 9 selected countries from the European migration data.\citep{stuart2020inverse, raymer2013integrated} The observed migration coupling ($T^g$) is shown in the left of Fig.~\ref{fig:heatmap_migration_and_cost}. 
%We first study the effect of prior on the cost function. 
All results in this section are obtained by performing MetroMC with 10,000 burn-in steps, 10,000 samples with lags of 1000,
and the sum of cost matrix is assumed to be a constant, see details in Appendix~\ref{apd:sec:migration}.

First, we demonstrate the ability of PIOT by inferring the latent costs under various priors.
Three priors are considered with increasing strength:
(1) Fully uniform prior, Dirichlet with all $\alpha=1$; 
(2) Semi-uniform prior, diagonal $\alpha$=25 and 1 elsewhere, as the data does not consider migration within a country itself.
(3) Graph-geometrical prior, the diagonals are 25  and $\alpha$=1 if the two countries are directly connected and 1.5 if not, 
as comparison to the hard Graph-geometrical constraint imposed by \citep{stuart2020inverse}.
% (1) Uniform prior: Dirichlet with all $\alpha=1$; (2) Semi-uniform prior, diagonal $\alpha$=25 and 1 elsewhere;
% (3) Graph-geometrical prior, the diagonals are 25 and $\alpha$=1 if the two countries are directly connected and 1.5 if not. 
%The priors are stronger in increasing order. 



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/heatmap_migration_and_cost.png}
    \begin{tabular}{cc}
        \hspace{-8pt}\includegraphics[width=0.24\textwidth]{figs/scatter_cost_plan.png}
        \hspace{-8pt}\includegraphics[width=0.24\textwidth]{figs/cost_DE_to_FR.png}
    \end{tabular}
    \caption{(\textbf{Top-left.}) European migration data. 
    (\textbf{Top-right.}) Mean of the inferred cost using Prior 2.
    (\textbf{Bottom-left.}) Plots for logarithm of each migration data with its corresponding inferred cost mean.
     (\textbf{Bottom-right.}) The inferred cost distributions for DE$\rightarrow$FR under three priors.}
    \label{fig:heatmap_migration_and_cost}
\end{figure}

%The inverted color between two plots shows that PIOT captures the reciprocal relationship: lower costs 
%lead to higher migration numbers. 
Fig.~\ref{fig:heatmap_migration_and_cost}.top-right plots the mean of the inferred costs under the prior 2. 
Even with a weak prior, PIOT correctly captures the general reciprocal relation between coupling and cost,
lower costs lead to higher migration numbers, shown in Fig.~\ref{fig:heatmap_migration_and_cost}.bottom-left. 
Results for the other two priors are similar, see Appendix \ref{supsec: alg}. 
%Exceptions happen due to lots of reasons such as population of the country, immigration policy, and ticket prices, but these practical effects on the cost are out of our scope. 
%Before each simulation we put ones to the diagonal of $T^g$ so that $T^g \in \mathbf{R}_{+}$.  
%The results of the (5,7) matrix element (DE$\rightarrow$FR)
Fig.~\ref{fig:heatmap_migration_and_cost}.bottom-right plots the inferred costs from Germany to France (DE$\rightarrow$FR).
The implications of priors can be observed: the stronger the prior is, the narrower the inferred cost distribution is.
In particular, using prior 3, the mass is concentrated between 0 and 0.01 the same as in \citep{stuart2020inverse}, where hard graphical constraint on the cost is considered. 
%the distributions become more structural as 
% The weakest prior 1 has the widest distribution which is expected. 
% Prior 2 considers a soft constraint on the diagonal following the fact that no migration within each country, and thus the cost should be higher on the diagonal. Such constraint diminishes most of the cost of the other elements. Prior 3 is stronger where the geometrical relations are taken into account, therefore, the cost function becomes more structural. In fact, our result using prior 3 is comparable to the result of \citep{stuart2020inverse}, whereas they considered a much stronger constraint. 
% In Fig.~\ref{fig:heatmap_migration_and_cost} we plot the heat map of the ground truth coupling and the mean of the inferred cost function using prior 2. Our model correctly captures the general reciprocal relation between coupling and cost. Exceptions happen due to lots of reasons such as population of the country, immigration policy, and ticket prices, but these practical effects on the cost are out of our scope. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figs/cost_DE_to_FR.png}

%     \caption{The inferred cost distributions for DE$\rightarrow$FR.}
%     \label{fig:cost_DE_to_FR}
% \end{figure}

%An upper limit = 0.012 for the values is set to increase resolution on low cost areas.

%Comparison between the predicted coupling, $T^p$, with the ground truth coupling, $T^g$. $\Delta=(T^p-T^g)/T^g$. \textbf{(Left)} Corresponding element is corrupted by a 4\% Gaussian noise. \textbf{(Right)} Value of the corresponding element is missing. 
\begin{table}[h!]
\caption{Comparison between the predicted coupling, $T^p$, with the ground truth coupling, $T^g$. $\Delta=(T^p-T^g)/\overline{T}^g$. 
Corresponding element is corrupted by a 4\% Gaussian noise on the left column, and missing on the right column. }
\label{table:missing_value}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c | ccc | ccc}
\toprule
& & Noise & & \multicolumn{3}{c}{Missing value} \\
%& (4,5)  & (3,6) & (5,7) & (7,3) & (2,6) & (5,3) \\
& (3,6) & (4,5) & (5,7) & (3,6) & (4,5) & (5,7) \\
\midrule
% $T^g$ & 6635 & 452  & 16560 & 8760 & 440  & 19690 \\
% $T^p$ & 6593 & 454  & 16515 & 8993 & 3844 & 14824 \\
$T^g$ & 452 & 6635  & 16560 & 452 & 6635  & 16560 \\
$T^p$ & 454 & 6593  & 16515 & 3699 & 7462 & 12349 \\
\midrule
% $|\Delta|$ & 0.8\% & 0.4\% & 0.3\% &  &  & \\
$|\Delta|$ & .45\% & .87\% & .25\% & 26\% & 6.6\% & 34\%\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.3in
\end{table}

% We start with a Toeplitz ground truth cost function $C^g$ and obtain an OT plan, $T^g$, with $C^g$ and uniform $\mu, \nu$. A random Gaussian noise $\epsilon \sim \mathcal{N}(0, 0.004^2)$, about 4\% of the average value of $T$, is added to $t^g_{1,2}$, and the corrupted plan $T=T^g+\epsilon$. We then infer the posterior distribution $P(C|T)$. We put a $\mathbf{P}_1$ prior on $C$ with the hyperparameters follows toeplitz matrix format. 
% %The prior of $P_0(C)$ is assumed to be toeplitz Dirichlet, where the matrix of the Dirichlet parameters is diagonal-constant and $\sum_{i,j}{C_{i,j}}=1$. 
% Inference is done by first generating 10 random numbers $\epsilon_i^{*}\sim \mathcal{N}(0, 0.004^2)$ and apply the noise on $t_{12}$ to get $T_i^{*}=T+\epsilon_i^{*}$. Then, we utilize MetroMC on every $T_i^{*}$ to obtain $P(C|T_i^{*}$), and finally $P(C|T)\approx\sum_i P(C|T_i^{*})$. 


Next, we test PIOT's performance on noisy data. 
%The noisy coupling $T$ is obtained by c
We corrupting an element of $T^g$ with a Gaussian noise to obtain $T$, 
whose standard deviation is set to be 4\% of the value. 
With prior~2, inference on cost distributions is done in the same fashion as in 
Fig.~\ref{fig:Gaussian noise}. 
We then apply EOT on the cost matrix formed by means of inferred distributions with the observed marginals, 
to predict the true migration data.
%We infer the plan by applying EOT to the estimated cost %\hl{E?}OT on 
% $C^M_{(i,j)}$ with the observed marginals to predict the migration number $T^p_{(i,j)}$. 
% %Our predictions are within 1\% to the ground truth values. 
Left of Table~\ref{table:missing_value} shows the results when noise occurs at 
$T^g_{36},T^g_{45}, T^g_{57}$. Our predictions $T^p$ are within 1\% to 
the mean of prior on the ground truth, denoted by $\overline{T}^g$ as shown in the third row. 

% Next, we study the effect of noise on $T^g$. We assume the $(i,j)$-th matrix elements shown in the left of table~\ref{table:missing_value} are corrupted by a Gaussian noise with $\sigma_{i,j}$ equals to 4\% of the value. We generate 10 random numbers $x_{i,j} \in N(0,\sigma_{i,j})$, and each $x_{(i,j)}$ is added to the corrupted element to obtain the corrupted plan. MetroMC is performed to obtain 10,000 inferred cost functions. 
% %We do 10,000 burn-ins and take 10,000 samples with lags of 1,000 for each noise. 
% We take the mean value of all the samples, $C^M_{(i,j)} = \sum_{k}C^(k)_{(i,j)}$, 
%where $k$ numerates each inferred cost function. We infer the plan by applying EOT to the estimated cost %\hl{E?}OT on 
% $C^M_{(i,j)}$ with the observed marginals to predict the migration number $T^p_{(i,j)}$. 
% %Our predictions are within 1\% to the ground truth values. 


Finally, we explore PIOT's capacity on recovering missing data.
%Assuming incomplete observation on $T^g$,
We fill in the missing element with 100 samples ranging uniformly over $[100, 25000)$.
With semi-uniform prior, we estimate the cost and perform EOT as described above.
Right column of Table~\ref{table:missing_value} shows that %the results when $T^g_{36},T^g_{45}, T^g_{57}$ are missing.
PIOT successfully recovered the ground truth with estimation error less than 35\% of the prior mean.
%The predictions are ranked the same as the ground truth %\pw{what shall we say here}.
%We suspect the large difference on $\Delta_{36}$ is due to the small magnitude of $T^g_{36}$ and the uniform prior .

% Finally, we predict the value of $T^g$ where the matrix element is missing. We fill in the missing element with 100 numbers ranging uniformly from 100 to 25000, and for each we perform the MetroMC to obtain 10,000 samples. Then, we estimate the cost and perform EOT to obtain $T^p_{(i,j)}$ as described above (Table~\ref{table:missing_value}, right). 
%The results are shown in the right of table~\ref{table:missing_value}. 
%The predicted numbers appear to be closer to the actual migration number than the average of the wild guesses, 12550. \pat{huh? FIXME!}





%Priors used in order: (1) Fully uniform prior. (2) Semi-uniform prior. (3) Graph-geometrical prior.

% \begin{figure}[h!]
%     \centering
%     \begin{tabular}{c c}
%     \includegraphics[width=0.225\textwidth]{figs/cost_pred_4_5.png}
%     \includegraphics[width=0.225\textwidth]{figs/heatmap_noise_mat_diff.png}
%     \end{tabular}

%     \caption{The results where the (4,5)-element of the coupling is corrupted by a 4\% noise.  \textbf{(Left)} The PDF of the predicted cost $C^p(4,5)$ (CZ$\rightarrow$DE). \textbf{(Right)} The difference from the ground truth coupling to the predicted coupling, $T^p$. 
%     }
%     \label{fig:migration_noise}
% \end{figure}




%\pw{what plot for real data?}

==> ICML-sumission/4-conclusion_ICML.tex <==
\section{Conclusion}
%In conclusion, we presented an analysis of probabilistic Inverse Optimal Transport which infers latent costs from observed couplings. 
%In contrast with prior work on IOT, we consider the geometric foundations inherited from Sinkhorn scaling of entropy-regularized Optimal Transport. We analyze the support of the cost matrices associated with an observed coupling, the implications of prior distributions on costs, and introduce MCMC algorithms for posterior inference. Our models perform well on synthesis data and the results are comparable to previous works. \wt{Do we need to include a short discussion on the limitations of our model?}
We have generalized prior treatments of IOT by defining and studying the underlying support manifold and associated inference problems. 
We provided MCMC methods for inference over general priors on discrete costs and induced kernels. 
Simulations illustrate underlying geometric structure and demonstrate the feasibility of the inference. 
%\pat{FIXME: one last thing?}

==> ICML-sumission/customized_command_ICML.tex <==
% \usepackage[utf8]{inputenc}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{fullpage}

% \usepackage{graphicx}
% \usepackage{color,soul}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amstext}
% \usepackage{mathrsfs}
% \usepackage{amssymb}
% \usepackage{bm}
% \usepackage{pictexwd,dcpic}
% \usepackage{enumitem}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{empheq,etoolbox}
% Update display of subequation numbering (Xy) > (X.y)
% \usepackage{cases}
% \usepackage{cleveref} 

\usepackage[font=small,skip=0pt]{caption}

% \usepackage{tikz}
% \usetikzlibrary{calc,intersections,through}
% \tikzset{
%     partial ellipse/.style args={#1:#2:#3}{
%         insert path={+ (#1:#3) arc (#1:#2:#3)}
%     }
% }

% %\usepackage{pgfplots}

\newcommand{\pat}[1]{\textcolor[rgb]{.7,0,.2}{#1}}
\newcommand{\pw}[1]{\textcolor[rgb]{0.6,0.6,0}{#1}}
\newcommand{\wt}[1]{\textcolor[rgb]{0,0,0.7}{#1}}
%theorem styles



\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
\def\rep@title{#2 \ref{##1}}%
\begin{rep@theorem}}%
{\end{rep@theorem}}}
\makeatother

% \newtheorem{thm}{Theorem}[section]
% \newtheorem*{thm*}{Theorem}
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{conj}[thm]{Conjecture}
% \newtheorem{cor}[thm]{Corollary}
% \newtheorem{prop}[thm]{Proposition}

% \newreptheorem{lemma}{Lemma}
% \newreptheorem{prop}{Proposition}
% \newreptheorem{thm}{Theorem}
% \newreptheorem{cor}{Corollary}

\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{theorem}{Theorem}
\newreptheorem{corollary}{Corollary}

% \newtheorem{exercise}{Exercise}
% \newtheorem{question}{Question}


% \theoremstyle{definition}
% \newtheorem{definition}[thm]{Definition}
% \newtheorem*{definition*}{Definition}
% \newtheorem{problem}[thm]{Problem}
% \newtheorem{remark}[thm]{Remark}
% \newtheorem{example}[thm]{Example}
% \newtheorem*{example*}{Example}
% \newtheorem{examples}[thm]{Examples}
% \newtheorem{notation}[thm]{Notation}
% \newtheorem*{framework*}{Unifying OT Framework}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

% \newtheorem{theorem}{Theorem}[section]
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{note}[theorem]{Note}
% \newtheorem{remark}[theorem]{Remark}



% Notations
\newcommand{\D}{\mathcal{D}} % data space
\newcommand{\hp}{\mathcal{H}} % hypothesis space
\newcommand{\R}{\mathbb{R}} % all real numbers.
\newcommand{\e}{\epsilon} % a small parameter
\newcommand{\E}{\mathbb{E}}%  expectation
\newcommand{\kl}{\text{KL}}%  
\newcommand{\diag}{\text{diag}}%  
\newcommand{\CR}{\text{CR}}%  
\newcommand{\parallelsum}{\mathbin{\!/\mkern-5mu/\!}}

% \usepackage[
% backend=biber,
% style=alphabetic,
% sorting=ynt
% ]{biblatex}


==> ICML-sumission/supp_algs_ICML.tex <==
\section{Additional details of experiments} \label{supsec: alg}


\subsection{Auto-correlation function.} \label{apd:sec:autocorrelation}

To monitor the efficiency of our MC methods, we compute the auto-correlation function during the burn-in phase and choose the lags accordingly.

The auto-correlation function is defined as
\begin{equation}
R(t)=\frac{1}{(N-t)\sigma^2}\sum_{l=1}^{N-t}\sum_{i,j}(K_{i,j}^{(l)}-\bar{K}_{i,j})\cdot(K^{(l+t)}_{i,j}-\bar{K}_{i,j}),
\label{eq:autocorrelation}
\end{equation}
where $N$ is the total number of samples generated, (i,j) runs over all indices of the matrices $K$, $\bar{K}$ is the mean averaging over all the samples, and $\sigma_K^2=\sum_{i,j}\sigma_{K,i,j}^2$ is the variance. 

\subsection{Re-normalization of $T$ for MetroMC over prior $\mathbf{P}_1$.}

For using this method, not every random $T$ satisfies the condition such that $C^{(0)}=-\text{ln}(K^{(0)})=-\text{ln}(T)$ lies on the support of the posterior, therefore, we need to re-normalize $T$ so that $C^{(0)}-\text{ln}[T/F(T)]$ is on the support. $F(T)$ is defined as
\begin{equation}\label{eq:renormal_T}
    F(T) = \text{exp}\left({\frac{1+\sum_{i=1}^{m}\sum_{j=1}^{n}\text{log}(T_{i,j})}{m*n}}\right).
\end{equation}

\subsection{MHMC on uniform matrix.} \label{apd:sec:MHMC}
In this section, we validate our MHMC algorithm by apply it to an uniform $T$, i.e $T_{m,n}=1/m$ 
under prior $\mathbf{P}_2$.
%on uniform matrices, e.g. $T_{m,n}=1/m$ for the column-wise Dirichlet prior case. 
The cross-ratios of $T$ are all 1 and stay the same for all inferred sample $K^{(i)}$. 
Thus, each $K^{(i)}$ has same copies of $n$ columns. 
We compare posterior sampled by MHMC to a 
$m$-dimensional uniform symmetric Dirichlet distribution generated by the SciPy package \citep{2020SciPy-NMeth}.  


% Fig.~\ref{fig:uniform_3x3} shows the results the 3x3 case.
% are the same for every element. We choose $\alpha=1$ for the Dirichlet prior, 
% $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. 
% We run for 10,000 burn-in steps and take 10,000 samples 
% with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. 
% We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps.
% Also, the running averages of the row sums are stable at taking 10,000 samples, 
% which means 10,000 samples can effectively represent the posterior distribution. 

We perform our MHMC algorithm on a $3\times 3$ uniform matrix with prior $P_2$ and the Dirichlet concentration parameter $\alpha$ are the same for every element. We choose $\alpha=1$ for the Dirichlet parameter, $\sigma_0=0.5$, $\gamma=3$, and $\delta=1.0$. We run for 10,000 burn-in steps and take 10,000 samples with lags of 100. The result is shown in Fig.~\ref{fig:uniform_3x3}. We choose the lag by observing the auto-correlation function in the burn in, where the chain becomes uncorrelated after $\sim$ 100 steps. Also, the running averages of the row sums are stable at taking 10,000 samples, which means 10,000 samples can effectively represent the posterior distribution. 

The posterior distribution (Shown in top right of Fig.~\ref{fig:uniform_3x3}.) is compared to the distribution $P(K|T)$ of three-dimensional vectors generated by Dirichlet vector sampler \citep{2020SciPy-NMeth} with symmetric $\alpha=1$ in top left of  Fig.~\ref{fig:uniform_3x3}. The results are comparable, which suggests that our MHMC method is able to generate distributions which well represent the support of the posterior distributions.


\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
        \hspace{-4pt}\includegraphics[width=0.45\textwidth]{figs/dirichlet_3.png}
        \hspace{-6pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3.png}
    \end{tabular}
    \begin{tabular}{c c}
        \hspace{-4pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3_autocorr.png}
        \hspace{-6pt}\includegraphics[width=0.45\textwidth]{figs/uniform_posterior_3x3_running_avg.png}
    \end{tabular}
    
    \caption{\textbf{(Top left.)} The distributions of each component of three-dimensional Dirichlet vectors with symmetric $\alpha=1$ generated using SciPy package. \textbf{(Top right.)} The distributions of each component of the first column of $P(K|T)$ sampled by the MHMC method. \textbf{(Lower left.)} The auto-correlation function of the MHMC simulation. The black dashed lines indicate the range [$-1/e$, $1/e$]. \textbf{(Lower right.)} The running average of the row sums of the MHMC simulation.
    }
    \label{fig:uniform_3x3}
\end{figure}

\subsection{MetroMC on uniform matrix.}
We test MetroMC on 3x3 uniform $T$, where $T_{i,j}=1/(m*n)$, and assume the prior $\mathbf{P}_1$ is put on $C$. We take $K^{(0)}=T/F(T)$.
For each MC iteration we sample $m+n-1$ Gaussian random numbers with standard deviations of 0.02 for the diagonal matrices $D^r$ and $D^c$ satisfying the condition 
\begin{equation}
\sum_{i,j}\text{ln}(d^r_{i})+\text{ln}(d^c_j)=0. 
\label{eq:condition_bounded_noises}
\end{equation}
We burn in 10,000 steps and take 100,000 samples with 100 lags in between. The Gaussian Kernel density estimation (KDE) of each component of $P(C|T)$ is demonstrated in Fig.~\ref{fig:uniform_3x3_2}. We use bandwidths of 0.05 for all the Gaussian KDE in this article. There are a few notable features. First, we assume a Dirichlet prior on the whole $C$ matrix, the distributions will be smaller at large values because each large value will suppress the value of the other elements. Second, since we have cross-ratio = 1 everywhere in $T$ and prior $\mathbf{P}_1$ on $C$, there will not be a single element with value close to one. Otherwise, the cross-ratio involving that element could never be 1 anymore. Also, for the same reason all distributions should be similar.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.50\textwidth]{figs/pdf_unifrm_T_3x3.png}
    \begin{tabular}{c c}
        \includegraphics[width=0.45\textwidth]{figs/autocor_uniform_T_P2.png}
        \includegraphics[width=0.45\textwidth]{figs/running_average_uniform_T_P2.png}
    \end{tabular}
    \caption{\textbf{(Top.)} The distribution of each matrix element of $P(C|T)$ with a uniform $T$ and a prior $\mathbf{P}_1$ over $C$ matrix. \textbf{(Bottom left.)} The autocorrelation function of the simulation. \textbf{(Bottom right.)} The running averages of the row sums.}
    \label{fig:uniform_3x3_2}
\end{figure}


\subsection{Visualizing $\text{supp}[P(K|T)]$ with incomplete observations.}\label{apd:sec:missing_value}
Fig.~\ref{fig:missing_element_T} illustrates the 
$\text{supp}[P(K|T)]$ for a $3\times 3$ observation $T$ with $t_{31}$ missing under prior $\mathbf{P}_2$. % \hl{FIXME}
%$T = [[5.84, 4.32, 4.10],[5.90, 9.00, 4.29],[t_{31}, 5.49, 7.18]]$ is constructed by sampling each element uniformly from $[0,10]$.
Columns of three sampled $K \in \text{supp}[P(K|T)]$ are plotted in three colored copies $\Delta_2$ as shown.
Here, three $\mathbf{k}_2$ are sampled uniformly from the middle $\Delta_2$. The uniquely determined $\mathbf{k}_3$ are shown in the right $\Delta_2$.
The corresponding set for $\mathbf{k}_1$ ($\mathcal{K}_1$) is plotted in the left $\Delta_2$.
$\mathcal{K}_1$ is obtained by uniformly sample a thousand $t_{31}$ from $[0,10]$. 
Each $t_{31}$ uniquely determines a $\mathbf{k}_1$.
As explained in Corollary~\ref{cor:missing_element}, 
each $\mathcal{K}_1$ forms a line segments. 
The slope of each line is determined by $T$'s cross ratios. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/missing_value_2.png}
    \caption{Visualization of $\text{supp}[P(K|T)]$ for a $3\times 3$ observed $T$ with $t_{31}$ missing.
    Three sampled $K \in \text{supp}[P(K|T)]$ are shown here with 
    each column is plotted in a copy of $\Delta_2$ as shown.
    Colored dots in the middle $\Delta_2$ represents uniformly sampled $\mathbf{k}_2$'s. 
    The uniquely determined $\mathbf{k}_3$'s are shown on the right, 
    the set $\mathcal{K}_1$ for the corresponding $\mathbf{k}_1$'s is shown on the left.}
    \label{fig:missing_element_T}
\end{figure}

\subsection{Supporting plots for the MetroMC method on noisy T.}

In this section, we provide data for diagnostics of the MetroMC simulations on the noise models in section 5 of the main text.

\textbf{Bounded noise on observed plan.} The autocorrelation function and the running averages of row sums of the samples for each noise are plotted in Fig.~\ref{fig:MC_details_bounded_noise}. In the simulation we set 100 for the lags by observing that the chains become uncorrelated after $\sim$ 100 steps for all cases. We take 100,000 samples in total for all cases since the running averages are stable at (or before) 100,000 MC steps, which means the samples reaches a stationary distribution.

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.44\textwidth]{figs/autocor_bounded_noise.png}
            \put(-30,125){\textbf{a.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_1.png}
            \put(-30,125){\textbf{b.}}
        \end{picture}

    \end{tabular}
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_2.png}
            \put(-30,125){\textbf{c.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_3.png}
            \put(-30,125){\textbf{d.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c}
        \begin{picture}(140,140)(80,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_4.png}
            \put(-30,125){\textbf{e.}}
        \end{picture}
        \begin{picture}(140,140)(0,0)% width and height of the picture
            \includegraphics[width=0.45\textwidth]{figs/running_average_bounded_noise_5.png}
            \put(-30,125){\textbf{f.}}
        \end{picture}
    \end{tabular}
    \caption{MC diagnostics for the Bounded noise example. \textbf{(a.)} The autocorrelation funciton for all noises. \textbf{(b.)-(f.)} The running averages of row sums of the samples for noises -0.01, -0.005, 0.0, 0.005, and 0.01 added to $t_{11}$, respectively.
    }
    \label{fig:MC_details_bounded_noise}
\end{figure}

\textbf{Gaussian noise on observed plan.}
The autocorrelation function and the running averages of row sums of the samples for the 10 Gaussian noises are plotted in Fig.~\ref{fig:MC_details_running_average_gaussian_noise}. We set 200 for the lags since the chains become uncorrelated after $\sim$ 180 steps for all cases. 10,000 samples are taken for all cases since the running averages of the row sums are stable at 10,000 MC steps.

\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c c c}
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/autocor_gaussian_noise.png}
            \put(-30,80){\textbf{a.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_1.png}
            \put(-30,30){\textbf{b.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_2.png}
            \put(-30,30){\textbf{c.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}   
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_3.png}
            \put(-30,30){\textbf{d.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_4.png}
            \put(-30,30){\textbf{e.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_5.png}
        \put(-30,30){\textbf{f.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}  
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_6.png}
            \put(-30,30){\textbf{g.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_7.png}
            \put(-30,30){\textbf{h.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_8.png} 
            \put(-30,30){\textbf{i.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}  
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_9.png}
        \put(-30,30){\textbf{j.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.32\textwidth]{figs/running_average_gaussian_noise_10.png}      
            \put(-30,30){\textbf{k.}}
        \end{picture}
    \end{tabular}

    \caption{MC diagnostics for the Bounded noise example. \textbf{(a.)} The autocorrelation function for all noises. \textbf{(b.)-(k.)} The running averages of row sums of the samples for the 10 random Gaussian noises added to $t_{12}$.
    }
    \label{fig:MC_details_running_average_gaussian_noise}
\end{figure}

\newpage

\subsection{Matrices.}\label{apd:sec:matrices}

We list the matrices used in section 5: \textbf{Simulations on synthetic data} below.

The three $T$ matrices in Fig.~\ref{fig:2x2_subspace} are

\begin{align*}
T_a = 
\begin{bmatrix}
0.3096 & 0.3785 & 0.0544 & 0.2575 \\
0.2522 & 0.3203 & 0.1860 & 0.2415 \\
0.4318 & 0.1433 & 0.4196 & 0.0053 \\
0.0064 & 0.1579 & 0.3400 & 0.4957 \\
\end{bmatrix},
\end{align*}

\begin{align*}
T_b = 
\begin{bmatrix}
0.2532 & 0.4143 & 0.2894 & 0.0431\\
0.1925 & 0.0548 & 0.0958 & 0.6569\\
0.4459 & 0.0905 & 0.3480 & 0.1156\\
0.1083 & 0.4404 & 0.2669 & 0.1844
\end{bmatrix},
\end{align*}

\begin{align*}
T_c = 
\begin{bmatrix}
0.4790 & 0.0994 & 0.0838 & 0.3378\\
0.1343 & 0.1514 & 0.1920 & 0.5224\\
0.1678 & 0.6182 & 0.1963 & 0.0177\\
0.2189 & 0.1310 & 0.5279 & 0.1222
\end{bmatrix}.
\end{align*}

The matrix $T$ in Fig.~\ref{fig:missing_element_T} is
\begin{align*}
T = 
\begin{bmatrix}
0.4583 & 0.2297 & 0.2633\\
0.4631 & 0.4785 & 0.2755\\
0.0785 & 0.2919 & 0.4611
\end{bmatrix}.
\end{align*}


The matrices $T$ in Fig.~\ref{fig:sample_supp} are

\begin{align*}
T_1 = 
\begin{bmatrix}
0.1104 & 0.0684 & 0.1545 \\
0.0505 & 0.2401 & 0.0428 \\
0.1725 & 0.0249 & 0.1360
\end{bmatrix},
\end{align*}

\begin{align*}
T_2 = 
\begin{bmatrix}
0.0950 & 0.1100 & 0.1283\\
0.1155 & 0.0343 & 0.1835\\
0.1228 & 0.1890 & 0.0215
\end{bmatrix},
\end{align*}

\begin{align*}
T_3 =
\begin{bmatrix}
0.1053 & 0.1193 & 0.1088\\
0.2148 & 0.0090 & 0.1096\\
0.0133 & 0.2051 & 0.1150
\end{bmatrix}.
\end{align*}

The matrix $T$ for the bounded noise case is

\begin{align*}
T =
\begin{bmatrix}
0.1067 & 0.1141 & 0.1125\\
0.1175 & 0.1052 & 0.1106\\
0.1092 & 0.1139 & 0.1102
\end{bmatrix}.
\end{align*}

The ground truth $C^g$ in the Gaussian noise example is
\begin{align*}
C^g = 
\begin{bmatrix}
0.2604 & 0.0521 & 0.0104\\
0.0208 & 0.2604 & 0.0521\\
0.0625 & 0.0208 & 0.2604
\end{bmatrix},
\end{align*}
and the hyperparameter matrix for the prior is
\begin{align*}
\alpha =
\begin{bmatrix}
25.0  & 5.0     & 1.9\\
3.0   & 25.0    & 5.0\\
6.0   & 3.0     & 25.0
\end{bmatrix}.
\end{align*}

\subsection{Details of the MCMC simulations on European migration data.}\label{apd:sec:migration}

For this part of simulations we consider the migration flows\citep{raymer2013integrated} between the following 9 countries: Austria (AT), Belgium (BE), Switzerland (CH), Czech Republic (CZ), Germany (DE), Denmark (DK), France (FR), Luxembourg (LU) and Netherlands (NL). The migration flow matrix is shown in Fig.~\ref{fig:heatmap_migration_only}.

We utilize MetroMC method to infer the cost functions. In this section we assume that the sum of cost function is a constant. We use $\sum_{i,j}C_{i,j}=\sum_{i,j}\lambda C_{i,j}'$=320 and put Dirichlet priors on $C'$ so that there exists cost functions following the Dirichlet priors can be inferred from the ground truth plan. For each MCMC simulation using the three different Dirichlet priors we burn-in 10,000 steps and then take 10,000 samples with lags of 1,000 between. The standard deviations of the independent Gaussian random numbers (Centered at 0.) in each MCMC iteration are 0.1, 0.1, and 0.07 for prior (1), (2), and (3), respectively. The acceptance rate for the MCMC simulations are 0.58-0.68. The autocorrelation function and the running average of each simulation are shown in Fig.~\ref{fig:MC_details_EU_migration}. 1,000 steps are enough to de-correlate samples and 10,000 samples are able to reach convergence. The kernel density estimations (KDE) of each matrix element of the inferred cost functions are shown in Fig.~\ref{fig:EU_migration_cost}. The mean of each element of the cost for the three priors are shown in Fig.~\ref{fig:heatmap_mean_cost}.

For the noisy simulations on the EU migration flow we first generate a noise ($\epsilon$) which is 4\% of the value of $T^g_{(i,j)}$ and add it to $T^g_{(i,j)}$. Then, we sample ten Gaussian random numbers centered at 0 having a standard deviation equal to 4\% of $T^g_{(i,j)}$. The generated numbers are shown in table \ref{table:Gaussian_noises}. The MetroMC method is used for cost function inferences. In each Monte Carlo step we sample random variables $x \in \mathcal{N}(0,0.1^2)$ for the diagonal matrices $D^r$ and $D^c$. For each MCMC simulation we burn-in 10,000 steps and take 10,000 samples with a lag of 1,000 steps in between samples. The acceptance rates are 0.5-0.7. Once we infer the cost functions we compute the mean of them, $C^M$. Afterwards, forward OT simulation on $C^M$ using the observed marginals is performed to obtain the predicted coupling, $T^p$. The results are shown in table~\ref{table:missing_value}.

We follow the same procedure and use the same parameters for the MCMC simulations of predicting the missing values, only instead of ten random Gaussian samples we take 100 samples uniformly in range of [100, 25000) to fill the missing value.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/heatmap_migration_only.png}
    \caption{European migration flow matrix between the selected 9 countries. }
    \label{fig:heatmap_migration_only}
\end{figure}

\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c c c}
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/correlation_p1.png}
            \put(-30,80){\textbf{a.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/correlation_p2.png}
            \put(-30,80){\textbf{b.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/correlation_p3.png}
            \put(-30,80){\textbf{c.}}
        \end{picture}
    \end{tabular}
    \begin{tabular}{c c c}   
        \begin{picture}(140,100)(20,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/MC_convergence_p1.png}
            \put(-30,80){\textbf{d.}}
        \end{picture}
        \begin{picture}(140,100)(10,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/MC_convergence_p2.png}
            \put(-30,80){\textbf{e.}}
        \end{picture}
        \begin{picture}(140,100)(0,0)% width and height of the picture
            \includegraphics[width=0.31\textwidth]{figs/MC_convergence_p3.png}
        \put(-30,80){\textbf{f.}}
        \end{picture}
    \end{tabular}
    

    \caption{MC diagnostics for the European migration flow data. \textbf{(a.)-(c.)} are the autocorrelation function for using prior 1, 2, and 3, respectively. \textbf{(d.)-(f.)} are the running averages of row sums of the samples for using prior 1, 2, and 3.
    }
    \label{fig:MC_details_EU_migration}
\end{figure}

\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_1_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_2_9.png}
    \end{tabular}    
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_3_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_4_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_5_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_6_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_7_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_8_9.png}
    \end{tabular}
    \begin{tabular}{c c c c c c c c c}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_1.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_2.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_3.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_4.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_5.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_6.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_7.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_8.png}
        \includegraphics[width=0.105\textwidth]{figs/EU_cost/C_9_9.png}
    \end{tabular}
    \caption{The KDE of the inferred cost functions from the EU migration flow coupling. All $9\times 9 $ matrix elements are shown in order. The red curves are for prior (1), green for (2), and blue for (3).
    }
    \label{fig:EU_migration_cost}
\end{figure}

\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c c c}
        \includegraphics[width=0.3\textwidth]{figs/heatmap_mean_cost_1.png}
        \includegraphics[width=0.3\textwidth]{figs/heatmap_mean_cost_2.png}
        \includegraphics[width=0.3\textwidth]{figs/heatmap_mean_cost_3.png}

    \end{tabular}
    
    \caption{The heatmaps of the mean of the inferred cost functions using \textbf{(left)} prior 1,  \textbf{(middle)} prior 2, and \textbf{(right)} prior 3.
    }
    \label{fig:heatmap_mean_cost}
\end{figure}


\begin{table}[h!]
\caption{Sampled Gaussian noises. }
\label{table:Gaussian_noises}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c | c | c | cccccccccc}
\toprule
(i,j) & $T^g_{(i,j)}$ & $\epsilon$ & \multicolumn{10}{c}{Noises} \\
\midrule
(3,6) & 452 & 3 & 7 & -2 & 5 & 22 & -22 & -6 & 3 & 6 & -24 & 5 \\
(4,5) & 6635 & -131 & -404 & 763 & -118 & -315 & 7 & 422 & -16 & 66 &-145 & 79 \\
(5,7) & 16560 & -243 & 785 & 205 & 269 & 525 & 678 & -164 & 217 & -180 & -379 & -459 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.3in
\end{table}







==> ICML-sumission/supp_proofs_ICML.tex <==
\section{Examples, Definitions and Proofs} \label{apdx:proofs}


\begin{example}\label{eg: sk}
Let $\mu =\nu=(\frac{3}{8},\frac{5}{8})$, 
$\tiny C = \begin{pmatrix} \ln 1 & \ln 2 \\
 \ln 4 & \ln 1 \end{pmatrix}$. 
For $\lambda=1$, we may obtain $T$ by applying SK scaling on
$\tiny K^{\lambda} = e^{-C} = \begin{pmatrix} 1 & 1/2\\ 1/4 & 1 \end{pmatrix}$:
first, row normalize $K^{\lambda} $ with respect to $\mu$ results:
$\tiny K_1^{\lambda} =  \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
Then column normalization of $ K_1^{\lambda}$ with respect to $\nu$ outputs 
$\tiny K_2^{\lambda} = \begin{pmatrix} 1/4 & 1/8\\ 1/8 & 1/2 \end{pmatrix}$. 
As $K_1^{\lambda}= K_2^{\lambda}$, the SK scaling has converged with $T = K_1^{\lambda}$.
In general, multiple iterations may be required to reach the limit. %\pw{may move to apdx}
\end{example} 


\begin{repproposition}{prop:piot}
When $T = T^*$, $ P(C|T)$ is supported on the intersection between $\Phi^{-1} (T)$ and the domain of $ P_0(C)$, moreover, we have that
$\displaystyle P(C|T) = \frac{P_0(C)}{\int_{\Phi^{-1} (T)} P_0(C) \text{d} C}$.
\end{repproposition}

\begin{proof}
When $T = T^*$, Eq~\eqref{eq: PIOT} and Eq~\eqref{eq: bayes} imply that:
$P(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$. $P(T) >0$ is the normalizing constant, 
so $\text{Supp}[P(C|T)] = \text{Supp}[P(T|C)] \cap \text{Domain}[P_0(C)] $.
Note that $P(T|C) P_0(C) = P_0(C)$ for $C \in \Phi^{-1}(T)$, otherwise $P(T|C) P_0(C) =0$.
Hence the proposition holds.
\end{proof}




\begin{repproposition}{prop:DAD}
Let $T$ be a non-negative optimal coupling of dimension $m\times n$. $C \in \Phi^{-1} (T)$ if and only if for every $\epsilon > 0$,
there exist two positive diagonal matrices $D^r = \diag\{d^r_1, \dots, d^r_m\}$ and $D^c =\diag \{d^c_1,\dots, d^c_n\}$ such that: 
$\displaystyle |D^r K D^c - T| < \epsilon$, where $K = e^{-C}$ and $|\cdot|$ is the $L^1$ norm. 
In particular, if $T$ is a positive matrix, then $C \in \Phi^{-1} (T)$ 
if and only if there exist positive diagonal matrices $D^r,D^c$ such that $D^r K D^c = T$, i.e.
\begin{equation*}
\Phi^{-1} (T) = \{C| \exists  D^{r} \text{ and } D^{c} \text{ s.t. } K = D^rTD^c\}    
\end{equation*}
\end{repproposition}

\begin{proof}
Let the row and column of marginals of $T$ be $\mu$ and $\nu$.
Then $C \in \Phi^{-1} (T)$ if and only if $(\mu, \nu)$-Sinkhorn scaling of $K$ converges to $T$ in $L^1$ norm 
(for finite matrices, convergence in all $L^k$ norms are equivalent).
Notice that a row (column) normalization step in the Sinkhorn scaling is equivalent to a left(right) matrix multiplication of a positive diagonal matrix. 
Indeed, let $K_0 = {K}$, $\mathbf{r}_0 = K_0 \mathbf{I}_n$ (vector for row sums of $K_0$), $D_0^{r} = \diag(\mu /\mathbf{r}_0)$.
Here $\mu /\mathbf{r}_0$ represents element-wise division. 
Let $K'_0$ be the matrix obtained by row normalization of $K_0$ with respect to $\mu$. Then $K'_0 = D_0^{r} K_0$.
Similarly, let $K_1$ be the matrix obtained by column normalization of $K'_0$ with respect to $\nu$.
Then $K_1 = K'_0 D_0^c$, where $D_0^c = \diag (\nu/ \mathbf{I}_m^T K'_0)$.
Iteratively, we have $K_s = \Pi_{i=1}^{s} D_i^r \cdot K_0 \cdot \Pi_{i=1}^{s} D_i^c$.

The \textbf{only if direction} [${C} \in \Phi^{-1} (T) \Longrightarrow$ existence of $D^r$ and $D^c$ for any $\epsilon$]: 
${C} \in \Phi^{-1} (T) \Longrightarrow $ $(\mu, \nu)$-Sinkhorn scaling of ${K}$ converges to $T$
$\Longrightarrow $, for any $\epsilon >0$, there exists $N>0$ such that for any $s>N$, $|K_s - T| < \epsilon$, 
where $K_s = \Pi_{i=1}^{s} D_i^r \cdot {K} \cdot \Pi_{i=1}^{s} D_i^c$.
Let $D^r = \Pi_{i=1}^{s} D_i^r$, $D^c = \Pi_{i=1}^{s} D_i^c$, the only if direction is complete.

The \textbf{if direction} [existence of $D^r$ and $D^c$ for any $\epsilon$ $\Longrightarrow$ ${C} \in \Phi^{-1} (T)$]: 
Let the limit of $(\mu, \nu)$-Sinkhorn scaling on ${K}$ be $K^{*}$.
Hence $K^{*}$ and $T$ have the same marginals and pattern. 
According to Lemma~A.3 of \citep{pei2019generalizing}, $K^{*}$ and $T$ are diagonally equivalent. 
Further by Proposition~1 of \citep{pretzel1980convergence} $K^{*} = T$.


In particular, when $T$ is a positive matrix, ${K}$ must also be a positive matrix.
Then $T$ and ${K}$ have the same pattern. 
$T = \lim_{s\to \infty} \Pi_{i=1}^{s} D_i^r \cdot {K} \cdot \Pi_{i=1}^{s} D_i^c$
implies that $\lim_{s\to \infty} \Pi_{i=1}^{s} D_i^r$ and $\lim_{s\to \infty} \Pi_{i=1}^{s} D_i^c$ exist. 
Hence the claim. \citep{rothblum1989scalings, idel2016review}

\end{proof}



\begin{replemma}{lemma:cr_dr}
For two positive matrices $A, B$, 
$A \overset{c.r.}{\sim}B$ if and only if 
there exist positive diagonal matrices $D^r$ and $D^c$ such that $A = D^r B D^c$.
\end{replemma}
\begin{proof}
The \textbf{if direction}:
$A = D^r B D^c$  $\Longrightarrow$ 
$\displaystyle \frac{a_{ik}a_{jl}}{a_{il}a_{jk}} = \frac{d^r_ib_{ik}d^{c}_{k} \cdot d^{r}_{j}b_{jl}d^{c}_l}{d^{r}_ib_{il}d^{c}_{l} \cdot d^{r}_jb_{jk}d^{c}_k} 
=  \frac{b_{ik}b_{jl}}{b_{il}b_{jk}}$  $\Longrightarrow$  $A \overset{c.r.}{\sim}B$.

The \textbf{only if direction}: Let the dimension of $A, B$ be $m\times n$, we will prove by induction on $m+n$. 
\textit{Step1.} Assume the dimension of $A, B$ is $2\times 2$.
Let the marginal of $A$ be $\mu_A$ and $\nu_A$, and  $B^* = \Phi (B, \mu_A, \nu_A)$. Then $A$ and $B^*$ 
have the same marginals and cross ratios, which put four same independent constraints on elements of $A$ and $B$,
hence $A =  B^* = D^r B D^c$  for some $D^r, D^c$.
\textit{step2.} Assume the statement holds for $m+n< N$. 

\newpage
Now assume that $m+n = N$. 
Denote the submatrices of $A$ and $B$ consisted by their first $n-1$ by $A_{1}$ and $B_{1}$.
$A\overset{c.r.}{\sim} B \Longrightarrow A_{1}\overset{c.r.}{\sim} B_{1}$. By the inductive assumption, there exist
diagonal matrices $D^r_1$ and $D^{c}_1$ such that $A_{1} = D^r_1 B_1 D^c_1$. 
Further $\frac{a_{11}a_{1n}}{a_{i1}}a_{in} = \frac{b_{11}b_{1n}}{b_{i1}}b_{in}$ holds for any $i\in \{1,\dots, m\}$ imply that
there exists an $d>0$ such that $\mathbf{a}_{n} = d \cdot \mathbf{b}_{n}$. Let $D^r = D^r_1$, $D^{c} = \diag{D^c_1, d}$, 
we have $A = D^rB D^c$ holds. Hence the only if direction is completed.
\end{proof}


\begin{reptheorem}{thm:IOT}
Let $T$ be an observed positive optimal coupling of dimension $m\times n$. 
Then $\Phi^{-1} (T)$ is a hyperplane of dimension 
$m+n-1$ embedded in $ (\mathbb{R}^*)^{m\times n}$, which consists all the cost matrices 
that of the form:
\begin{equation}\label{supeq:cr_equiv}
 \Phi^{-1} (T) = \{C \in (\mathbb{R}^*)^{m\times n} | K= e^{-C} \overset{c.r.}{\sim} T\}.    
\end{equation}
\end{reptheorem}

\begin{proof}
Combining Proposition~\ref{prop:DAD} and Lemma~\ref{lemma:cr_dr}, we have Eq.~\eqref{supeq:cr_equiv} holds.
Hence $\Phi^{-1} (T)$ contains all the matrices $C$ satisfying the following set of equations:
$\frac{k_{ik} k_{jl}}{k_{il} k_{jk}} = \frac{t_{ik} t_{jl}}{t_{il} t_{jk}} $ 
for any $i, j \in \{1, \dots, m\}$ and $k, l \in \{1, \dots, n\}$, where $K = e^{-C}$, i.e. $k_{ik} = e^{-c_{ik}}$.
Thus $\Phi^{-1} (T)$ is the solution set of the system of linear equations:
\begin{equation} \label{supeq:linear_sys}
    c_{il}+c_{jk} - c_{ik}-c_{jl} = \ln (t_{ik} t_{jl}) - \ln (t_{il} t_{jk})
\end{equation}
Further Remark~\ref{rmk:basis} shows that there are only $(m-1)(n-1)$ independent equations in the system \eqref{supeq:linear_sys}.
Hence $\Phi^{-1} (T)$ is a hyperplane of dimension $mn - (m-1)(n-1) = m+n-1$.
\end{proof}




\begin{repcorollary}{cor:proj_single_column}
Under prior $\mathbf{P_2}$,
the projection of $\text{supp}[P(K|T)]$ onto each column is a $(m-1)$-dimensional manifold that is homeomorphic to the simplex $\Delta_{m-1}$. 
\end{repcorollary}

\begin{proof}
According to prior $\mathbf{P_2}$, for any $K \in \text{supp}[P(K|T)]$, each column of $K$ sums to $1$. 
Hence the projection of $\text{supp}[P(K|T)]$ onto any $j$-th column is embedded in the simplex $\Delta_{m-1}$. 
To show `homeomorphic ', 
we only need to show that for each $v \in \Delta_{m-1}$, there exists a $K \in \text{supp}[P(K|T)$ such that $\mathbf{k}_{j} =v$.
As discussed in Remark~\ref{rmk: one_free_column}, let $D'^{r} = \diag(v/\mathbf{t}_{j})$, 
$K' = \text{Col}( D'^{r}T)$. It's easy to check that $K'\in \text{supp}[P(K|T)]$, and $\mathbf{k'}_{j} = v$.
Hence the corollary holds.
\end{proof}
% \textit{Cross ratio equivalent} is defined in \citep{pei2019generalizing} as following:
% \begin{definition}
% Let $A = (a_{ij})_{n\times n}$ be a square matrix and $S_n$ be the set of all permutations of length~$n$.
% For any $\sigma \in S_n$, the set of $n$-elements $\{a_{1,\sigma(1)}, a_{2,\sigma(2)}, \dots,a_{t,\sigma(n)}\}$
% is called a \textbf{diagonal} of $A$.
% If every $a_{k, \sigma(k)} > 0$, then the diagonal is said to be \textbf{positive}.
% \end{definition}


% \begin{definition}\label{def:cross ratios}
% Let $A, B$ be two $n\times n$ matrices and $D^A_1=\{a_{1,\sigma(1)},\dots, a_{n, \sigma(n)}\}$ and $D^A_2=\{a_{1,\sigma'(1)},\dots, a_{n, \sigma'(n)}\}$ be two positive diagonals of $A$ determined by permutations $\sigma, \sigma'\in S_n$. 
% Denote the products of elements on $D^A_1$ and $D^A_2$ by $d^A_1=\Pi_{i=1}^{n}a_{i, \sigma(i)}, d^A_2=\Pi_{i=1}^{n}a_{i, \sigma'(i)}$ respectively. Then $\CR(D^A_1, D^A_2)=d^A_1/d^A_2$ is called the \textbf{cross ratio} between $D^A_1$ and $D^A_2$ of $A$. Further, let the diagonals in $B$ determined by the same $\sigma$ and $\sigma'$ be 
% $D^B_1=\{b_{1,\sigma(1)},\dots, b_{n, \sigma(n)}\}$ and $D^B_2=\{b_{1,\sigma'(1)},\dots, b_{n, \sigma'(n)}\}$. We say $A$ is \textbf{cross ratio equivalent} to $B$, denoted by $A\overset{cr}{\sim} B$, if $d_i^A\neq 0 \Longleftrightarrow d_i^B\neq 0$
% and $\CR(D^A_1, D^A_2)=\CR(D^B_1, D^B_2)$ holds for 
% any $D^A_1$ and $D^A_2$.
% \end{definition}

\begin{repproposition}{prop:submanifold}
$C_s \in \text{supp}[P(C_s|T)]$ if and only if there exists positive diagonal matrices $D_s^c, D_s^r$ such that $K_s = D_s^c T_s D_s^r$ and
the system of equations shown below have a positive solution for $\{x_1, \dots, x_{m-s_1}\}$.
\begin{equation}\label{supeq: submainfold}
  (x_1, \dots, x_{m-s_1}) T_{m-s}  = (1/d^c_1, \dots, 1/d^c_{s_2}) - \mathbf{1}_s D_s^rT_s  
\end{equation}

\end{repproposition}

\begin{proof}
The \textbf{if direction}: Let $(x_1, \dots, x_{m-s_1})$ be a positive solution of Eq.~\eqref{supeq: submainfold}, 
let $D'^{r} = \diag (D^{r}_s, x_1, \dots, x_{m-s_1})$ be an extension of $D^r_s$.
Denote the column sum of $D'^{r} T$ by $\nu'$. Then Eq.~\eqref{supeq: submainfold} implies that $\nu'_i = d^c_i$ for 
$i \in \{1, \dots, s_2\}$. Let $D'^c = \diag(D^c_s, \nu'_{s_2+1}, \dots,\nu'_{n})$. 
It is clear that $K' = D'^r T D'^c \in \text{supp}[P(K|T)]$, and $K_s$ is $K'$'s submatrix corresponding to $X_s\times Y_s$.

The \textbf{only if direction}: for $C_s \in \text{supp}[P(C_s|T)]$, let $K_s = e^{-C_s}$ be the submatrix of $K'\in \text{supp}[P(K|T)$.
Then there exists $D'^r, D'^c$ such that $K' = D'^r T D'^c $. Let the corresponding submatrices of $D'^r, D'^c$ be $D^r_s, D^c_s$. 
We have $K_s = D_s^c T_s D_s^r$ hold. Further it is easy to verify that $(d'^r_{s_1+1}, \dots d'^r_{n})$ is a positive solution for 
Eq.~\eqref{supeq: submainfold}. Hence the proof is completed.
\end{proof}


\begin{repcorollary}{cor:missing_element}
Under prior $\mathbf{P_2}$, 
$\mathcal{K}_1$ is a line segment in $\Delta_{m-1}$ that can be parameterized as:
$\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} \in (0,\infty) \}$.
\end{repcorollary}

\begin{proof}
Corollary~\ref{cor:proj_single_column} implies that $\mathcal{K}_1 \subset \Delta_{m-1}$. 
Further Remark~\ref{rmk: one_free_column} implies that for each choice of $t_{m1} >1$, 
a known $\mathbf{k}_l$ uniquely determines a point in form of $(d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}$ 
in $\mathcal{K}_1$. Hence the corollary holds.
\end{proof}


\begin{repcorollary}{cor:parallel}
Let $T_1, T_2$ be two positive matrices of dimension $m \times n$.
The hyperplanes $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
In particular, if $T_1 \overset{c.r.}{\sim}T_2$ then $\Phi^{-1}(T_1) = \Phi^{-1}(T_2)$.
Otherwise $\Phi^{-1}(T_1)$ is parallel to $\Phi^{-1}(T_2) $.
\end{repcorollary}


\begin{proof}
According to the proof of Theorem~\ref{thm:IOT} above, 
both $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$ are defined by system of equations in form of
Eq.~\eqref{supeq:linear_sys}. In particular, they have the same coefficients, 
only the constants on the right side of the equations are different.
Hence, $\Phi^{-1}(T_1)$ and $\Phi^{-1}(T_2)$, have the same normal direction.
\end{proof}


\begin{repproposition} {prop: bounded_noise}
For a coupling $T$,  assume uniform observation noise on $t_{11}$ with bounded size $a$, 
\begin{equation}\label{supeq: bounded_noise}
 \text{supp}[P(C|T)] = \cup_{T'\in \mathbb{B}_{a}(T)} \Phi^{-1}(T'),   
\end{equation}

where $\mathbb{B}_{a}(T)$ is the set of matrices $T'$ of the same dimension as $T$ with the property that:
$t'_{11}>0$, $|t'_{11} - t_{11}| \leq a$ and $t'_{ij} = t_{ij}$ for other $i, j$.
Moreover, $\Phi^{-1}(T')$ can be expressed as intersection of two hyperplanes (may be in different dimensions):
one with equation: $c_{11} + c_{22} - c_{21} - c_{12} = - \ln\frac{t'_{11} t_{22}}{t_{21}t_{12}}$, 
and the other equation does not depend on the value of $t'_{11}$. Assume the angle between these two hyperplanes is $\theta$.
Then $d(\Phi^{-1}(T_1'), \Phi^{-1}(T_2')) \leq \ln \frac{t_{11} + a}{t_{11} - a} /\sin \theta $ for $T_1', T_2' \in \mathbb{B}_{a}(T)$.
\end{repproposition}

\begin{proof}
With bounded noise on $t_{11}$, the domain for $t^*_{11}$ is $[t_{11}-a, t_{11}+a] \cap \{t^*_{11} > 0\}$.
Hence Eq.~\eqref{supeq: bounded_noise} holds. $\Phi^{-1}(T')$ is defined by the cross ratios of $T$ as shown in 
Eq.~\ref{supeq:linear_sys}. Using cross-ratio basis say $\mathcal{B} =\{r_{mjnk}(T')| j = 1, \dots, m-1, k=1,\dots, n-1 \}$, Eq.~\ref{supeq:linear_sys} 
can be simplified into a system with only independent $(m-1)(n-1)$, where only the equation defined by $r_{m1n1}(T')$ involves $t'_{11}$,
the other equations can be combined into one equation by substitutions.
Each of these two equations determines a hyperplane,
hence $\Phi^{-1}(T')$ can be expressed as the intersection of two hyperplanes.
Moreover, let the defining hyperplanes for $T^1, T^2 \in \mathbf{B}_a(T)$ be $\{H^1_1, H^1_2\}$ and  $\{H^2_1, H^2_2\}$ respectively,
where $H^i_1$ is the one defined by $ c_{11}+c_{mn} - c_{m1}-c_{1n} = \ln (t_{m1} t_{1n}) - \ln (t^i_{11} t_{mn})$, where $i =1,2$.
Then the Euclidean distance between $H^1_1, H^1_1$ is $d(H^1_1, H^1_1) = |\ln t^1_{1,1} - \ln t^2_{1,1}| \leq |\ln (t_11 +a) - \ln (t_11 -a)|$.
Notice that $H^1_2 = H^2_2$. So the distance between $\Phi^{-1}(T^1), \Phi^{-1}(T^2)$ is bounded by $(\ln (t_{11} +a) - \ln (t_{11} -a))/\sin\theta$.
\end{proof}


\begin{repproposition}{prop: gaussian_noise}
Let $T$ be an observed coupling of dimension $m\times n$ with Gaussian noise on $t_{11}$.
Further, let $\mathcal{B}$ be a basis for cross ratios of $m\times n$ matrices, that contains only one cross ratio depending on $t_{11}$.
Eliminate the cross ratio depending on $t_{11}$ in $\mathcal{B}$, denote the new set by $ \mathcal{B}^{-}$. Then: 

\centerline{$\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$}
In particular, $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T^*)$.
\end{repproposition}

\begin{proof}
Since the domain for $\epsilon \sim \mathcal{N}(0,\sigma^2)$ is $(-\infty, \infty)$, 
hence the domain for possible $t^*_{11}$ is $(0, \infty)$. 
Thus the observation $T$ essentially put no constraint on the cross ratio of $T^*$ depends on $t^*_{11}$.
Hence $\text{supp}[P(C|T)] = \{C|r(K) = r(T) \text{ for } r \in \mathcal{B}^{-}\}$. 
As only one equation was eliminated, so $P(C|T)$ is supported on a hyperplane that is one dimensional higher than $P(C|T^*)$.
\end{proof}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> neurips_2021/customized.tex <==
% \usepackage[utf8]{inputenc}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{fullpage}

\usepackage{graphicx}
\usepackage{color,soul}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amstext}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{pictexwd,dcpic}




\usepackage{tikz}
\usetikzlibrary{calc,intersections,through}
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

%\usepackage{pgfplots}

\newcommand{\pat}[1]{\textcolor[rgb]{.7,0,.2}{#1}}
\newcommand{\pw}[1]{\textcolor[rgb]{0.6,0.6,0}{#1}}
\newcommand{\wt}[1]{\textcolor[rgb]{0,0,0.7}{#1}}
%theorem styles



\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
\def\rep@title{#2 \ref{##1}}%
\begin{rep@theorem}}%
{\end{rep@theorem}}}
\makeatother

\newtheorem{thm}{Theorem}[section]
\newreptheorem{thm}{Theorem}
\newtheorem*{thm*}{Theorem}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newreptheorem{prop}{Proposition}
\newtheorem{exercise}{Exercise}
\newtheorem{question}{Question}


\theoremstyle{definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{problem}[thm]{Problem}
% \newtheorem{remark}[thm]{Remark}
\newtheorem{example}[thm]{Example}
\newtheorem*{example*}{Example}
\newtheorem{examples}[thm]{Examples}
\newtheorem{notation}[thm]{Notation}
\newtheorem*{framework*}{Unifying OT Framework}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

% \newtheorem{theorem}{Theorem}[section]
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{note}[theorem]{Note}
% \newtheorem{remark}[theorem]{Remark}



% Notations
\newcommand{\D}{\mathcal{D}} % data space
\newcommand{\hp}{\mathcal{H}} % hypothesis space
\newcommand{\R}{\mathbb{R}} % all real numbers.
\newcommand{\e}{\epsilon} % a small parameter
\newcommand{\E}{\mathbb{E}}%  expectation
\newcommand{\kl}{\text{KL}}%  
\newcommand{\diag}{\text{diag}}%  
\newcommand{\CR}{\text{CR}}%  


% \usepackage[
% backend=biber,
% style=alphabetic,
% sorting=ynt
% ]{biblatex}



==> neurips_2021/main.tex <==

\section{Introduction}

%A common goal in machine learning is to infer, given some observations, estimate the model(s) that may have generated the observations. 
%Suppose, however, that the observed data are not the outcome of a single model, but a collection of models and the observed data they produce are an efficient assignment of models to instances. Such situations commonly occur among collections of individuals, where the possible outcomes are a constrained set, all of which must be covered. See
%In such situations, we may also wish to draw inferences about the underlying models, but in order to do so we must account for the interactions among individuals arising from the coupling process. This class of problems is naturally formalized via Inverse Optimal Transport (IOT). 

\pat{set up the paper against prior work. assume squared noise on plan. do not understand underlying geometric structure}

\pat{our contributions: 
(1) describe geometry of underlying manifold 
(2) Geometry provides insight into missing value problems
(3) Algorithm for inference based on geometry (current algorithm, show it works for randomly generated matrix)
(4) standardly assumed noise model iteracts with support (claim: high CR means more concentrated posterior, due to "fewer" manifolds in the same Gaussian ball.)
(5) improved inference for standard noise model based on cross ratios??? 
-- Clever way for thinking about which manifolds are nearby, avoids computing sinkhorn over and over
(6) Geometry provides insight into behavior of different possible noise models (multiple agents, noise on perceived costs)
}

%A common goal in machine learning is to infer, given some observations, estimate the costs that underlie the observations. 
Given a coupling of two discrete probability distributions, can we infer the underlying costs that explain the observed joint density? Such couplings appear commonly when one set is matched with a second set. Examples include team sports like basketball where players must serve different functions, in movement of commuters in and out of cities, and in performance of ad hoc teams. Where the problem of computing stochastic couplings is formulated as Entropy regularized optimal transport, we investigate the problem of inferring underlying costs via Inverse entropy regularized Optimal Transport.  

In contrast with (entropy-regularized) Optimal Transport (OT) \citep{villani2008optimal,cuturi2013sinkhorn}, Inverse Optimal Transport has received less systematic attention. 
Although researchers have studied IOT in migration \citep{stuart2020inverse} and matching problems \citep{li2019learning}, and through adversarial robustness \citep{paty2020regularized} formulation and investigation of the general problem of probabilistic inference of latent costs from stochastic couplings given priors has not been systematically undertaken. Like EOT, 
IOT inherits interesting geometric structure from Sinkhorn scaling \citep{sinkhorn1964relationship}, which gives rise to natural questions about the nature of posterior distributions, the existence of samplers, and questions about the feasibility and effectiveness of inferences from observed couplings to underlying costs. 

In this paper, we investigate properties of probabilistic IOT with several contributions. We begin by formalizing the problem and proving some basic results. Our first contribution is to characterize the manifold of support of the posterior distribution along with the implications of prior distributions on posterior inference. Our second contribution is to present an elementary MCMC algorithm for posterior inference which derives directly from properties of Sinkhorn scaling. Our third contribution is to explore the feasibility of inference in this model by simulation and by demonstration on a real-world performance of NBA basketball teams. We conclude by discussing implications of the approach and interesting directions for extending the work. 

\paragraph{Notation:} $\mathbb{R}^*$ is non-negative reals. $\Delta_k$ is the $k$-dimensional simplex.
For a space $X$, $\mathcal{P}(X)$ denotes the set of distributions over $X$. 
For a matrix $M_{s\times t}$, $\mathbf{m}_1, \dots,\mathbf{m}_{t}$ denotes columns of $M$; $\text{Col}(M)$ denotes column normalization of $M$.

\section{Probabilistic inverse optimal transport} \label{sec:piot}

%Consider the situation where data from a collection of models were observed and the inference needs to be made on the underlying interactions between those models.
%In this section we formalize such inference as probabilistic inverse optimal transport. 

%\pw{discuss, notations, name for H,  T and C, $t_{ij}, c_{ij}$}

\pat{pull out all details about column normalization to make it fully general to dirichlet prior on cost}

Given two spaces $X = \{x_1, \dots, x_m\}$ and $Y = \{y_1, \dots, y_n\}$, 
let $T = (t_{ij})_{m\times n}$ be a \textit{coupling} that records the co-occurrence distribution between $X$ and $Y$.
%Each column of $P$ is indexed by an $h$ and each row of $P$ is indexed by a $d$.
Each element $t_{ij}$ represents the probability of observing $x_i$ and $y_j$ simultaneously. 
The interaction between $X$ and $Y$ can be captured by a \textit{cost matrix} $C = (c_{ij})_{m\times n}$, 
where $c_{ij} \geq 0$ measures the underlying cost of coupling $x_i$ and $y_j$. 
Hence, the probabilistic inference on the underlying structure over $X$ and $Y$ is then to obtain $P(C|T)$, 
the distribution over all possible cost $C \in (\mathbb{R}^*)^{m\times n}$ given an observed coupling $T$.

%The total cost of a plan $T$ is defined to be $\langle C, T\rangle = \sum_{i\in \D, j\in \hp} c_{ij}t_{ij}$, the Frobenius inner product.
%Let the prior of $C$ be $P_0(C)$, a distribution over $(\mathbb{R}^*)^{m\times n}$. %($\mathbb{R}^*$ is the set of non-negative real numbers). 
%Then the inference on $C$ 
%can be concluded using Bayes Rule: $P_t(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$.

% \pw{How do we justify the assumption that $T$ is optimal, by assuming the underlying model is cooperative?}
% \pw{directly go for EOT or OT}

%Assuming the $T$ is obtained by minimizing the total cost, we may 
\textbf{Inverse entropy regularized optimal transport} is the fundamental building block in modelling $P(C|T)$. 
Given a cost matrix $C$ and distributions $\mu,\nu$ over $X$ and $Y$ respectively, 
\textit{Entropy regularized optimal transport (EOT)} \citep{cuturi2013sinkhorn} solves the optimal plan $T^{\lambda}$ that 
minimizes the entropy regularized cost of coupling $X$ with distribution $\mu$ into $Y$ and distribution $\nu$. 
Thus for a parameter $\lambda >0$: 

\centerline {$\displaystyle T^{\lambda} = \arg\min_{T\in U(\mu, \nu)} \{\langle C, T\rangle - \frac{1}{\lambda} H(T)\},$}

\noindent where $U(\mu, \nu)$ is the set of all couplings between 
between $\mu$ and $\nu$ (i.e. joint distributions with marginals $\mu$ and $\nu$), $\langle C, T\rangle = \sum_{i\in X, j\in Y} c_{ij}t_{ij}$ is 
the Frobenius inner product between $C$ and $T$, and $H(T) := \sum_{i=1}^{m}\sum_{j=1}^{n} t_{ij} \log t_{ij}$ 
is the \textit{entropy} of $T$. $T^{\lambda}$ is called an \textit{optimal coupling} with parameter $\lambda$. 

\textbf{Sinkhorn scaling} is used to efficiently compute optimal couplings.
$(\mu,\nu)$-\textit{Sinkhorn Scaling (SK)} \citep{sinkhorn1964relationship} of a matrix M 
is the iterated alternation between row normalization of $M$ with respect to $\mu$ and 
column normalization of $M$ with respect to $\nu$. \cite{cuturi2013sinkhorn} proved that: 
fix a cost matrix $C$, the optimal coupling $T^{\lambda}$ between $\mu$ and $\nu$ 
can be solved by applying $(\mu, \nu)$-Sinkhorn scaling on \textit{negative exponential cost matrix} $K^{\lambda}$, where $K^{\lambda} = e^{-\lambda C} = (e^{-\lambda\cdot c_{ij}})_{m\times n}$.


Therefore inverse entropy regularized optimal transport can be interpreted as map from an optimal 
coupling $T^{\lambda}$ to the set of all possible triples of cost and marginals $\{(\widehat{C}, \widehat{\mu},\widehat{\nu})\}$. 
For a fixed $\lambda$, we may view EOT as a map $\Phi$:$(\mathbb{R}^*)^{m\times n} \times \mathcal{P} (\mathbb{R}^{m}) \times 
\mathcal{P} (\mathbb{R}^{m}) \to \mathcal{P} ((\mathbb{R}^*)^{m\times n})$ with $\Phi(C, \mu, \nu) = T^{\lambda}$.
Hence we define \textbf{inverse entropy regularized optimal transport (IOT)} as $\Phi^{-1}: T^{\lambda} \to \{(\widehat{C}, \widehat{\mu},\widehat{\nu})\}$.


Note that in IOT, the observed $T^{\lambda}$ completely determines $\widehat{\mu}$ and $\widehat{\nu}$. If $(\widehat{C}, \widehat{\mu},\widehat{\nu}) \in \Phi^{-1}(T^{\lambda})$, then 
$T^{\lambda} \in U(\widehat{\mu},\widehat{\nu})$. Thus $\widehat{\mu}$ and $\widehat{\nu}$ must equal the row and column marginals of $T^{\lambda}$.
Hence we may reduce IOT into $\Phi^{-1}: T^{\lambda} \to \{\widehat{C}\}$. Furthermore, an observed $T^{\lambda}$ does not uniquely determines the cost matrix $\widehat{C}$. 
In fact, according to the property of Sinkhorn scaling, we show that:

\begin{prop}\label{prop:DAD} \footnote{Proofs for all results are included in the supplemental materials.}
Let $T^{\lambda}$ be an observed optimal coupling, $\widehat{C} \in \Phi^{-1} (T^{\lambda})$ if and only if for every $\epsilon > 0$, 
there exist two positive diagonal matrices $D^r = \diag\{d^r_1, \dots, d^r_m\}$ and $D^c =\diag \{d^c_1,\dots, d^c_n\}$ such that: 
$\displaystyle |D^r \widehat{K}^{\lambda} D^c - T^{\lambda}| < \epsilon$, where $\widehat{K}^{\lambda} = e^{-\lambda \widehat{C}}$ and $|\cdot|$ is the $L^1$ norm. 
In particular, assume $T^{\lambda}$ is a positive matrix. Then $\widehat{C} \in \Phi^{-1} (T^{\lambda})$ 
if and only if there exists positive diagonal matrices $D^r,D^c$ such that $D^r \widehat{K}^{\lambda} D^c = T^{\lambda}$.
\end{prop}

\begin{remark}\label{rmk:cross-ratio}
Two square matrices are said to be \textit{cross-ratio equivalent} if the ratio between any two positive diagonals of the two matrices are the same. (See definition in supplemental materials.)  
\citep{pei2019generalizing} showed that if $m=n$, then any $\widehat{C}_1,\widehat{C}_2 \in \Phi^{-1} (T^{\lambda})$ are cross-ratio equivalent.
When $T^{\lambda}$ is positive, \cite{fienberg1970iterative} showed that $\Phi^{-1} (T^{\lambda})$ forms a special case of determinantal manifold that is studied in \cite{room1938geometry}.
The general space of $\Phi^{-1} (T^{\lambda})$ has not been studied.
%In general, format of $\Phi^{-1} (T^{\lambda})$ is not studied.
\end{remark}


\textbf{Probabilistic inverse optimal transport} is defined as $\displaystyle P(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$, 
where $P_0(C)$ is a prior of cost matrix $C$ over $(\mathbb{R}^*)^{m\times n}$, and likelihood $P(T|C) = 1$ if $C\in \Phi^{-1}(T)$, otherwise $P(T|C) = 0$.


\begin{prop}\label{prop:piot}
$ P(C|T)$ is supported on the intersection between $\Phi^{-1} (T)$ and domain of $ P_0(C)$, moreover, we have that
$\displaystyle P(C|T) = \frac{P_0(C)}{\int_{\Phi^{-1} (T)} P_0(C) \text{d} C}$.
\end{prop}



%Let the prior of $C$ be $P_0(C)$, a distribution over $(\mathbb{R}^*)^{m\times n}$. %($\mathbb{R}^*$ is the set of non-negative real numbers). 
%Then the inference on $C$ 
%can be concluded using Bayes Rule: $P_t(C|T) = \frac{P(T|C) P_0(C)}{P(T)}$.


To simplify the notation, in the rest of this paper, we will omit the superscript $\lambda$ for $T$ and $K$, and fix $\lambda = 1$ unless otherwise stated.
Results will be described in term of negative exponential cost matrix $K$. Corresponding statements in terms of $C$ can be obtained by $K = e^{-C}$.
Prior $P_0(K)$ is set to be the distribution where each column is follows symmetric Dirichlet distribution with hyperparameter $\alpha$ independently.
Since for any non-negative cost matrix $C$, elements in $K$ are in the range of $(0,1]$, which can be cross-ratio equivalently 
converted into a $K$ in the prior by column normalization.
Observed $T$ is assumed to be a positive matrix, the case when $T$ is non-negative can be derived using  machinery of \textit{maximal partial pattern} 
developed in \citep{pei2019generalizing}.

\subsection{Support Manifold of Inverse Optimal transport}
%\pw{We need to chat a bit about K and C.}
In this section, we characterize the manifold $\Phi^{-1} (T) \cap \text{Domain}(P_0(K))$ where the posterior distribution $P(K|T)$ is supported on.
On one hand, according to Proposition~\ref{prop:DAD}, we have:

\centerline{ $\displaystyle \Phi^{-1} (T) = \{\widehat{K}\in (0,1]^{m\times n}| \exists \text{ positive diagonal matrices } D^{r} \text{ and } D^{c} \text{ such that } \widehat{K} = D^rTD^c\}$.} 

On the other hand, $P_0(K)$ is supported on $\mathcal{P}(\mathbb{R}^{n})^{m} $. 
Therefore $P(K|T)$'s support, $\Phi^{-1} (T) \cap \text{Domain}(P_0(K))$, is of the form:
\begin{equation} \label{eq:supp_posterior}
    \text{supp}[P(K|T)] = \{ \widehat{K} \in (0,1]^{m\times n} | \exists D^{r} \text{ s.t. } \widehat{K} = \text{Col}(D^{r}T) \}
\end{equation}
%\centerline{$\displaystyle \text{supp}[P(C|T)] = \{ \widehat{C} \in (\mathbb{R}^{+})^{m\times n} | \exists D^{r} \text{ s.t. } \widehat{C} \text{ is column normalization of } D^{r}T \}$ }


\begin{remark}\label{rmk: one_free_column}
In particular, Eq.~\eqref{eq:supp_posterior} indicates that: \textbf{(i)} a known column of $\widehat{K}$ uniquely determines all the other columns. 
Indeed, denote the $j$-th column of $\widehat{K}$ by $\mathbf{k}_j = (k_{1j}, \dots, k_{mj})^T$ and use the same notation for $T$. 
Let $d_i = k_{ij}/t_{ij} $ and $D^{r} = \diag\{d_1, \dots, d_m\}$. 
Then the $l$-th column $\mathbf{k}_l$ equals to the column normalization of $D^{r} \mathbf{t}_l$.
\textbf{(ii)} for any $\mathbf{v} \in \mathcal{P}((\R^+)^m)$, there exists a $\widehat{K} \in  \text{supp}[P(K|T)]$ such that $\mathbf{k}_j = \mathbf{v} $.
Therefore, we have:
\end{remark}

\begin{cor}
$\text{supp}[P(K|T)]$ is a $(m-1)$-dimensional manifold that is homeomorphic to the simplex $\Delta_{m-1}$. 
\end{cor}

% \begin{figure}[h!]
%     \centering
%     \begin{tabular}{c|c}
%   $T$\hspace{0.05in}
%          & 
%   \hspace{0.8in}$P(\widehat{C}|T)$
%     \end{tabular}
    
%     \begin{tabular}{c|c}
%     \includegraphics[width=0.15\textwidth]{figs/simplex_T_1.png}
%          & 
%     \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_1.png}
%     \end{tabular}
%     \begin{tabular}{c|c}
%     \includegraphics[width=0.15\textwidth]{figs/simplex_T_2.png}
%          & 
%     \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_2.png}
%     \end{tabular}
%     \begin{tabular}{c|c}
%     \includegraphics[width=0.15\textwidth]{figs/simplex_T_3.png}
%         &
%     \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_3.png}
%     \end{tabular}
%     \caption{ %\pw{add some title to the plots?} \pat{not a fan of titles on plots}
%     Effect of $T$ on the posterior distribution $P(\widehat{C}|T)$.
%     The left panel plots three different observed $3\times 3$ couplings $T$. Columns $\mathbf{t_1},\mathbf{t_2},\mathbf{t_3}$ of $T$ are 
% represented by \textcolor{red}{red}, \textcolor{green}{green} and \textcolor{blue}{blue} points in a copy of $\Delta_2$.
% The right panel plots samples from the corresponding posteriors $P(\widehat{C}|T)$, where three triangles in each row represents three columns of these samples.
% (Since the prior $P_0(\widehat{C})$ is column-wise Dirichlet, each column of 
% a sample $\widehat{C} = \{\mathbf{c}_1, \mathbf{c}_2, \mathbf{c}_3\}$ can be represented by a point in a copy of $\Delta_2$).
% Here the samples are obtained by uniformly sample the second column $\mathbf{c}_2$ from $\Delta_2$, then construct $\mathbf{c}_1$ and $\mathbf{c}_3$ according to Remark~\ref{rmk: one_free_column}~(i)} 
%     \label{fig:cr}
% \end{figure}

\begin{figure}[h!]
    \centering
    \begin{tabular}{c|c c|c}
  $T$
         & 
  $P(\widehat{K}|T)$
   &
   \hspace{0.3in}$\alpha$
   &
$P(\widehat{K}|T)$ \\
    
    \raisebox{4pt}{\includegraphics[width=0.14\textwidth]{figs/simplex_T_1.png}}
    & 
    \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_1.png}
    &
     \raisebox{18pt}{\hspace{0.2in}$0.25$}
    & 
     \includegraphics[width=0.35\textwidth]{figs/simplices_alpha_0p25.png}
    \\
    
    \raisebox{4pt}{\includegraphics[width=0.14\textwidth]{figs/simplex_T_3.png}}
    & 
    \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_3.png}
    &
     \raisebox{18pt}{\hspace{0.2in} 1}
    &
    \includegraphics[width=0.35\textwidth]{figs/simplices_alpha_1p0.png}
    \\

    \raisebox{4pt}{\includegraphics[width=0.14\textwidth]{figs/simplex_T_2.png}}
    &
    \includegraphics[width=0.35\textwidth]{figs/simplices_uniform_col2_2.png}
    &
    \raisebox{18pt}{\hspace{0.2in} 4}
    &
    \includegraphics[width=0.35\textwidth]{figs/simplices_alpha_4p0.png}
    \end{tabular}
    \caption{ %\pw{add some title to the plots?} \pat{not a fan of titles on plots}
\textbf{Left and Middle:} The effect of $T$ on $\text{supp}[P(K|T)]$.
The far left panel plots three sampled $3\times 3$ couplings $\{T_1, T_2, T_3\}$. Normalized columns of $T_i$'s are 
represented by \textcolor{red}{red}, \textcolor{green}{green} and \textcolor{blue}{blue} points in $\Delta_2$.
The middle panel plots samples from the corresponding posteriors $P(\widehat{K}|T)$, where three triangles in each row represents three columns of these samples.
Here the samples are obtained by taking equally distanced $\mathbf{k}_2$ from a copy of $\Delta_2$, then construct $\mathbf{k}_1$ and $\mathbf{k}_3$ according to Remark~\ref{rmk: one_free_column}~(i).
\textbf{Right:} The effect of prior $P_{0}(K)$ on $\text{supp}[P(\widehat{C}|T)]$. Fixing $T=T_2$, $P_{0}(K)$ varies by altering hyperparameter $\alpha$ in $[0.25, 1, 4]$. As in the middle panel, $\mathbf{k}_2$ is uniformly sampled from a copy of $\Delta_2$, $\mathbf{k}_1$ and $\mathbf{k}_3$ are then constructed accordingly.} 
    \label{fig:cr}
\end{figure}

% Due to the column-wise Dirichlet prior $P_0(\widehat{C})$, $P(C|T)$ is supported on $\mathcal{P}((\R^+)^m) \sim \Delta_2 \times \Delta_2 \times \Delta_2$.
% Each column of a sample $\widehat{C}$ lives in a copy of $\Delta_2$.
%Due to the column-wise Dirichlet prior $P_0(\widehat{C})$, $P(C|T)$ is supported on $\mathcal{P}((\R^+)^m) \sim \Delta_2 \times \Delta_2 \times \Delta_2$.  

    % \caption{\wt{Discussion: the plots here are all $\lambda=1.0$ but with different $P$. I want to see the effect of $P$ on the posterior distributions. Maybe this could be another figure? I will add plots for different $\lambda$.} Effects of variation in the cross-ratio on the manifold of possible cost matrices for a $3 \times 3$ matrix. Due to normalization, the manifold lives in \pat{fixme: 3simplex by 3simplex by 3 simplex}. \wt{The matrices indicate the starting OT plan $P$.} In each row, the middle column represents the sampling of the unconstrained simplex. \wt{We take equally spaced samples.} The left and right depict the implied constraints for the remaining two simplices. All rows are derived from the same randomly sample initial cost matrix, raised to a different power $\lambda$, iterated to a converged $P$ via Sinkhorn scaling. Each dot is a sample from the supported region of the posterior distribution. \pw{caption not checked yet}} 
Left of Fig.~\ref{fig:cr} shows the effect of $T$'s on the posterior $P(K|T)$.
We start by sampling the columns for a $3\times 3$ coupling $T$ according to a symmetric Dirichlet distribution with hyperparameter equals $1$.
Three samples $T_1, T_2, T_3$ are shown on the left panel:
normalized columns of each $T_i$ are 
represented by \textcolor{red}{red}, \textcolor{green}{green} and \textcolor{blue}{blue} points in $\Delta_2$.
$\widehat{K} \in \text{supp}[P(K|T)] $ is generated by sampling $D^{r}$. 
In order to see the effect of cross-ratios, we let the second column $\mathbf{k}_2$ of the $\widehat{K}$ be unconstrained.
Remark~\ref{rmk: one_free_column}~(ii) guarantees that the point representing $\mathbf{k}_2$ 
can be taken as any point in $\Delta_2$. The middle triangles of the second panel plot equally distanced $\mathbf{k}_2$ on a copy of $\Delta_2$.
%\pw{Weiting, please check if this is accurate.} \wt{I took equally distanced in 2D Cartesian space for the first two elements, and then project them onto a simplex.}
Then, the $\mathbf{k}_1$ and $\mathbf{k}_3$ are uniquely determined by $\mathbf{k}_2$ as in Remark~\ref{rmk: one_free_column}~(i).
The first and third triangles of the right panel plot the corresponding $\mathbf{k}_1$ and $\mathbf{k}_3$ as $\mathbf{k}_2$ vary. 

Plots illustrate $P(K|T)$'s dependency on the cross ratio of $T$. For example, consider the relative position of the blue and red dots relative to the green dot in the middle simplex: although the blue dot is relatively close to the middle in absolute terms, because it is considerably closer to the bottom left than the green dot, its support concentrates in that region, and although the red dot is almost in middle of the simplex, its relative position compared to the green dot results in focused support on the left side of the simplex. 
%The posterior distributions reflect these trends and are modulated by the Dirichlet hyperparameter. 

Right of Fig.~\ref{fig:cr} shows effects of prior on $\text{supp}[P(K|T)]$. 
Taking $T = T_2$ fixed, $P_0(K)$ is altered by considering hyperparameter $\alpha$ in $[0.25,1,4]$. 
Similarly as in the left picture, the second column $\mathbf{k}_2$ is uniformly sampled in a copy of $\Delta_2$, which determines $\mathbf{k}_1 ,\mathbf{k}_3$ in the first and third columns. 
Plots illustrate that the concentration of $P(K|T)$ varies with its prior accordingly.

% Fig. \ref{fig:cr} shows an example of the effect of the cross-ratio on the density of the manifold. We start by generating a matrix $P$ with columns following the Dirichlet distribution with concentration equaling to one. With $P$, we can generate the cost matrices. In order to see the effect of cross-ratio on the cost matrix, we let the second column of the matrix to be unconstrained and take uniformly distributed samples on the simplex for the second column. After that, the first and third columns can be computed by keeping the cross-ratio to be the same as $P$, which can be done by scaling the rows of $P$ to the designated numbers of the sampled second column and then normalizing first and third columns. \wt{Add some discussion on the density...} -\pw{weiting's original description}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.25\textwidth]{figs/simplices_alpha_0p25.png}
%     %\includegraphics[width=0.5\textwidth]{figs/simplices_alpha_0p5.png}
%     \includegraphics[width=0.25\textwidth]{figs/simplices_alpha_1p0.png}
%     %\includegraphics[width=0.5\textwidth]{figs/simplices_alpha_2p0.png}
%     \includegraphics[width=0.25\textwidth]{figs/simplices_alpha_4p0.png}
%     \caption{Effects of variation in the $\alpha$ prior for posterior inferences for a $3 \times 3$ matrix. For all simulations, we use plan associated with the $\lambda=1$ cost matrix from Figure~\ref{fig:cr}. In each row, the middle column represents the sampling of the unconstrained simplex, which reflects the influence of the prior. The left and right depict the implied posterior distributions for the other two columns. Rows differ in the value of $\alpha= \{0.25, 0.5, 1.0, 2.0, 4.0\}$ from top to bottom. Each dot is a sample from the posterior distribution.
%     \pw{caption not checked yet}}
%     \label{fig:alpha}
% \end{figure}

\subsection{Visualizing subspaces of $\Phi^{-1} (T^{\lambda})$.} \label{sec:subspace}

For $X^{s_1} = \{x_1, \dots, x_{s_1}\} \subset X$, $Y^{s_2} = \{y_1, \dots, y_{s_2}\}\subset Y$, let $K^s$ be the submatrix of a negative exponential cost $K$ 
that corresponds to $X^{s_1}\times Y^{s_2}$.
In this section, for a given observation $T$, we characterize the support of $P(K^s|T)$ as a subspace of $\text{supp}[P(K|T)]$.

For any $\widehat{K}^s \in \text{supp}[P(K^s|T)]$, there exists a $\widehat{K} \in \text{supp}[P(K|T)]$ such that $\widehat{K}^s$ is a submatrix of $\widehat{K}$.
As the domain for a column $\mathbf{k}_i$ of $\widehat{K}$ is a copy of $\Delta_{n-1}$, the domain for a column of $\mathbf{k}^s_i$ of $\widehat{K}^s$ is 
a copy of $\Sigma_{s_1} = \{\mathbf{k} = (k_1, \dots, k_{s_1}) \in (\mathbb{R}^* )^{s_1}| k_{1}+\dots +k_{s_1} < 1\}$.
Without loss, we may pick the first column $\mathbf{k}_1$ of $\widehat{K}$ to be the a free column which uniquely determines all the other columns.
Then according to Remark~\ref{rmk: one_free_column}, for any $\mathbf{v} = \{v_1, \dots, v_{s_1}\} \in \Sigma_{s_1}$, 
there exists a $\widehat{K}^s \in \text{supp}[P(K^s|T)]$ such that $\mathbf{k}^{s_1}_1 = \mathbf{v}$. % where $\mathbf{c}^{s_1}_1$ is the first column of $\widehat{C}^s$.
Intuitively, as each $\mathbf{k}_1$ uniquely determines other $\mathbf{k}_k$'s,
each choice of $\mathbf{k}^{s_1}_1$ determines a set 
$\mathcal{K}^{s_1}_l$ of $\mathbf{k}^{s_1}_l$ , for $l \in {2, \dots, s_1}$.
In more detail, let $d^s_i = k^{s_1}_{i1}/t_{i1}$, $D^{s} = \diag\{d^s_1, \dots, d^s_{s_1}\}$. 
Since $\widehat{K} = \text{Col} (D^{r} T)$, $\widehat{K}^s$ equals to $D^{s}T^s$ up to a scalar. 
Thus $\mathcal{K}^{s_1}_l \subset \mathcal{W}_l = \{(d^s_1*t_{1l}*a_l, \dots, d^s_{s_1}*t_{s_1,l}*a_l) | a_l>0 \text{ and }\sum_{i=1}^{s_1} d^s_1*t_{1l}*a_l < 1\}$.
Here $\mathcal{W}_l$ forms a ray staring at $(0,0)$ (not including $(0,0)$) with slope $(d^s_1*t_{1l},\dots, d^s_{s_1}*t_{s_1,l})$ in the copy of $\Sigma_{s_1}$ for $\mathbf{k}^{s_1}_{l}$.


It is important to note that not every point on $\mathcal{W}_l$ is included in $\mathcal{K}^{s_1}_l$. 
As $\widehat{K}^s$ is a submatrix of $\widehat{K}$, the choice of $a_l$ must be a proper column normalizing constant of a $D^rT$. 
Thus, the choice of $a_l$ needs to guarantee that there exist $d_{s_1 +1}, \dots, d_{m}>0$,
such that the $l$-th column sum of $D^{r*} T$ is $a_l$, where $D^{r*} = \diag\{d^s_1, \dots, d^s_{s_1},d_{s_1 +1}, \dots, d_{m}\}$.
Let $T^{m-s}$ be the submatrix of $T$ corresponding to $\{x_{s_1+1}, \dots, x_{m}\} \times Y^{s_2}$, $A = \diag\{1, 1/a_2, \dots, 1/a_s\}$.
Therefore we have:
\begin{prop}
$D^sT^sA \in \text{supp}[P(C^s|T)]$ if and only if the system of equations 
$(x_1, \dots, x_{m-s_1}) T^{m-s}  = (1, a_2, \dots, a_{s_1}) - \mathbf{I}_s D^sT^s$ have a set positive solution for $\{x_1, \dots, x_{m-s_1}\}$, where $\mathbf{I}_s = (1, \dots, 1)$.
\end{prop}







\subsection{Visualizing space of $\Phi^{-1} (T^{\lambda})$ with a missing element in $T$.} \label{sec:missing_element}
In this section, we will characterize the support of $P(\widehat{K}|T)$, when $T$ has a missing element.
%\pw{It seems up to here we do not need to assume T is column normalized, will proceed with no such assumption in this subsection too.}
%
Without loss, assume that $T$ is observed with $t_{m1}$ missing. 
Let the domain of $t_{m1}$ be $(0, \infty)$. Then according to \eqref{eq:supp_posterior} we have:

 \centerline{$ \text{supp}[P(K|T)] = \{ \widehat{K} \in (\mathbb{R}^{+})^{m\times n} | \exists D^{r} \text{ and } \widehat{t}_{m1} >0, \text{ s.t. } \widehat{K} = \text{Col}(D^{r}\widehat{T}) \}$}
 
 where $\widehat{T}$ is $T$ with $\widehat{t}_{m1}$ as its $m1$-th element.

In this case, a known column $\mathbf{k}_l$ of $\widehat{K}$ determines a set $\mathcal{K}_1$ of $\mathbf{k}_1$ which forms a line segment in $\Delta_{m-1}$.
Let $D^{r} = \diag \{k_{1l}/t_{1l}, \dots, k_{ml}/t_{ml}\}$. Then the line segment can be parameterized as 
$\mathcal{K}_1 = \{ (d_1t_{11}, \dots, d_m t_{m1})/\sum_{i = 1}^{m} d_it_{i1}| t_{m1} = \widehat{t}_{m1} \in (0,\infty) \}$.

\begin{remark}
Note that for different choice of prior, $\mathcal{K}_1$ could be a curve instead of a line segment. 
Denote the prior imposed constraint equation on $\mathbf{k}_1$ be $f_1(\mathbf{k}_1) = 0$,
the ratio imposed linear constraint on $\mathbf{k}_1$ be $f_i(\mathbf{k}_1) = 0$, where $f_i(\mathbf{k}_1) = k_{11}/k_{i1} - d_1*t_{11}/(d_i*t_{i1})$,
for $i = 2, \dots, m-1$.
Then $\mathcal{K}_1$ is the solution set for system of equations $\{f_1, f_2, \dots, f_{m-1}\}$.
With Dirichlet prior, $f_1$ is also linear, so $\mathcal{K}_1$ is a line segment. 
\end{remark}

\subsection{Approximate inference via MCMC}

%\pat{Please read and check this section. When done, please delete this comment.}
%\pat{mathcal K is the set of samples. declare?}
For a given observed optimal plan $T$ and a prior on the columns of the cost matrix $C$, we propose an Markov Chain Monte Carlo (MCMC) method based on the Metropolis algorithm for sampling from the posterior distribution. %The cross-ratio of the generated cost matrices are the same as $T$. 
%
The algorithm works as follows.\footnote{We suppress the $\lambda$ superscript to simplify notation of iterations.} 
At iteration $i$, given the exponential of the cost matrix $K^{(i)}$, we generate two vectors $D^m$ and $D^n$ with randomly sampled elements drawn from an exponential of a Gaussian distribution with mean zero and variance $\sigma$, and scale rows in $K^{(i)}$ by left multiplying $K^{(i)}$ by $D^m$ and columns by right multiplying $K^{(i)}$ by $D^n$ to give $K^{(i+1)}$. 
%We compute the probability of the cost matrix, $P($log$(K^{(i)} | \mu)$. 
The acceptance ratio, $r = \frac{P_0(C^{i+1})}{P_0(C^{i})} = \frac{P(\text{log}(K^{(i+1)}) | \theta)}{P(\text{log}(K^{(i)}) | \theta)}$, where $\theta$ represents the parameters of the model. Because our proposal distribution preserves the cross-ratios, we are guaranteed to stay on the manifold of support. Therefore, $P(T|C)$ is always $1$ and is omitted (see Proposition~\ref{prop:piot}). 
We accept or reject the move by comparing the acceptance ratio to an uniform random variable, $u$, which concludes a single step of the MCMC algorithm. A detailed description is provided in Algorithm 1. 

%Then, we then normalize the columns of $K^{(i+1)}$ and calculate the Dirichlet probability density function of the newly generated matrix Dir($K^{(i+1)}|\mu$)$=\prod_j$ Dir($\mathbf{k}_{j}|\mu$) where $\mathbf{k}_{j}$ is column $j$ of matrix $K^{(i+1)}$, and $\mu$ is the concentration of the Dirichlet distribution. The acceptance ratio is determined by Dir($K^{(i+1)}| \mu$)/Dir($K^{(i)}|\mu$). We accept or reject the move by comparing the ratio to an uniform random variable, which concludes a single step of the MCMC algorithm. A detailed description is provided in Algorithm 1. 
%We loop over all rows and stop until there are enough samples. The detailed procedure is shown in algorithm 1.
%\pat{we should talk through this. i'm not sure that the text and the algorithm are describing the same thing?}

\begin{algorithm}[H]\label{alg:MCMC}
\caption{Monte Carlo method for generating $\mathcal{K}$}
Inputs: OT plan $K^{(0)} = $ exp$(-\lambda T_{m \times n}$), Gaussian variance $\sigma$, Prior parameter(s) $\theta$, uniform random variable $u$ $\in$ [0, 1)\;
\For{i = 1 to ITERMAX}{
    $D^{m} =$ exp$( N(0, \sigma * \mathbb{I}_m) )$\; %\text{ones}(m,n)$ \; 
    $D^{n} =$ exp$( N(0, \sigma * \mathbb{I}_n) ) $\;
    $K^{(i+1)}\leftarrow$ diag($D^r$) $K^{(i)}$ diag($D^c$)\;
    %$K^{\lambda}_{i+1}\leftarrow$ ColumnNormalize[diag($D^r$) $K^{\lambda}_i$ diag($D^c$)]\;
    
   $r$ $\leftarrow P($log$(K^{(i+1)})| \theta) / P($log$(K^{(i)})| \theta)$\;
    \eIf{r > u}{
        Accept $K^{(i+1)}$\;
    }{
        Reject $K^{(i+1)}$\;
        $K^{(i+1)} \leftarrow K^{(i)}$
    }
}
\end{algorithm}

%To enable standard checks of convergence and mixing, we employ multiple chains based on random restarts. 
%Each chain is run for \pat{should this be 20,000? I'm confused.} 11,000 total steps, with 10,000 burn-in, and samples drawn with a lag of 1,000. Thus, we draw 10 total samples from each chain and a total of 500 samples in one simulation. 
%Sometimes during the MC simulation the matrix stuck at one of the vertex on the simplex and it takes long for the simulation to move it out of the vertex. In order to mitigate this issue and explore a larger part of the support we restart the Markov chain after running for fixed MC steps.

\section{Experiments}\label{sec:exp}

\paragraph{Effects of matrix size on manifold behavior.} 
%\pat{embed the 3x3 used for the above simulations inside progressively larger matrices, create the same figure as above (infer the costs for the whole matrix but show a picture of the same 3x3 subset. This will likely be boring in the sense that the picture is the same. (this seems very likely to be true. good to check. if so, this provides a nice decomposition result.) }

\begin{figure}[ht]
    \centering
    \begin{tabular}{c c c c}
        \textbf{a.}\includegraphics[width=0.2\textwidth]{figs/submat_1.png}
        &
        \textbf{b.}\includegraphics[width=0.2\textwidth]{figs/submat_2.png}
        &
        \textbf{c.}\includegraphics[width=0.2\textwidth]{figs/submat_3.png}
        &
        \textbf{d.}\includegraphics[width=0.2\textwidth]{figs/submat_4.png}
    \end{tabular}
    \caption{
    Visualization of $2\times 2$ subspaces of negative exponential cost of $4\times 4$ observations. 
    In each panel, a $T$ is sampled columnwise according to a Dirichlet distribution with $\alpha = 1$. 
    Each colored mark represents a uniformly sampled first column, $\mathbf{k}^s_1 = (k_{11}, k_{21})^T$, of the subspace from $\Sigma_2$.
    Solid segment with the same color plots the corresponding set $\mathcal{K}^s_2$ for the second column, and
    the dashed ray plots $\mathcal{W}_2$.
     }%Randomly generates the elements of first column of $K$ with $\sum_{i} K_{i,j} = 1$. Three sets of points are sampled for each plot and represented in different colors. Triangular points are ($K_{1,1}$, $K_{2,1}$) of first column; Lines are sets of points ($K_{2,1}$, $K_{2,2}$) of column 2.}
    \label{fig:2x2_subspace}
\end{figure}

Fig~\ref{fig:2x2_subspace} (a-d) illustrate the support of a $2\times 2$ sub-matrices of negative exponential costs, $\text{supp}[P(K^s|T)]$, for an observed coupling $T$ with dimension $4\times 4$.
In each plot, a $T$ is sampled columnwise according to a symmetric Dirichlet distribution with $\alpha = 1$ \footnote{See sampled $T_1,\dots,T_4$ in supplement material.}.
Consider submatrix %$\tiny K^s=\begin{pmatrix} k_{11}& k_{12} \\ k_{21} & k_{22}\end{pmatrix}$ 
$K^s = [[k_{11}, k_{12}],[k_{21}, k_{22}]]$ of $K$. 
According to section~\ref{sec:subspace}, both columns $\mathbf{k}^s_1, \mathbf{k}^s_2$ of $K^s$ lie in a copy of $\Sigma_2$. 
Each colored triangle mark represents a uniformly sampled $\mathbf{k}^s_1$. 
For each $\mathbf{k}^s_1$, the corresponding $\mathcal{K}^s_2$, the set of $\mathbf{k}^s_2$, is shown by solid segment with the same color,
and $\mathcal{W}_2$ is shown by the dashed ray.
Here, $\mathcal{K}^s_2$ is obtained by: fix $\mathbf{k}^s_1 = (k_{11}, k_{21})^T$, further sample $k_{31}$ and $k_{41}$ to form the first column of $K$.
Then compute and plot the uniquely determined $\mathbf{k}^s_2$. 
As predicted in section~\ref{sec:subspace}, $\mathcal{K}^s_2$ is only a subset of $\mathcal{W}_2$. 
The size and location of $\mathcal{K}^s_2$ in $\mathcal{W}_2$ vary according to cross ratios of $T$. %\pw{can we make this precise?}.




\paragraph{Inferring censored values.} %\pat{FIXME: consider one missing value from the Plan. Simulate inferred cost matrices, for different sized square and rectangular matrices 3, 10, 30 (crossing values).}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/missing_value_2.png}
    \caption{
    % \pat{can we make the dots bigger for the two plots on the right?} \pw{also if revise, please also fix red dot over line on the left fig.} \wt{Fixed. I did not save the values used for second column, so it changes slightly. Sorry about that. But T is the same.}
    Visualization of $\text{supp}[P(K|T)]$ for a $3\times 3$ observed $T$ with $t_{31}$ missing.
    Here $T$ is obtained by sampling each element uniformly from $[0,10]$.
    Each column of $\widehat{K}$ is plotted in a copy of $\Delta_2$ as shown.
    Colored dots in the middle $\Delta_2$ represents uniformly sampled $\mathbf{k}_2$. While
    the uniquely determined $\mathbf{k}_3$ are shown on the right, 
    the set $\mathcal{K}_1$ for the corresponding $\mathbf{k}_1$ is shown on the left.}
    % The points in the left figure are for the 1st column of $K$, middle 2nd column and right 3rd column. Points of different colors are using different randomly sampled second column of $K$. We sample 1,000 points uniformly from (0, 10) for the missing value. \pat{FIXME: punchline}
    \label{fig:missing_element_T}
\end{figure}

Figure~\ref{fig:missing_element_T} illustrate the $\text{supp}[P(K|T)]$ for a $3\times 3$ observation $T$ with $t_{31}$ missing.% \hl{FIXME}
$T = [[5.84, 4.32, 4.10],[5.90, 9.00, 4.29],[t_{31}, 5.49, 7.18]]$ is constructed by sampling each element uniformly from $[0,10]$.
Three columns of $\widehat{K}$ are plotted in three copies of $\Delta_2$ as shown.
Points for $\mathbf{k}_2$ are sampled uniformly within the middle $\Delta_2$. The uniquely determined $\mathbf{k}_3$ are shown in the right $\Delta_2$.
The corresponding set for $\mathbf{k}_1$ ($\mathcal{K}_1$) is plotted in the left $\Delta_2$.
$\mathcal{K}_1$ is obtained by randomly sampling a thousand $t_{31}$ from $[0,10]$. Each sampled $t_{31}$ uniquely determines a $\mathbf{k}_1$.
As explained in section~\ref{sec:missing_element}, each $\mathcal{K}_1$ forms a line segments. The slope of each line is determined by $T$'s cross ratios.



\paragraph{Inferring latent costs from observed basketball statistics.} 
%\pat{FIXME: infer cost matrices for 3 teams for two seasons. Compare stability of inferences for a given team across seasons. Compare correlates for quality of fit? (e.g. team's record, etc). } 
We validate the model on real-world data of performances of players in NBA teams across two seasons. 
%Such statistics are recorded on the NBA official website. 
We treat seasonal data as observed couplings between players within a team. We then infer a distribution over possible costs associated with each player on each team for the tasks they could perform on the team: points, offensive rebounds, defensive rebounds, steals, and assists. 

We conduct four sets of analyses to validate our approach. First, we compare the inferred costs for players on the same team for adjacent seasons, with the assumption that the same players' skill level will be relatively constant so each player should be similar to himself. Second, we compare inferred costs for players that change teams between seasons. Third, based on the costs inferred from one season, we predict the coupling for the subsequent season. 
Fourth, we predict, based costs inferred in one season, the cross-ratios between pairs of players the subsequent season. 
%Taken together, these validate our assumptions and test the predictive validity of our model. We detail each of these analyses below. 

The dataset was obtained by scraping NBA statistics data for the eastern conference from NBA websites.\footnote{The dataset can be downloaded from https://www.nba.com and https://www.basketball-reference.com.} For each team, we include players who played at least half of the games in 17-18 and 18-19 seasons to ensure that we have reasonably robust couplings. We included five statistical categories as features---points, offensive rebounds, defensive rebounds, steals, and assists---thus, the dimension of an observed coupling, $T$, is number of players on the team that played in at least half of the games times number of features. We convert each statistic to column normalized format, so the coupling represents the proportion contribution by each player on that statistic, and we assume a column-wise Dirichlet prior. 
For each team, we apply Algorithm 1 to draw a set of 500 cost matrices, $\mathcal{K}^{t, s}$, from the posterior distribution on costs, for team $t$ in season $s$. Full details are in the supplement. 

\textit{Stability of inferred costs across seasons for players on the same team.} 
In general, a player's abilities should be consistent in adjacent seasons. %\pat{we probably don't need the text, all of this could just be stated mathematically and be more clear} 
Thus, we may assume $\mathcal{K}^{t_b, s_c}\sim \mathcal{K}^{t_b, s_{c'}}$, where the two inferred costs are close.
%inferred the cost matrices of a team from observed couplings between players in season 17-18 ($s_c$) and season 18-19 ($s_{c'}$), the two costs for the same player should be close. 
To demonstrate it we compute the 2-Wasserstein distance between the point cloud for each player for season 17-18 ($s_c$) and season 18-19 ($s_{c'}$) and compare with the 2-Wasserstein distance between random pairs of different players. We also compare with the simple Euclidean distance between the normalized observed statistics from the two seasons as a baseline. 

%\pat{generalized notation. needs more details.}
With these sets of $\mathcal{K}$ we can calculate the 2-Wasserstein distance between point clouds of MC samples from two teams $t_b$ and $t_{b'}$ in two seasons $s_c$ and $s_{c'}$: 
\begin{equation}
    W^{p_a, t_b, s_c, p_{a'} t_{b'}, s_{c'}}_{2} = \left(\inf_{\pi\in\Pi(\mu, \nu)} \sum_{i, j} \kappa^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_{i, j}\times \pi_{i, j} \right)^{1/2},
\end{equation}
where $p_a$ indicates players from team $t_b$ and season $s_c$, $\mu$ and $\nu$ are assumed to be uniform marginals, and $i$, $j$ are the indices labeling the MC samples, and 
\begin{equation}
    \kappa^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_{i, j} = \sum_{k} (K^{p_a, t_b, s_c}_{i, k} - K^{p_{a'}, t_{b'}, s_{c'}}_{j, k})^2,
\end{equation}
where $k$ indicates the feature. $\pi$ is the EOT plan obtained by performing the Sinkhorn algorithm on $\kappa$ with uniform marginals $\mu$ and $\nu$ and a regularization strength of 0.01. We also calculate a baseline distance, which is the $L_2$ distance between two players in the observed couplings $T^{p_a, t_b, s_c}$ and $T^{p_{a'}, t_{b'}, s_{c'}}$, for comparison. 

Fig. \ref{fig:W2} shows the $W_2$ distances between inferred cost matrices within the same team across the two seasons. Player-to-self compares the $W_2$ between samples for the same player for consecutive seasons if he played in both seasons; player-to-others compares the $W_2$ of samples for one who player participated in season 1 to a randomly sampled teammate in season 2. For simplicity, we do not consider players transferred teams in mid-season. 
%\hl{wei-ting could you please update?}
In the first row columns 1-3, Gaussian kernel density estimations (KDE) for the difference between $W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2$ and min$_{p_{a'}, s_{c'}}(W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2)$ are shown, which tells us whether a player in season 1 has the minimum $W_2$ among all teammates in season 2. If so, the point clouds of the inferred costs for the player in $s_c$ and $s_{c'}$ are close; if not, we can estimate how different the costs for each player from the two seasons are.  
The last column of the first row shows the distance between point clouds we compute the two-point $L_2$ distance from $p_a$ in the observed coupling $T^{p_a, t, s_c}$ to $p_{a'}$ in $T^{p_{a'}, t, s_{c'}}$. 
In the second row, normalized histograms of ranking of $W_2$ are plotted in columns 1-3. The rank equals to 1 if $W^{p_a, t_b, s_c, p_a{'}, t_{b'} s_{c'}}_2$ is minimum among all players in $s_2$. There are peaks at rank 1 for player-to-self, which means the cost point cloud for most players in $s_{c'}$ are closest to the point cloud for same player in $s_c$. Column 4 is the ranking computed directly on the normalized observed statistics. 

\textit{Comparing inferred costs across seasons for players who change teams.} 
In Fig. \ref{fig:W2_cross_team} we measure the same metrics as in Fig. \ref{fig:W2} but consider cross teams data where $t_b \neq t_{b'}$. If $p_a = p_{a'}$, then the player is transferred from $t_b$ in $s_c$ to $t_{b'}$ in $s_{c'}$. Note that there are only eleven players who played more than or equal to half of the games in both seasons and in two different teams, so we use a larger bandwidth of 0.4 for the Gaussian KDEs to obtain smoother densities. The results are comparable to within team data, which means for those players who play enough games in the teams, the inferred costs are consistent across the two seasons even when paired with different teammates.

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c | c}
        \includegraphics[width=0.22\textwidth]{figs/W2_linear_0p1_alpha0p5.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_linear_0p1.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_linear_0p1_alpha2.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_baseline_linear_0p1.png}
    \end{tabular}
    
    \begin{tabular}{c c c | c}
        \includegraphics[width=0.22\textwidth]{figs/W2_ranking_alpha0p5.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_ranking.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_ranking_alpha2.png}
        &
        \includegraphics[width=0.22\textwidth]{figs/W2_baseline_ranking.png}
    \end{tabular}
    
    \caption{ 
    Assessing inference via comparison of costs estimated from the 17-18 and 18-19 NBA seasons for eastern conference teams. 
    %Only players who appear on the same team in both seasons are included. 
    The blue lines represent the distances between same player across the two seasons, while the orange curves represent distances between different players. Results in the first three columns show the effect of a columnwise Dirichlet prior of $\alpha$ of 0.5, 1, and 2, respectively, while the last column is a baseline estimated directly from the raw statistics (see text for further details).   
    \textbf{(top)} Probability densities of $W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2$- min$_{p_{a'}, s_{c'}}(W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2)$ estimated via Gaussian kernel density estimation with a bandwidth of 0.1. 
    \textbf{(bottom)} Histograms of the ranking of $W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2$- min$_{p_{a'}, s_{c'}}(W^{p_a, t_b, s_c, p_{a'}, t_{b'}, s_{c'}}_2)$.   
    The inferred costs for the same player are closer than inferred costs for other players, and the inferred costs are closer than the distance between the observed couplings based directly on the observed statistics. 
    %\wt{Add some discussion.}}
    }
    \label{fig:W2}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c | c}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_MC_linear_alpha0p5.png}
        & %\hspace{-2pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_MC_linear.png}
        & \hspace{5pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_MC_linear_alpha2.png}
        & %\hspace{-2pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_baseline_linear.png}
    \end{tabular}
    \begin{tabular}{c c c | c}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_ranking_MC_alpha0p5.png}
        & %\hspace{-2pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_ranking_MC.png}
        & \hspace{5pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_ranking_MC_alpha2.png}
        & %\hspace{-2pt}
        \includegraphics[width=0.22\textwidth]{figs/W2_cross_team_ranking_baseline.png}
    \end{tabular}
    
    \caption{
    Comparison of the inferred costs from 17-18 and 18-19 seasons for all eastern conference teams for players who switched teams. The plots in this figure are similar to Fig. \ref{fig:W2}, and we similarly find that distances between inferred costs for the same player are smaller than between different players and smaller than distances based directly on the observed statistics. 
    % The probability densities of the 2-Wasserstein distances for players who transfer from one team to another. The blue curves are for players comparing to themselves across the two seasons, while the orange curves are for players comparing to other players in the team. We apply Gaussian kernel density estimation with a bandwidth of 0.4 on the curves. The inferred costs for the same player are closer than inferred costs for other players, and the inferred costs are closer than the distance between the observed couplings based on the raw statistics.
    %$W_2$ for players transfer from one team to the other. 
    %Bandwidth = 0.4 due to less player-to-self data points.}
    }
    \label{fig:W2_cross_team}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{tabular}{c c c c}
        \includegraphics[width=0.47\textwidth]{figs/KDE_transfer_prediction.png}
        &
        \includegraphics[width=0.47\textwidth]{figs/KDE_transfer_CR.png}
    \end{tabular}
    \caption{Predicting player performance based on the previous season's inferred costs. \textbf{(left)} The blue curve plots the KDE of the $L_2$ distance between the predicted couplings for the assembled team, $\tilde{T}$ and the observed coupling, $T$. The orange curve plots the KDE of the $L_2$ distance but we shuffle the elements in $\tilde{K}$ and then compute the EOT plan, $\tilde{T}^{shfl}$. \textbf{(right)} The blue curve represents the KDE of the $L_2$ distance between the log of the cross-ratio matrices of the negative log of the cost for the assembled team and the log of the cross-ratio matrix of the observed coupling. The orange curve plots the same KDE of the $L_2$ distance but the elements in $\tilde{K}$ are shuffled. The bandwidths of the KDE are 0.2.}
    \label{fig:KDE_transfer}
\end{figure}

%\pw{Discuss: what are the two marginal spaces we have in mind here: players vs some statistics? a bit careful with the marginal distributions}

%\paragraph{Testing inferences via changes in teammates.} 
%\pat{this is predicting how new team will do with added player. compare statistics (coupling)?}
\textit{Predicting future relative performance between players.} 
We predict the team coupling between players in season 2 based on the inferred cost from season 1. We pick two teams, Chicago Bulls as $t_b$ and Orlando Magic as $t_{b'}$, and a player, Jerian Grant, who transferred from $t_b$ to $t_{b'}$ after the 17-18 season. ($s_c$ = 17-18 season and $s_{c'}$ = 18-19 season.) We first take the observed season 1 couplings for $t_b$ and $t_{b'}$ and utilize algorithm 1 to generate inferred cost matrices, $\mathcal{K}^{t_b, s_c}$ and $\mathcal{K}^{t_{b'}, s_{c'}}$, with 500 of each. Then, we compose new cost matrices, $\tilde{\mathcal{K}}^{t_{b'}, s_c}$, by taking the inferred costs from seven static $t_{b'}$ players and the new player who transferred into $t_{b'}$ from $t_b$. All combinations are considered with a total number of 250,000 in $\tilde{\mathcal{K}}^{t_{b'}, s_c}$. With the assumption that the cost for each player does not change in adjacent seasons, we assume $\tilde{\mathcal{K}}^{t_{b'}, s_{c'}} \sim \tilde{\mathcal{K}}^{t_{b'}, s_c}$, and the predicted coupling for the new team in season 2, $\tilde{\mathcal{T}}^{t_{b'}, s_{c'}}$, is computed by solving the EOT problem for $\tilde{\mathcal{K}}^{t_{b'}, s_{c'}}$. We use uniform column marginal and take the row marginal from the observed coupling $T^{t_{b'}, s_{c'}}$. The $L_2$ distance between the predicted couplings and the observed eight-player coupling, $D(\tilde{T}^{t_{b'}, s_{c'}}, T^{t_{b'}, s_{c'}})$, can be calculated. 

As a baseline, we compute the the distance between the shuffled couplings, $\tilde{T}^{t_{b'}, s_{c'}, shfl}$, and $T^{t_{b'}, s_{c'}}$.  The shuffled couplings are obtained by shuffling all the matrix elements randomly in $\tilde{K}^{t_{b'}, s_{c'}}\in\tilde{\mathcal{K}}^{t_b'{}, s_{c'}}$ and solve the EOT problems for each matrix. The Gaussian KDEs with bandwidth = 0.2 for the distances are shown in the left panel of Fig. \ref{fig:KDE_transfer}. The blue curve is narrow and the mean value is about half of the orange curve, which suggests that (1) the predicted couplings from all combinations of sample costs are close to each other and (2) the distances from the predicted couplings to the observed coupling are substantially smaller than the distances from bootstrapped random matrices to the observed coupling. 

\textit{Predicting relative relationship between players who change teams.}
Next, we investigate the relationship between the cross-ratio \citep{pei2019generalizing,NEURIPS2020_cc58f7ab} of $\tilde{K}^{t_{b'}, s_{c'}}$ and $T^{t_{b'}, s_{c'}}$. We build the cross-ratio matrices, $CR(M)$, whose elements are the cross-ratio of 2$\times$2 sub-matrices of $M$. The 2$\times$2 sub-matrices are built from $M_{sub} = [[M_{ij}, M_{il}], [M_{kj}, M_{kl}]]$ with $i<k$  $\forall i \in [1, m), k\in (1, m]$ and $j<l$ $\forall j \in [1, n), l\in (1, n]$.
%\wt{Is this accurate?}\hl{No. cr=ad/bc or log(cr)=log(ad/bc); det=ad-bc}\pat{please make sure computations are correct!} \wt{Computations are correct. I should not write determinant here. I am not sure what I was thinking.}
%\pat{also, we should be a bit more precise. what is the dimension of M here? it is 2x5, correct? and we construct a set of 4 minimally sufficient CRs. (there are more but they don't contain additional information)}\wt{Dimension of M is 8$\times$5, 8 for 1 (new) + 7 (static) players and 5 features. I took all 2x2 sub-matrices. }
The distances between log$[CR(\tilde{K}^{t_{b'}, s_{c'}})]$ and log$[CR(T^{t_{b'}, s_{c'}})]$ are plotted in the right panel of Fig. \ref{fig:KDE_transfer}. %Gaussian KDE with bandwidth = 0.2 is applied. \pat{this is in the caption}
The result from $\tilde{K}^{t_{b'}, s_{c'}}$ is narrow, suggesting that (1) the cross-ratio of the inferred cost matrices are consistent. The result from shuffled matrices (orange curve) is wide spread and the average is three times larger than the non-shuffled result, suggesting that (2) 
%(2) the randomness breaks the cross-ratio equivalence \wt{Citation.} of matrix scaling and 
our method accurately predicts the observed cross-ratios. 
%finds cost matrices with cross-ratio closer to the observed coupling. 

%\pat{1) compare players on the same team across adjacent seasons in terms of inferred costs}
%\pat{1b) plot frequency of ranking between player and self}
%\pat{2) compare players who have changed teams across adjacent seasons in terms of inferred cost} 
%\pat{3) predict team plan for season 2 based on season 1 by composing the inferred costs and computing the predicted plan. Marginals taken from second season.}
%\pat{3b) compare cross ratios predicted based on cost estimates, versus observed.}
%\pat{4) censored value prediction}

%\pat{redo all above analyses with two additional alpha values, one greater than 1, one less than one}

\section{Related work}

Although the inverse optimal transport problem is usually ill-posed, researchers have been tackling it with various approaches. 
The most common approach is to impose additional structure on the problem to turn it into an optimization problem. 
For example, \cite{dupuy2019estimating} parameterize the cost by a bilinear form with an affinity matrix and used proximal gradient descent algorithm to find a solution to the affinity matrix by solving the EOT problem and regularizing the low-rank singular values of the affinity matrix iteratively.
\cite{li2019learning} model the cost by a nonlinear kernel representation. 

Related approaches, largely the lovely work of Curturi and colleagues, formulate the problem as ground metric learning. 
\cite{cuturi2014ground} proposed algorithms for Ground Metric Learning (GML) which learns a distance from labeled normalized histograms given a criterion.
\cite{heitz2021ground} extended the work of GML to learn the ground metric where only a geodesic distance on a graph is considered.
\cite{paty2020regularized} re-interpreted regularized OT problems as ground cost adversarial and solved for robust solutions robust under different regularization. 

\cite{stuart2020inverse} utilized a probablistic approach to formulate inverse OT problems. They modeled the probability of observing a noisy coupling as the posterior distribution of a cost using a domain model to specify the underlying costs and solved via MCMC. 

Our work differs from these approaches by formulating the general probabilistic inference problem, providing insight into the geometric foundations, and general MCMC methods that derive from the geometric foundations. 

%\cite{dupuy2019estimating} proposed a method to solve the inverse OT problem, where they parametrized the cost by a bilinear form with an affinity matrix and used proximal gradient descent algorithm to find a solution to the affinity matrix by solving the EOT problem and regularizing the low-rank singular values of the affinity matrix iteratively. They applied the inverse low-rank OT method to marriage market data. Another similar work was done by \cite{li2019learning}, where instead of using a bilinear form for the cost they proposed to model the cost by a nonlinear kernel representation and solved the robust inverse optimal transport (RIOT) problem with regularized Wasserstein distance for marginal relaxation. The RIOT method was applied to synthetic, election, New York taxi, and marriage data sets in their work. %\pat{quick sentence stating the most important way(s) we are different}

%\cite{stuart2020inverse} utilized a Bayesian approach to formulate inverse OT problems, where they modeled the probability of observing a noisy coupling as the posterior distribution of a cost. They proposed to solve the IOT problem by minimizing the model-data misfit using Markov-chain-Monte-Carlo methods where only a random number generator and solution of the OT problems are needed. Their method was used to investigate the European migration flows. 
%\pat{quick sentence stating the most important way(s) we are different}

%\cite{cuturi2014ground} proposed algorithms for Ground Metric Learning (GML) which learns a distance from labeled normalized histograms given a criterion. They applied a projected sub-gradient descent algorithm to minimize the difference between the OT distance of a metric matrix and the similarity for pairs of histograms, so observed movement of histograms is optimal under the ground metric. \cite{heitz2021ground} extended the work of GML to learn the ground metric where only a geodesic distance on a graph is considered.   %\pat{quick sentence stating the most important way(s) we are different}

%\cite{paty2020regularized} re-interpreted regularized OT problems as ground cost adversarial. They proposed algorithms, such as gradient ascent and Sinkhorn-like,  to solve robust adversarial cost OT problem with different forms of regularization. %\pat{quick sentence stating the most important way(s) we are different}

%Inspired by the above works we tackle IOT problems with a probabilistic formulation. We study the geometry and characterize the manifold of IOT problems, propose a MCMC approach to infer latent costs from observed couplings, demonstrate effectiveness of probabilistic inference without detailed domain assumptions, and successfully apply our method to real-world datasets. Our approach can be useful for inferring the underlying costs of heavily cooperative team compositions of agents with observations or measurements of couplings between team members and a simple assumption on the prior. 

% \pat{or just one paragraph stating why we are *importantly* different from these! we characterize the geometry, we directly derive an MCMC approach from EOT, and we demonstrate effectiveness of probabilistic inference without detailed domain assumptions. others?}

%\pw{connection to IOT when $T$ is perfectly observed!!}

% \pat{talk about migration paper} \cite{stuart2020inverse}\wt{done}

% \pat{talk about matching paper} \cite{li2019learning}\wt{done}

% \pat{talk about paty and curuti paper}\wt{done}

% \pat{OTHERS?????}

% \wt{Cuturi and Avis 2014, Ground metric learning} \cite{cuturi2014ground}

% \wt{Heitz et al. 2020, Ground metric learning on graphs} \cite{heitz2021ground}

\section{Conclusions}

Couplings are stochastic matchings in which the observed solution reflects trade offs between latent costs.  
We presented an analysis of probabilistic Inverse Optimal Transport which infers latent costs from observed couplings. 
In contrast with prior work on IOT, we consider the geometric foundations inherited from Sinkhorn scaling of entropy-regularized Optimal Transport. We analyze the support of the cost matrices associated with an observed coupling, the implications of prior distributions on costs, and introduce an MCMC algorithm for posterior inference. Our model performs well in validations on synthetic data, and on a real-world dataset of NBA players. 
%Inferring the costs from noisy coupling or limited samples of coupling makes the problem unstable and may require a more complex model to solve it. We plan to extend our work to such problems in the future. 

\newpage

\section*{Broader Impact}
%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences.
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a)
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages biases in the data. If authors believe this is not applicable to them, authors can simply state this.
This work provides a potential application to predict the future performance of teams. It could benefit people who seek to form such teams. 
In contrast with independent evaluation (e.g. testing), the method is based directly on performance, and therefore avoids biases introduced by such tests. However, the approach should not be considered bias-free. Answers to this and other basic questions are important directions for future work. 
%However, some player who has the potential to be a key player might be undiscovered or ignored because of his predicted score is low based on the simulations of our model. 
%On the contrary, if the predicted score for a player is high but the actual performance is not as good as expected, the player might suffer from high social pressure and depression. 
%We should also be careful on the malicious usage of our method. For example, people might use it to predict results of games for illegal gambling. 
%\hl{FIXME}



% \textbf{Global moves}
% \pat{i don't think this is a proper MH proposal. also, i don't think we need it. If we are concerned that the algorithm gets trapped in minima, we can just run multiple independent chains, which is proper.}
% During the simulation, the columns of the matrix stuck at the same vertex of the simplex from time to time. We propose a global move shown in algorithm 2 in order to mitigate this problem. The global move can transfer the columns from a vertex to center of a simplex efficiently by re-scaling the rows.

% \begin{algorithm}[H]
% \caption{Global move}
% Inputs: Matrix $M_i, $Threshold $th$, Dirichlet concentration $\mu$, uniform random variable rv $\in$ [0, 1)\;
% \For{k = 1 to $N_r$}{
%     ROWSUM$_k$ = $\sum_{l=1}^{N_c} M_{i, kl}$ \;
%     \If{ROWSUM$_k$<$th$}{
%         $M_{i+1, k} \leftarrow M_{i, k}$ / ROWSUM$_k$\;
%     }
%     ratio $\leftarrow Dir(M_{i+1}, \mu) / Dir(M_i, \mu)$\;
%     \eIf{ratio > rv}{
%         Accept $M_{i+1}$\;
%     }{
%         Reject $M_{i+1}$\;
%         $M_{i+1} \leftarrow M_{i}$
%     }
% }
% \end{algorithm}
